Design and Testbed Deployment of Frequency-Domain Equalization Full Duplex Radios

Full-duplex (FD) wireless can significantly enhance spectrum efficiency but requires effective self-interference (SI) cancellers. RF SI cancellation (SIC) via frequency-domain equalization (FDE), where bandpass filters channelize the SI, is suited for integrated circuits (ICs). In this paper, we explore the limits and higher layer challenges associated with using such cancellers. We evaluate the performance of a custom FDE-based canceller using two testbeds; one with mobile FD radios and the other with upgraded, static FD radios in the PAWR COSMOS testbed. The latter is a lasting artifact for the research community, alongside a dataset containing baseband waveforms captured on the COSMOS FD radios, facilitating FD-related experimentation at the higher networking layers. We evaluate the performance of the FDE-based FD radios in both testbeds, with experiments showing 95 dB overall achieved SIC (52 dB from RF SIC) across 20 MHz bandwidth, and an average link-level FD rate gain of 1.87x. We also conduct experiments in (i) uplink-downlink networks with inter-user interference, and (ii) heterogeneous networks with half-duplex and FD users. The experimental FD gains in the two types of networks depend on the users' SNR values and the number of FD users, and are 1.14x-1.25x and 1.25x-1.73x, respectively, confirming previous analytical results.

==> tex/algo.tex <==
$\OptProblem$ in Section~\ref{sec:background} indicates that given the RF canceller design, optimal canceller configuration is required to achieve the best RF SIC performance.
% In addition, two realistic models, $\ICTF(f_k)$ {\eqref{eq:rfic-tf}} and $\PCBTF(f_k)$ {\eqref{eq:pcb-tf}} are presented for our RFIC and PCB canceller implementations.
In this section, we present the optimization of the FDE-based RF canceller configuration based on realistic canceller models presented in Section~\ref{sec:impl}. We also derive a closed-form, near-optimal RFIC canceller configuration with $1$ FDE tap and under an ideal antenna interface. We also show that our proposed canceller configuration optimization outperforms the previously proposed iterative configuration algorithm.

% Based on the practical FDE-based RF canceller models described in Section~\ref{sec:impl}, efficient algorithms are required to optimize the configuration for each FDE tap, $\ICPCBTapTF{i}(f_k)$, to best emulate the antenna interface response, $\AntTF(f_k)$. However, there are two main challenges: (i) the real-world antenna response is non-ideal and experience high variance, and (ii) it is difficult to main analytical tractability when optimizing the joint response of multiple non-convex, complex functions.

%%
\subsection{Optimization of Canceller Configuration}
\label{ssec:algo-opt}
We present a general optimization framework that jointly optimizes all the FDE taps in the FDE-based cancellers. Although our implemented RFIC and PCB cancellers have only two FDE taps, both their models and the optimization of canceller configuration can be easily extended to the case with a larger number of FDE taps. The inputs to the FDE-based canceller configuration optimization are: (i) the RFIC or PCB canceller model with given number of FDE taps, $\NumTap$, (ii) the antenna interface response, $\AntTF(f_k)$, and the desired RF SIC bandwidth $\{f_k\}$. Then, the optimized canceller configuration are obtained by respectively solving the optimization problems $\OptProblemIC$ or $\OptProblemPCB$, in which $\ICTF(f_k)$ is given by {\eqref{eq:rfic-tf}} and $\PCBTF(f_k)$ is given by {\eqref{eq:pcb-tf-calibrated}}.
%%
\begin{align*}
\OptProblemIC\ \min: &\ \littlesum_{k=1}^{\NumChnl} \NormTwo{\ICResTF(f_k)} = \littlesum_{k=1}^{\NumChnl} \NormTwo{ \AntTF(f_k) - \ICTF(f_k) }^2 \\
\textrm{s.t.:} &\ \ICTapAmp{i} \in [\ICTapAmpMin, \ICTapAmpMax],\ \ICTapPhase{i} \in [-\pi, \pi], \\
&\ \ICTapCF{i} \in [\ICTapCFMin, \ICTapCFMax],\ \ICTapQF{i} \in [\ICTapQFMin, \ICTapQFMax],\ \forall i.
\end{align*}
%%
\begin{align*}
\OptProblemPCB\ \min: &\ \littlesum_{k=1}^{\NumChnl} \NormTwo{\PCBResTF(f_k)} = \littlesum_{k=1}^{\NumChnl} \NormTwo{ \AntTF(f_k) - \PCBTF(f_k) }^2 \\
\textrm{s.t.:} &\ \PCBTapAmp{i} \in [\PCBTapAmpMin, \PCBTapAmpMax],\ \PCBTapPhase{i} \in [-\pi, \pi], \\
&\ \PCBTapCFCap{i} \in [\PCBTapCFCapMin, \PCBTapCFCapMax],\ \PCBTapQFCap{i} \in [\PCBTapQFCapMin, \PCBTapQFCapMax],\ \forall i.
\end{align*}
%%

Note that the objectives of $\OptProblemIC$ and $\OptProblemPCB$ are non-convex and non-linear due to the specific forms of the configuration parameters such as (i) the higher-order terms introduced by $f_k$ in the canceller models (see {\eqref{eq:rfic-tf}} and {\eqref{eq:pcb-tf-calibrated}}), and (ii) non-linear, non-convex trigonometric terms introduced by the phase controls, $\ICTapPhase{i}$ and $\PCBTapPhase{i}$. Moreover, the non-ideal, time-varying antenna interface, $\AntTF(f_k)$, makes the optimization problem more challenging.
% Even for the RFIC canceller model {\eqref{eq:rfic-tf}} using $2^{\rm nd}$-order BPFs with an ideal antenna interface response,
In general, it is difficult to maintain analytical tractability of $\OptProblemIC$ or $\OptProblemPCB$. Therefore, a non-linear optimization solver is used to solve $\OptProblemIC$ and $\OptProblemPCB$, where the obtained canceller configuration may only be locally optimal (thus not globally optimal). However, in practice, it is unnecessary to obtain the globally optimal solution to $\OptProblemIC$ or $\OptProblemPCB$ as long as the local minimum achieved is sufficiently good, which we will show later in Sections~\ref{sec:eval-rfic} and~\ref{sec:eval-pcb}. In our FD radio design described in Section~\ref{sec:eval-pcb}, the optimized PCB canceller configuration can be obtained in less than $\SI{10}{ms}$ via a non-optimized solver.
% The conventional RF canceller~\cite{fd_demo_mobihoc16} which can only emulate the antenna interface response, $\AntTF(f_k)$, at a single frequency point, the key idea here is to use all the $\NumTap$ filter taps to jointly emulate the $\AntTF(f)$ \emph{across the desired bandwidth} $\BW = [f_1,f_\NumChnl]$.
% Essentially, solving optimizations $\OptProblemIC$ and $\OptProblemPCB$ allows the FDE-based cancellers to match with $\AntTF(f)$ not only in both amplitude and phase across the desired bandwidth, but more importantly, with the slope of the amplitude and the slope of phase (i.e., group delay).

%%
% \noindent\textbf{Optimization Algorithm}:
% \begin{enumerate}[topsep=0pt,leftmargin=*]
% %
% \item[1.]
% Given the number of FDE taps, $\NumTap$, desired RF SIC bandwidth $\BW = [f_1,f_\NumChnl]$, and the antenna interface response, $\AntTF(f_k)$;
% %
% \item[2.]
% Solve the following optimization problem $\OptProblemICPCB$ with a given RF canceller model using a nonlinear optimization solver:
% %
% %%
% \begin{align*}
% \OptProblemICPCB\ \min &\ \sum_{k=1}^{\NumChnl} \NormTwo{ \AntTF(f_k) - \ICPCBTF(f_k) }^2 \\
% \textrm{s.t.} &\ \ICTF(f_k)\ \textrm{in}\ {\eqref{eq:rfic-tf}}\ \textrm{with variables}\ \{\ICTapAmp{i}, \ICTapPhase{i}, \ICTapCF{i}, \ICTapQF{i}\},\ \forall i,\ \textrm{or} \\
% &\ \PCBTF(f_k)\ \textrm{in}\ {\eqref{eq:pcb-tf-calibrated}}\ \textrm{with variables}\ \{\PCBTapAmp{i}, \PCBTapPhase{i}, \PCBTapCFCap{i}, \PCBTapQFCap{i}\},\ \forall i.\ \Box
% \end{align*}
% %%
% \end{enumerate}
%%


%% Joint optimization
% \begin{algorithm}[!h]
% \caption{Joint Optimization for the FDE Canceller}
% \label{algo:opt-joint}
% \begin{algorithmic}[1]
% % input
% \State
% Input: The number of FDE taps, $\NumTap$, the desired RF SIC bandwidth, $f_k \in [f_1,\cdots,f_K]$, and the antenna interface response, $\SIChnlTF(f_k)$,
% % solve opt
% \State
% Solve the following optimization problem using a gradient descent method:
% \begin{align}
% \min:\ & \littlesum_{k=1}^{K} \NormTwo{ \SIChnlTF(f_k) - \littlesum_{i=1}^{N} \ICPCBTapTF{i}(f_k) }^2 \nonumber \\
% \textrm{subject to}:\
% & \textrm{Variable tuning range}, \nonumber
% \end{align}
% % return
% \State
% Return the filter tap configuration.
% \end{algorithmic}
% \normalsize
% \end{algorithm}
%%


%%
%%
% \subsection{RFIC Canceller with One FDE Tap}
% \label{ssec:algo-example}
% Although it is difficult to maintain analytical tractability of $\OptProblemIC$ or $\OptProblemPCB$, if we assume that the antenna interface has an ideal response with constant amplitude of $A_{\rm SI} = |\AntTF(f_k)|$ and a constant group delay of $\tau_{\rm SI}$ (e,g., $\AntTF(f_k) = A_{\rm SI} e^{-j2\pi f_k\tau_{\rm SI}}$)\footnote{This is a reasonable assumption from our measurements (e.g., see $\AntTF(f_k)$ in Fig.~\ref{fig:exp-usrp-algo}).}, a closed-form near-optimal\footnote{This configuration is not truly optimal since approximations are applied.} configuration can be derived for the RFIC canceller with $1$ FDE tap. As we will show below, the results in this case also reveal interesting trade-offs between the amount of RF SIC that can be achieved and the desired RF SIC bandwidth. 

% We drop the subscript $i$ and superscript $\textrm{I}$ below for brevity. Let $P(f_k) := \QF{} (\CFNoidx/f_k-f_k/\CFNoidx)$, the frequency response of the RFIC canceller {\eqref{eq:rfic-tf}} with $1$ FDE tap is given by
% %%
% \begin{align}
% \label{eq:rfic-tf-expand}
% \TF{}(f_k) & = \Amp{} \cdot \frac{ 1 + jP(f_k) }{1+P^2(f_k)} \left(  \cos{\Phase{}} - j\sin{\Phase{}} \right) \nonumber \\
% & = \Amp{} \cdot \frac{(\cos{\Phase{}} + P(f_k)\sin{\Phase{}}) + j(-\sin{\Phase{}} + P(f_k)\cos{\Phase{}})}{1+P^2(f_k)} \nonumber \\
% & = \Amp{} \cdot (1+P^2(f_k))^{-1/2} \cdot e^{-j(\Phase{} - \tan^{-1}P(f_k))},
% \end{align}
% %%
% where the last step comes from the fact that
% %%
% \begin{align*}
% & \quad \left( \cos{\Phase{}} + P(f_k)\sin{\Phase{}} \right) + j \left( -\sin{\Phase{}} + P(f_k)\cos{\Phase{}} \right) \\
% & = (1+P^2(f_k))^{1/2} \cdot e^{-j(\Phase{}-\tan^{-1}P(f_k))}
% \end{align*}
% %%
% For $|f_k-\CFNoidx| \ll \CFNoidx$, it holds that $P(f_k) \approx -2\QF{}(f_k-\CFNoidx)/\CFNoidx \ll 1$. Applying the approximations $(1+x^2)^{-1/2} \approx (1-x^2/2)$ and $\tan^{-1}x \approx x$ as $x \to 0$ to {\eqref{eq:rfic-tf-expand}} yields $\TF{}(f_k) \approx \TFApprox{}(f_k) := \widetilde{\Amp{}}(f_k) e^{-j\widetilde{\ICTapPhase{}}(f_k)}$,
% where $\widetilde{\Amp{}}(f_k) := \Amp{} ( 1-P^2(f_k)/2 )$ and $\widetilde{\Phase{}}(f_k) := \Phase{}-P(f_k)$. Then, the optimal configuration of the RFIC canceller with one FDE tap can be obtained by solving $\OptProblemIC$,
% %%
% \begin{align}
% \label{eq:example-opt-obj}
% & \min:\ \littlesum_{k=1}^{K} \NormTwo{ \AntTF(f_k) - \TFApprox{}(f_k) }^2 \\
% & \textrm{s.t.:}\ \Amp{}>0,\ \Phase{} \in [-\pi, \pi],\ \CFNoidx >0,\ \QF{} > 0.
% \end{align}
% %%
% From basic trigonometric equations, we have for $\forall f_k$,
% %%
% \begin{align*}
% & | \AntTF(f_k) - \TFApprox{}(f_k) |^2 = | A_{\rm SI} e^{-j2\pi f_k \tau_{\rm SI}} - \widetilde{\Amp{}}(f_k) e^{-j\widetilde{\Phase{}}(f_k)} |^2 \\
% & \quad = (A_{\rm SI})^2 + (\widetilde{\Amp{}}(f_k))^2 - 2A_{\rm SI}\widetilde{\Amp{}}(f_k) \cos{(2\pi f_k \tau_{\rm SI} - \widetilde{\Phase{}}(f_k))}
% \end{align*}
% %%
% Using approximation $P(f_k) \approx -2\QF{}(f_k-\CFNoidx)/\CFNoidx$ yields
% %%
% \begin{align*}
% \widetilde{\Phase{}}(f_k) = \Phase{} - P(f_k) \approx \Phase{} + 2\QF{}(f_k-\CFNoidx)/\CFNoidx.
% \end{align*}
% %%
% By setting $\Phase{} = 2\pi\CFNoidx\tau_{\rm SI}\ (\textrm{mod}\ 2\pi)$ and $\QF{} = \pi\CFNoidx\tau_{\rm SI}$, we have $\widetilde{\Phase{}}(f_k) = 2\pi f_k \tau_{\rm SI},\ \forall k$. Therefore, {\eqref{eq:example-opt-obj}} becomes
% %%
% \begin{align}
% \label{eq:example-opt-obj-approx}
% \min:\ \littlesum_{k=1}^{K} \NormTwo{ \Amp{\textrm{SI}} - \Amp{} ( 1-2\pi^2\tau_{\rm SI}^2 (f_k-\CFNoidx)^2 ) }^2,
% \end{align}
% %%
% which is a quadratic function with respect to the FDE tap amplitude, $\Amp{}$, whose optimal value is given by
% %%
% \begin{align}
% \label{eq:example-opt-obj-approx-amp}
% \Amp{} = \Amp{\textrm{SI}} \cdot \left(\littlesum_{k=1}^{K} \gamma_k\right) \big/ \left(\littlesum_{k=1}^{K} \gamma_k^2\right),\ \gamma_k := 1-2\pi^2\tau_{\rm SI}^2 (f_k-\CFNoidx)^2.
% \end{align}
% %%
% Therefore, the near-optimal configuration of the FDE tap given its center frequency $\CFNoidx$, which can be selected as the center frequency of the desired SIC bandwidth (i.e., $\CFNoidx = f_{\NumChnl/2}$), is given by
% %%
% \begin{align}
% \Amp{}\ \textrm{in}\ {\eqref{eq:example-opt-obj-approx-amp}},\ \Phase{} = 2\pi f_c \tau_{\rm SI}\ (\textrm{mod}\ 2\pi),\ \textrm{and}\ \QF{} = \pi \CFNoidx \tau_{\rm SI}.
% \end{align}
% %%
% {\eqref{eq:example-opt-obj-approx}} and {\eqref{eq:example-opt-obj-approx-amp}} show that as the desired RF SIC bandwidth increases (i.e., $|f_k-\CFNoidx|$ increases for given values of $\CFNoidx$ and $K$), the residual SI power level {\eqref{eq:example-opt-obj-approx}} increases, resulting in degraded RF SIC performance.


%%
%%
% \subsection{Iterative Configuration Algorithm}
% \label{ssec:algo-iter}
% In~\cite{Zhou_WBSIC_JSSC15}, an iterative configuration algorithm was proposed to find the RFIC canceller configuration. Specifically, the first FDE tap $\ICTapTF{1}(f_k)$ is optimized to match with the amplitude and phase and their slopes of the antenna interface at a given cancellation frequency $f_{\textrm{canc}, 1}$. Then, the second FDE tap $\ICTapTF{2}(f_k)$ is optimized to match with those of the residual SI channel ($\AntTF(f_k) - \ICTapTF{2}(f_k)$), at a different cancellation frequency $f_{\textrm{canc}, 2}$. We generalize this iterative configuration algorithm based on both the RFIC and PCB canceller models as the process below.
% %%
% \begin{enumerate}[topsep=0pt, leftmargin=*]
% \item[1.]
% Given the FDE-based canceller model with $\NumTap$ FDE taps, the desired RF SIC bandwidth $\{f_k\}$, the antenna interface response, $\AntTF(f_k)$. Select a sequence of cancellation frequencies, $\{f_{\textrm{canc}, i}\}_{i=1}^{\NumTap}$, and set the initial residual SI channel as $\ResTapTF{0}(f_k) = \AntTF(f_k)$;
% %
% \item[2.]
% For $\forall i$, solve for the configuration of the $i^{\rm th}$ FDE tap such that $\ResTapTF{i-1}(f_k)$ and $\RFCancTapTF{i}(f_k)$ are equal in amplitude, phase, and the slopes of amplitude and phase, at cancellation frequency $f_{\textrm{canc},i}$. Update the residual SI channel by setting $\ResTapTF{i}(f_k) = \ResTapTF{i-1}(f_k) - \RFCancTapTF{i}(f_k)$.
% \end{enumerate}
% %%
% For the RFIC canceller {\eqref{eq:rfic-tf}}, closed-form solutions of $\{\ICTapAmp{i}, \ICTapPhase{i}, \ICTapCF{i}, \ICTapQF{i}\}$ when solving step 2 can be obtained by simple analysis~\cite{Zhou_WBSIC_JSSC15}. For the PCB canceller {\eqref{eq:pcb-tf-calibrated}}, $\{\PCBTapAmp{i}, \PCBTapPhase{i}, \PCBTapCFCap{i}, \PCBTapQFCap{i}\}$ can be obtained easily by solving step 2 numerically.

% In Section~\ref{ssec:eval-rfic-compare}, we compare the RFIC canceller performance under both the iterative configuration algorithm and with the optimized canceller configuration. As we will show, the iterative configuration algorithm performs poorly since it does not jointly optimize all the FDE taps. More importantly, the introduction of a new $i^{\rm th}$ FDE tap, $\RFCancTapTF{i}(f_k)$, will adversely affect the residual SI channel $\ResTapTF{i-1}(f_k)$ from the previous iteration (see step 2) at its cancellation frequency $f_{\textrm{canc}, i-1}$. Despite one strength which is its low complexity, it also remains unclear how the cancellation frequencies, $f_{\textrm{canc,} i}$, can be optimally selected for the FDE taps.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/append_pcb_model.tex <==
We use transmission (ABCD) matrix to derive $\BPFTapTF{i}(f)$, given by {\eqref{eq:pcb-bpf-tf}}. From Fig.~\ref{fig:diagram-pcb} and $Y_{\textrm{F}}(f_k)$ and $Y_{\textrm{Q}}(f_k)$ in {\eqref{eq:pcb-admittance}},
% \footnote{We use subscripts $A$, $B$, $C$, and $D$ to denote the entries in the $2 \times 2$ matrix.}
%%
\begin{align}
\hspace*{-10pt}
\begin{bmatrix}
V_{\textrm{in}} \\ I_{\textrm{in}}
\end{bmatrix}
& =
\begin{bmatrix}
1 & 0 \\ Y_{\textrm{Q}}(f_k) & 1
\end{bmatrix}
% \times
\mathbf{M}^{\textrm{TL}}
% \times
\begin{bmatrix}
1 & 0 \\ Y_{\textrm{F}}(f_k) & 1
\end{bmatrix}
% \nonumber \\
% & \qquad \times
\mathbf{M}^{\textrm{TL}}
% \times
\begin{bmatrix}
1 & 0 \\ Y_{\textrm{Q}}(f_k) & 1
\end{bmatrix}
% \times
\begin{bmatrix}
V_{\textrm{out}} \\ I_{\textrm{out}}
\end{bmatrix}
\nonumber \\
& :=
\begin{bmatrix}
M_{A}^{\textrm{BPF}}(f_k) & M_{B}^{\textrm{BPF}}(f_k) \\
M_{C}^{\textrm{BPF}}(f_k) & M_{D}^{\textrm{BPF}}(f_k)
\end{bmatrix}
\begin{bmatrix}
V_{\textrm{out}} \\ I_{\textrm{out}}
\end{bmatrix},
\label{eq:pcb-bpf-matrix}
\end{align}
%%
where $\mathbf{M}^{\textrm{TL}}$ is the ABCD matrix of a T-Line with wavenumber $\beta$, characteristic impedance $Z_0$, and length $l$, i.e., 
%%
\begin{align}
\label{eq:pcb-tl-matrix}
\mathbf{M}^{\textrm{TL}} & = 
\begin{bmatrix}
\cos{(\beta l)} & jZ_{0}\sin{(\beta l)} \\
j\sin{(\beta l)}/Z_{0} & \cos{(\beta l)} \\
\end{bmatrix}.
% :=
% \begin{bmatrix}
% a & bZ_{0} \\
% b/Z_{0} & a \\
% \end{bmatrix}
\end{align}
%%
With the parameters described in Section~\ref{ssec:impl-pcb}, the frequency response of the implemented PCB BPF, $\BPFTapTF{i}(f_k)$, is given by
%%
\begin{align}
% \label{eq:pcb-bpf-tf}
& \BPFTapTF{i}(f_k) = \frac{V_{\textrm{out}}(f_k)}{V_{\textrm{in}}(f_k)} = \frac{1}{R_{\textrm{S}}} \cdot \frac{V_{\textrm{out}}(f_k)}{I_{\textrm{in}}(f_k)} = \frac{1}{R_{\textrm{S}}} \cdot \frac{1}{M_C^{\textrm{BPF}}(f_k)}. \nonumber % \\
% & \quad = R_s^{-1} \Big[ a^2Y_1(f) + 2(a^2+b^2)Y_2(f) + 2abZ_02Y_1(f)Y_2(f_k) \nonumber \\
% & \qquad + abZ_0(Y_2(f))^2 + b^2Y_1(f)(Y_2(f))^2Z_0^2 + 2ab/Z_0 \Big]^{-1},
\end{align}
%%
Plugging {\eqref{eq:pcb-admittance}} and {\eqref{eq:pcb-tl-matrix}} into {\eqref{eq:pcb-bpf-matrix}} yields the model $\BPFTapTF{i}(f)$.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/cosmos.tex <==
\addedMK{In this section, we describe an open-access, remotely accessible testbed for FD experimentation integrated in the COSMOS testbed~\cite{raychaudhuri2020challenge}. The testbed features four improved PCBs which implement the canceller circuit described in Section~\ref{ssec:impl-pcb}. We also present the results from a version of the UL-DL experiment from Section~\ref{sssec:exp-net-ul-dl} implemented on the testbed.}

\subsection{Integration of the FDE Canceller}
\label{ssec:cosmos-integration}
An initial version of the testbed integration was presented in~\cite{kohli2021open}. The testbed makes use of the ``Generation 2'' (Gen-2)\footnote{The Gen-2 Canceller succeeds the narrowband Gen-1 Canceller which was integrated in the ORBIT testbed~\cite{kohli2021open}} canceller box, which houses the improved FDE canceller PCB, as shown in Figure~\ref{fig:cosmos-fde-integration}~\subref{fig:cosmos-gen2-box}, with four such boxes mounted on the corners of a 4.5$\times$3.5\thinspace{m} rectangle within a square laboratory room. Each Gen-2 canceller box also contains a circulator and antenna tuner to support the single antenna interface, and serves as the frontend to a USRP X310 with SBX-120 RF daughterboards. 

\noindent\textbf{Improved PCB Canceller.} The improved PCB's design was consolidated to include all components on a single PCB; the first revision required a daughterboard to provide the analog voltage to control the FDE path phase shifters. 




% The testbed integration has been further developed since the version presented~\cite{kohli2021open}. Henceforth known as the \textit{Generation 2 (Gen-2) Canceller} (G2C)\footnote{The G2C succeeds the Gen-1 Canceller which was integrated in the ORBIT testbed~\cite{kohli2021open}}, Figure~\ref{fig:cosmos-fde-integration} shows one \textit{Gen-2 Canceller Box} containing the G2C and accompanying components mounted at its fixed position within the testbed, where it is connected as the frontend to a USRP X310 SDR and powered by a Keysight E36312A supply. The other three G2C boxes are organized in the same fashion; the four boxes are located at the corners of a 4.5$\times$3.5\thinspace{m} rectangle within a square laboratory room.}

% \addedMK{An architecture diagram providing a high-level overview of the testbed is provided in Figure~\ref{fig:cosmos-fde-architecture}. The USRP X310 radios are connected to servers through a 10\thinspace{Gb/s} switch and the SUB-20 device in the G2C Box}

==> tex/eval_rfic.tex <==
Our RFIC canceller implementation in~\cite{Zhou_WBSIC_JSSC15} has only $2$ FDE taps and achieves an average $\SI{40}{dB}$ RF SIC across $\SI{27}{MHz}$ bandwidth. Recall that the model {\eqref{eq:rfic-tf}} (see Section~\ref{ssec:impl-rfic}) accurately captures the responses of the RFIC canceller~\cite{ghaffari2011tunable,Zhou_WBSIC_JSSC15} and can be scaled up to a larger number of FDE taps. Therefore, we numerically evaluate the performance of the RFIC canceller using the model {\eqref{eq:rfic-tf}}, and the optimized canceller configuration described in Section~\ref{ssec:algo-opt}. Throughout our evaluation, we use a \emph{real, practical} antenna interface response, $\AntTF(f_k)$, measured using a $698$-$\SI{960}{MHz}$ swivel blade antenna with a coaxial circulator with operating frequency range $860$-$\SI{960}{MHz}$ in a lab environment.

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-rfic-20mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_20mhz.eps}
}
% \hspace{-12pt}
\subfloat{
\label{fig:eval-rfic-bw-40mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_40mhz.eps}
}
\\ \vspace{-\baselineskip}
%%
% \subfloat{
% \label{fig:eval-rfic-bw-60mhz}
% \includegraphics[width=0.45\columnwidth]{./figs/sim/sim_rfic_bw_60mhz.eps}
% }
% \hspace{-12pt}
\subfloat{
\label{fig:eval-rfic-bw-80mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_80mhz.eps}
}
\vspace{-0.5\baselineskip}
\caption{TX/RX isolation of the antenna interface and with the RFIC canceller {\eqref{eq:rfic-tf}} with varying number of FDE taps, $\NumTap \in \{1,2,3,4\}$, and desired RF SIC bandwidth of $\{20,40,80\}\thinspace\SI{}{MHz}$.}
\label{fig:eval-rfic}
\vspace{-\baselineskip}
\end{figure}
%%

%%
\subsection{The Ideal Case}
To evaluate and validate the concept of FDE, we first simulate the RF SIC achieved by the RFIC canceller with varying number of FDE taps, $\NumTap \in \{1,2,3,4\}$, and desired RF SIC bandwidth of $\{20,40,80\}\thinspace\SI{}{MHz}$. We only report the RF SIC performance with up to $\NumTap=4$ FDE taps since, as we show below, this case can achieve sufficient RF SIC performance up to $\SI{80}{MHz}$ bandwidth.\footnote{We select $\{20,40,80\}\thinspace\SI{}{MHz}$ desired RF SIC bandwidth since: (i) these are the standard WiFi bandwidths, and (ii) the circulator has an operating frequency range of $\SI{100}{MHz}$.} Fig.~\ref{fig:eval-rfic} shows the TX/RX isolation (defined in Section~\ref{sec:background}) without and with the RFIC canceller, where the isolation at the antenna interface $|\AntTF(f_k)| \approx -\SI{20}{dB}$. The optimized RFIC canceller configurations are obtained by solving the optimization problem $\OptProblemIC$ with the following constraints: $\forall i$, $\ICTapAmp{i} \in [-40, -10]\thinspace\SI{}{dB}$, $\ICTapPhase{i} \in [-\pi, \pi]$, $\ICTapCF{i} \in [875, 925]\thinspace\SI{}{MHz}$, and $\ICTapQF{i} \in [1, 50]$. These constraints are practically selected and can be easily realized in an RFIC implementation.

Fig.~\ref{fig:eval-rfic} shows that (i) a larger number of FDE taps can significantly enhance the RF SIC bandwidth, and (ii) under the same desired RF SIC bandwidth, a larger number of FDE taps results in better average RF SIC performance. With only $2$ FDE taps, the RFIC canceller achieves an average $\SI{58}{dB}$ RF SIC with $\SI{20}{MHz}$ bandwidth, but this value decreases to only $\SI{47}{dB}$ with $\SI{40}{MHz}$ bandwidth. With $4$ FDE taps, the RFIC canceller achieves an average amount of more than $\SI{56}{dB}$ RF SIC for all considered RF SIC bandwidth up to $\SI{80}{MHz}$.
% Fig.~\ref{fig:theory-sim-varying-bw} also shows that the RF SIC performance does not degrade for $N=2,3$ FDE taps when the desired SIC bandwidth is increased, ilustrating that $2$ or $3$ ideal FDE taps are robust to medium SIC bandwidth requirements.
Fig.~\ref{fig:eval-rfic} also shows that in some scenarios, adding more FDE taps does not help increase the RF SIC performance. For example, an RFIC canceller with $3$ FDE taps already achieves more than $\SI{70}{dB}$ RF SIC with $\SI{20}{MHz}$ bandwidth, and adding a fourth FDE tap only introduces minimal performance improvement. Note that we constrain the center frequency of the $2^{\rm nd}$-order BPFs in {\eqref{eq:rfic-tf}} to be within a $\SI{50}{MHz}$ range, and performance improvement is expected by relaxing this constraint.


%%
\subsection{Adding Practical Quantization Constraints}
In practice, the values of $\{\ICTapAmp{i}, \ICTapPhase{i}, \ICTapCF{i}, \ICTapQF{i}\}$ can not be arbitrarily selected from a continuous range. Instead, they are often restricted to discrete values given the resolution of the corresponding hardware components. We evaluate the effect of such practical quantization constraints with the following settings. The amplitude $\ICTapAmp{i}$ has a $\SI{0.25}{dB}$ resolution within range $[-40, -10]\thinspace\SI{}{dB}$. For $\ICTapPhase{i} \in [-\pi, \pi]$, $\ICTapCF{i} \in [875, 925]\thinspace\SI{}{MHz}$, and $\ICTapQF{i} \in [1, 50]$, an $8$-bit resolution constraint is introduced, which is equivalent to $2^8=256$ discrete values spaced equally in the given range. The RFIC canceller configurations with quantization constraints are obtained by rounding the configurations returned by $\OptProblemIC$ to their closest quantized values.

Fig.~\ref{fig:eval-rfic-quantized} presents the TX/RX isolation without and with the RFIC canceller with $\NumTap \in \{1,2,3,4\}$ and $\{40, 80\}\thinspace\SI{}{MHz}$ desired RF SIC bandwidth, under practical quantization constraints. The results for $20\thinspace\SI{}{MHz}$ desired RF SIC bandwidth are similar and thus omitted here. Comparing Fig.~\ref{fig:eval-rfic-quantized} with Fig.~\ref{fig:eval-rfic} shows that adding practical quantization constraints slightly reduces the amount of RF SIC achieved across the desired bandwidth. In particular, the effect of quantized configurations is the most significant for the case with $4$ FDE taps. This is because that as more FDE taps are available, more flexibility exists due to a larger number of variables that can be controlled. As a result, the RF SIC performance becomes more sensitive to the coupling between individual FDE tap responses after quantization. However, as Fig.~\ref{fig:eval-rfic-quantized} suggests, even under practical quantization constraints, an RFIC canceller with $4$ FDE taps can achieve an average $\SI{50}{dB}$ RF SIC across up to $\SI{80}{MHz}$ desired bandwidth. In addition, by relaxing the quantization constraints (e.g., through using components with higher resolutions), performance improvement is expected.

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-rfic-quantized-bw-40mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_40mhz_quantized.eps}}
% \hspace{-10pt} \hfill
\subfloat{
\label{fig:eval-rfic-quantized-bw-80mhz}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_bw_80mhz_quantized.eps}
}
\vspace{-0.5\baselineskip}
\caption{TX/RX isolation of the antenna interface and with the RFIC canceller {\eqref{eq:rfic-tf}} with varying number of FDE taps, $\NumTap \in \{1,2,3,4\}$, and desired RF SIC bandwidth of $\{40,80\}\thinspace\SI{}{MHz}$, under practical quantization constraints}
\label{fig:eval-rfic-quantized}
\vspace{-\baselineskip}
\end{figure}
%%


%%
\subsection{Comparison with the Iterative Algorithm}
\label{ssec:eval-rfic-compare}
We now compare the RFIC canceller performance under the iterative configuration algorithm and with the optimized canceller configuration, with the same practical quantization constraints as described above. As described in Section~\ref{ssec:algo-iter}, for the iterative configuration algorithm, the selection of the cancellation frequency is unclear. Therefore, we manually find the best cancellation frequencies, $\{f_{\textrm{canc},i}\}$, such the RFIC canceller performance is optimized under the iterative configuration algorithm. Moreover, we consider only $2$ FDE taps since the performance of the iterative configuration algorithm with a larger value of $\NumTap$ performs even poorly when compared with the that with the optimized canceller configuration.

Fig.~\ref{fig:eval-rfic-iter}\subref{fig:eval-rfic-iter-detail} shows the process of the iterative configuration algorithm, where $\ICTapTF{1}(f_k)$ and $\ICTapTF{2}(f_k)$ are used to match with $\AntTF(f_k)$ and $H_{\textrm{res},1}(f_k) = \AntTF(f_k)-\ICTapTF{1}(f_k)$, respectively, at the manually-optimized cancellation frequencies $\SI{896}{MHz}$ and $\SI{904}{MHz}$ indicated by the asterisks. As Fig.~\ref{fig:eval-rfic-iter}\subref{fig:eval-rfic-iter-detail} shows, the $\SI{40}{dB}$ RF SIC bandwidth is improved from $\SI{10}{MHz}$ to $\SI{16}{MHz}$ by using a second FDE tap. However, Fig.~\ref{fig:eval-rfic-iter}\subref{fig:eval-rfic-iter-compare} shows that this approach suffers from a large performance degradation when compared with the RFIC canceller performance with the optimized canceller configuration. Therefore, the optimal canceller configuration is more beneficial, which is also used to evaluate the PCB canceller performance in Section~\ref{sec:eval-pcb}.

%%
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[]{
\label{fig:eval-rfic-iter-detail}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_iter_detail.eps}
}
% \hspace{-6pt} \hfill
\subfloat[]{
\label{fig:eval-rfic-iter-compare}
\includegraphics[width=0.4\columnwidth]{./figs/sim/sim_rfic_iter_compare.eps}
}
\vspace{-\baselineskip}
\caption{(a) TX/RX Isolation of the antenna interface and with the RFIC canceller after each iterative configuration step. (b) Comparison of TX/RX isolation performance under the iterative and optimal configurations.}
% where each FDE tap matches with the residual SI channel response from the previous iteration at a cancellation frequency indicated by the marker.
\label{fig:eval-rfic-iter}
\vspace{-\baselineskip}
\end{figure}
%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/experiments.tex <==
%%
In this section, we discuss the integration of the PCB canceller described in Section~\ref{sec:impl} with an SDR testbed. Then, we present extensive experimental evaluation of the FDE-based FD radio at the node, link, and network levels.

%%%%%
%%%%%
\subsection{Implementation and Testbed}
\label{ssec:exp-testbed}

% \subsubsection*{FDE-based FD Radio and the SDR Testbed}
\noindent\textbf{FDE-based FD radio and the SDR testbed}.
Figs.~\ref{fig:intro}\subref{fig:intro-fd-radio} and~\ref{fig:intro}\subref{fig:intro-fd-net} depict our FDE-based FD radio design (whose diagram is shown in Fig.~\ref{fig:diagram}) and the SDR testbed. A {698--960}\thinspace{MHz} swivel blade antenna and a coaxial circulator with operating frequency range {860--960}\thinspace{MHz} are used as the antenna interface. We use the NI USRP-2942 SDR with the SBX-120 daughterboard operating at {900}\thinspace{MHz} carrier frequency, which is the same as the operating frequency of the PCB canceller. As mentioned in Section~\ref{ssec:impl-pcb}, our PCB canceller design can be easily extended to other operating frequencies. The USRP has a measured noise floor of $-${85}\thinspace{dBm} at a fixed receiver gain setting.\footnote{This USRP receiver noise floor is limited by the environmental interference at around {900}\thinspace{MHz}. The USRP has a true noise floor of around $-${95}\thinspace{dBm} at the same receiver gain setting, when not connected to an antenna.}

We implemented a full OFDM-based PHY layer using NI LabVIEW on a host PC with a real-time RF bandwidth of $\BW = {20}\thinspace\textrm{MHz}$.\footnote{We consider a general OFDM-based PHY but do not consider the specific frame/packet structure defined by the standards (e.g., LTE or WiFi PHY).}
% A real-time RF bandwidth of $\BW=\SI{20}{MHz}$ is used through our experiments.
The baseband complex (IQ) samples are streamed between the USRP and the host PC through a high-speed PCI-Express interface. The OFDM symbol size is 64 samples (subcarriers) with a cyclic-prefix ratio of 0.25 (16 samples). Throughout the evaluation, $\{f_k\}_{k=1}^{K=52}$ is used to represent the center frequency of the 52 non-zero subcarriers. The OFDM PHY layer supports various modulation and coding schemes (MCSs) with constellations from BPSK to 64QAM and coding rates of 1/2, 2/3, and 3/4, resulting in a highest (HD) data rate of {54}\thinspace{Mbps}.
% Unless mentioned otherwise, we cycle through all MCSs in the experiments and record the maximal achieved data rate.
The digital SIC algorithm with a highest non-linearity order of 7 is implemented in LabVIEW to further suppress the residual SI signal after RF SIC.\footnote{The digital SIC algorithm is based on Volterra series and a least-square problem, which is similar to that presented in~\cite{bharadia2013full}. We omit the details here due to limited space.}

In total, our testbed consists of 3 FDE-based FD radios, whose performance is experimentally evaluated at the node, link, and network levels. Regular USRPs (without the PCB canceller) are also included in scenarios where additional HD users are needed.

%%
%%
% \subsubsection*{Optimized PCB Canceller Configuration}
\noindent\textbf{Optimized PCB canceller configuration}.
The optimized PCB canceller configuration scheme is implemented on the host PC and the canceller is configured by a SUB-20 controller through the USB interface. For computational efficiency, the PCB canceller response {\eqref{eq:pcb-tf-calibrated}} (which is validated in Section~\ref{sec:pcb-validation} and is independent of the environment) is pre-computed and stored.
% The detailed steps of the canceller configuration are as follows.
The canceller configuration has the following steps.
%%
\begin{enumerate}[leftmargin=*,topsep=0pt]
\item[1.]
Measure the real-time antenna interface response, $\AntTF(f_k)$, using a preamble of 2 OFDM symbols by dividing the received preamble by the known transmitted preamble in the frequency domain;
\item[2.]
Solve for an initial PCB canceller configuration using optimization {\OptProblemPCB} based on the measured $\AntTF(f_k)$ and the canceller model {\eqref{eq:pcb-tf-calibrated}} (see Section~\ref{ssec:impl-opt}). The returned configuration parameters are rounded to their closest possible values based on hardware resolutions (see Section~\ref{ssec:impl-pcb});
\item[3.]
Perform a finer-grained local search and record the optimal canceller configuration (usually around 10 iterations).
\end{enumerate}
%%
In our design, the optimized PCB canceller configuration can be obtained in less than {10}\thinspace{ms} on a regular PC with quad-core Intel i7 CPU via a non-optimized MATLAB solver. Specifically, 100 instance runs of the optimized canceller configuration scheme require an average runtime of {6.7}\thinspace{ms} with a standard deviation of {0.4}\thinspace{ms}. Assuming that the canceller needs to be configured once per second, this is less than 1\% overhead. We note that a C-based optimization solver and/or an implementation based on FPGA/look-up table can significantly improve the performance of the canceller configuration scheme and is left for future work.
% \footnote{Assuming that the canceller needs to be configured once per second, this is only a 1\% overhead. We note that a C-based optimization solver and/or an implementation based on FPGA/look-up table can significantly improve the performance of the canceller configuration and is left for future work.}

%%
%%


%%%%%
%%%%%
\subsection{Node-Level: Microbenchmarks}
\label{ssec:exp-node}

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[]{
\label{fig:exp-usrp-algo-iq}
\includegraphics[width=0.47\columnwidth]{./figs/exp/exp_usrp_algo_iq.eps}
}
\hfill
\subfloat[]{
\label{fig:exp-usrp-algo-res}
\includegraphics[width=0.47\columnwidth]{./figs/exp/exp_usrp_algo_res.eps}
}
\vspace{-0.5\baselineskip}
\caption{(a) Real and imaginary parts of the optimized PCB canceller response, $\PCBTF(f_k)$, vs. real-time SI channel measurements, $\AntTF(f_k)$, and (b) modeled and measured RX signal power after RF SIC at {10}\thinspace{dBm} TX power. An average {52}\thinspace{dB} RF SIC across {20}\thinspace{MHz} is achieved in the experiments.}
\label{fig:exp-usrp-algo}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-0.5\baselineskip}
\includegraphics[width=0.8\columnwidth]{./figs/exp/exp_usrp_sic.eps}
\vspace{-0.5\baselineskip}
\caption{Power spectrum of the received signal after SIC in the RF and digital domains with {10}\thinspace{dBm} average TX power, {20}\thinspace{MHz} bandwidth, and $-${85}\thinspace{dBm} receiver noise floor.}
\label{fig:eval-usrp-spec-20mhz}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%
% \subsubsection*{Optimized PCB Canceller Response and RF SIC}
\noindent\textbf{Optimized PCB canceller response and RF SIC}.
We set up an FDE-based FD radio running the optimized PCB canceller configuration scheme and record the canceller configuration, measured $\AntTF(f_k)$, and measured residual SI power after RF SIC. The recorded canceller configuration is then used to compute the PCB canceller response using {\eqref{eq:pcb-tf-calibrated}}.

Fig.~\ref{fig:exp-usrp-algo}\subref{fig:exp-usrp-algo-iq} shows an example of the optimized PCB canceller response, $\PCBTF(f_k)$, and the measured antenna interface response, $\AntTF(f_k)$, in real and imaginary parts (or I and Q). It can be seen that $\PCBTF(f_k)$ closely matches with $\AntTF(f_k)$ with maximum differences in amplitude and phase are only {0.5}\thinspace{dB} and {2.5}$^{\circ}$, respectively. This confirms the accuracy of the PCB canceller model and the performance of the optimized canceller configuration. Fig.~\ref{fig:exp-usrp-algo}\subref{fig:exp-usrp-algo-res} shows the modeled (computed by subtracting the modeled canceller response from the measured $\AntTF(f_k)$) and measured RX signal power after RF SIC at $+${10}\thinspace{dBm} TX power. The results show that the FDE-based FD radio achieves an average {52}\thinspace{dB} RF SIC across {20}\thinspace{MHz} bandwidth, from which {20}\thinspace{dB} is obtained from the antenna interface isolation. Similar performance is observed throughout the experimental evaluation. Note that the profile of RF SIC is similar to that presented in the sensitivity analysis of the FDE-based cancellers (see Section~\ref{sec:sensitivity}).


%%
%%
% \subsubsection*{Overall SIC}
\noindent\textbf{Overall SIC}.
We measure the overall SIC achieved by the FDE-based FD radio including the digital SIC in the same setting as described above, and the results are presented in Fig.~\ref{fig:eval-usrp-spec-20mhz}. It can be seen that the FDE-based FD radio achieves an average {95}\thinspace{dB} overall SIC across {20}\thinspace{MHz}, from which {52}\thinspace{dB} and {43}\thinspace{dB} are obtained in the RF and digital domains, respectively. Recall from Section~\ref{ssec:exp-testbed} that the USRP has noise floor of $-${85}\thinspace{dBm}, the FDE-based RF radio supports a maximal average TX power of {10}\thinspace{dBm} (where the peak TX power can go as high as {20}\thinspace{dBm}). We use TX power levels lower than or equal to {10}\thinspace{dBm} throughout the experiments, where all the SI can be canceled to below the RX noise floor.


%%
%%
\subsection{Link-Level: SNR-PRR Relationship}
\label{ssec:exp-snr-prr-relationship}
We now evaluate the relationship between link SNR and link packet reception ratio (PRR). We setup up a link with two FDE-based FD radios at a fixed distance of 5 meters with equal TX power. In order to evaluate the performance of our FD radios with the existence of the PCB canceller, we set an FD radio to operate in HD mode by turning on only its transmitter or receiver. We conduct the following experiment for each of the 12 MCSs in both FD and HD modes, with varying TX power levels. In particular, the packets are sent over the link simultaneously in FD mode or in alternating directions in HD mode (i.e., the two radios take turns and transmit to each other). In each experiment, both radios send a sequence of 50 OFDM streams, each OFDM stream contains 20 OFDM packets, and each OFDM packet is 800-Byte long.

We consider two metrics. The \emph{HD (resp.\ FD) link SNR} is measured as the ratio between the average RX signal power in both directions and the RX noise floor when both radios operate in HD (resp. FD) mode. The \emph{HD (resp.\ FD) link PRR} is computed as the fraction of packets successfully sent over the HD (resp. FD) link in each experiment. We observe from the experiments that the HD and FD link SNR and PRR values in both link directions are similar. Similar experiments and results were presented in~\cite{zhou2016basic} for HD links.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[Code rate 1/2]{
\label{fig:exp-prr-vs-snr-1-2}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_prr_vs_snr_1_2.eps}
}
\hfill
\subfloat[Code rate 3/4]{
\label{fig:exp-prr-vs-snr-3-4}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_prr_vs_snr_3_4.eps}
}
\vspace{-0.5\baselineskip}
\caption{HD and FD link packet reception ratio (PRR) with varying HD link SNR and modulation and coding schemes (MCSs).}
\label{fig:exp-prr-vs-snr}
% \vspace{-\baselineskip}
\end{figure}
%% figure ends

Fig.~\ref{fig:exp-prr-vs-snr} shows the relationship between link PRR values and HD link SNR values with varying MCSs. The results show that with sufficient link SNR values (e.g., {8}\thinspace{dB} for BPSK-1/2 and {28}\thinspace{dB} for 64QAM-3/4), the FDE-based FD radio achieves a link PRR of 100\%. With insufficient link SNR values, the average FD link PRR is 6.5\% lower than the HD link PRR across varying MCSs. This degradation is caused by the link SNR difference when the radios operate in HD or FD mode, which is described later in Section~\ref{ssec:exp-link}. Since packets are sent simultaneously in both directions on an FD link, this average PRR degradation is equivalent to an average FD link throughput gain of 1.87$\times$ under the same MCS.


%%%%%
%%%%%
\subsection{Link-Level: SNR Difference and FD Gain}
\label{ssec:exp-link}

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[LOS deployment and an FD radio in a hallway]{
\label{fig:exp-map-los}
\includegraphics[width=\columnwidth]{./figs/exp/link/exp_los_setup.pdf}
} \\
\vspace{-0.5\baselineskip}
% \hspace{6pt}
\subfloat[NLOS deployment and an FD radio in a lab environment]{
\label{fig:exp-map-nlos}
\includegraphics[width=\columnwidth]{./figs/exp/link/exp_nlos_setup.pdf}
}
\vspace{-0.5\baselineskip}
\caption{(a) Line-of-sight (LOS), and (b) non-line-of-sight (NLOS) deployments, and the measured HD link SNR values (dB).}
\label{fig:exp-map}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%
%%
% \subsubsection*{Experimental Setup}
\noindent\textbf{Experimental setup}.
To thoroughly evaluate the link level FD throughput gain achieved by our FD radio design, we conduct experiments with two FD radios with {10}\thinspace{dBm} TX power, one emulating a base station (BS) and one emulating a user. We consider both line-of-sight (LOS) and non-line-of-sight (NLOS) experiments as shown in Fig.~\ref{fig:exp-map}. In the LOS setting, the BS is placed at the end of a hallway and the user is moved away from the BS at stepsizes of 5 meters up to a distance of 40 meters. In the NLOS setting, the BS is placed in a lab environment with regular furniture and the user is placed at various locations (offices, labs, and corridors). We place the BS and the users at about the same height across all the experiments.\footnote{In this work, we emulate the BS and users without focusing on specific deployment scenarios. The impacts of different antenna heights and user densities, as mentioned in~\cite{lopez2015towards}, will be considered in future work.} The measured HD link SNR values are also included in Fig.~\ref{fig:exp-map}. Following the methodology of~\cite{bharadia2013full}, for each user location, we measure the \emph{link SNR difference}, which is defined as the absolute difference between the average HD and FD link SNR values. Throughout the experiments, link SNR values between {0--50}\thinspace{dB} are observed.

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-\baselineskip}
\subfloat[LOS Experiment]{
\label{fig:exp-link-snr-loss-los}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_los_snr_loss.eps}
}
\hfill
\subfloat[NLOS Experiment]{
\label{fig:exp-link-snr-loss-nlos}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_nlos_snr_loss.eps}
}
\vspace{-0.5\baselineskip}
\caption{Difference between HD and FD link SNR values in the (a) LOS, and (b) NLOS experiments, with {10}\thinspace{dBm} TX power and 64QAM-3/4 MCS.}
\label{fig:exp-link-snr-loss}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends

%%
%%
% \subsubsection*{Difference in HD and FD Link SNR Values}
\noindent\textbf{Difference in HD and FD link SNR values}.
Fig.~\ref{fig:exp-link-snr-loss} shows the measured link SNR difference as a function of the HD link SNR (i.e., for different user locations) in the LOS and NLOS experiments, respectively, with 64QAM-3/4 MCS. For the LOS experiments, the average link SNR difference is {0.6}\thinspace{dB} with a standard deviation of {0.2}\thinspace{dB}. For the NLOS experiments, the average link SNR difference is {0.6}\thinspace{dB} with a standard deviation of {0.3}\thinspace{dB}. The SNR difference has a higher variance in the NLOS experiments, due to the complicated environments (e.g., wooden desks and chairs, metal doors and bookshelves, etc.). In both cases, the link SNR difference is minimal and uncorrelated with user locations, showing the robustness of the FDE-based FD radio.


%%
%%
% \subsubsection*{Impact of Constellations}
\noindent\textbf{Impact of constellations}.
Fig.~\ref{fig:exp-constellation} shows the measured link SNR difference and its CDF with varying constellations and 3/4 coding rate. It can be seen that the link SNR difference has a mean of {0.6}\thinspace{dB} and a standard deviation of {0.4}\thinspace{dB}, both of which are uncorrelated with the constellations.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[]{
\label{fig:exp-constellation-snr-loss}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/snr_loss_vs_constellation_err.eps}
}
\hfill
\subfloat[]{
\label{fig:exp-constellation-tput-gain}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/snr_loss_vs_constellation_cdf.eps}
}
\vspace{-0.5\baselineskip}
\caption{Difference between HD and FD link SNR values with {10}\thinspace{dBm} TX power under varying constellations: (a) mean and standard deviation, (b) CDF.}
\label{fig:exp-constellation}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends


%%
%%
% \subsubsection*{FD Link Throughput and Gain}
\noindent\textbf{FD link throughput and gain}.
For each user location in the LOS and NLOS experiments, the HD (resp.\ FD) link throughput is measured as the highest average data rate across all MCSs achieved by the link when both nodes operate in HD (resp.\ FD) mode . The FD gain is computed as the ratio between FD and HD throughput values. Recall that the maximal HD data rate is {54}\thinspace{Mbps}, an FD link data rate of {108}\thinspace{Mbps} can be achieved with an FD link PRR of 1.

Fig.~\ref{fig:exp-link-tput} shows the average HD and FD link throughput with varying 16QAM-3/4 and 16QAM-3/4 MCSs, where each point represents the average throughput across 1,000 packets. The results show that with sufficient link SNR values (e.g., {30}\thinspace{dB} for 64QAM-3/4 MCS), the FDE-based FD radios achieve an \emph{exact} link throughput gain of 2$\times$. In these scenarios, the HD/FD link always achieves a link PRR of 1 which results in the maximum achievable HD/FD link data rate. With medium link SNR values, where the link PRR less than 1, the average FD link throughput gains across different MCSs are 1.91$\times$ and 1.85$\times$ for the LOS and NLOS experiments, respectively. We note that if higher modulation schemes (e.g., 256QAM) are considered and the corresponding link SNR values are high enough for these schemes, the HD/FD throughput can increase (compared to the values in Fig.~\ref{fig:exp-link-tput}). However, considering such schemes is not required in order to evaluate the FDE-based cancellers and the FD gain.
% We note that the HD/FD throughput will increased if higher modulation schemes are considered and the link SNR values are sufficient for the considered modulation scheme. However, such schemes are not essential to evaluate the FDE-based cancellers and FD gain.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[LOS Experiment]{
\label{fig:exp-link-tput-los}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_los_tput_3_4.eps}
}
\hfill
\subfloat[NLOS Experiment]{
\label{fig:exp-link-tput-nlos}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_nlos_tput_3_4.eps}
}
\vspace{-0.5\baselineskip}
\caption{HD and FD link throughput in the (a) LOS, and (b) NLOS experiments, with {10}\thinspace{dBm} TX power and 16QAM-3/4 and 64QAM-3/4 MCSs.}
\label{fig:exp-link-tput}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends


%%%%%
%%%%%

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[]{
\label{fig:exp-net-setup-ul-dl}
\includegraphics[width=0.31\columnwidth]{./figs/exp/net_ul_dl/exp_ul_dl_setup.pdf}
}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:exp-net-setup-two-users}
\includegraphics[width=0.31\columnwidth]{./figs/exp/net_two_users/exp_two_users_setup.pdf}
}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:exp-net-setup-three-users}
\includegraphics[width=0.31\columnwidth]{./figs/exp/net_three_users/exp_three_users_setup.pdf}
}
\vspace{-0.5\baselineskip}
\caption{An example experimental setup for: (a) the UL-DL networks with varying $\SNRUL$ and $\SNRDL$, (b) heterogeneous 3-node network with one FD BS and 2 FD users, and (c) heterogeneous 4-node networks with one FD BS, 2 FD users, and one HD user.}
\label{fig:exp-net-setup}
% \vspace{-0.5\baselineskip}
\end{figure}
%% figure ends

\subsection{Network-Level FD Gain}
\label{ssec:exp-net}
We now experimentally evaluate the network-level throughput gain introduced by FD-capable BS and users. The users can significantly benefit from the FDE-based FD radio suitable for hand-held devices. We compare experimental results to the analysis (e.g.,~\cite{marasevic2017resource}) and demonstrate practical FD gain in different network settings. Specifically, we consider two types of networks as depicted in Fig.~\ref{fig:exp-net-setup}: (i) \emph{UL-DL networks} with one FD BS and two HD users with inter-user interference (IUI), and (ii) \emph{heterogeneous HD-FD networks} with HD and FD users. Due to software challenge with implementing a real-time MAC layer using a USRP, we apply a TDMA setting where each (HD or FD) user takes turn to be activated for the same period of time.


%%%%%
%%%%%
\subsubsection{UL-DL Networks with IUI}
\label{sssec:exp-net-ul-dl}
We first consider UL-DL networks consisting of one FD BS and two HD users (indexed 1 and 2). Without loss of generality, in this setting, user 1 transmits on the UL to the BS, and the BS transmits to user 2 on the DL (see Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-ul-dl}).

%%
%%
\noindent\textbf{Analytical FD gain}.
We use Shannon's capacity formula $\DataRate{}(\SNR{}) = \BW \cdot \log_{2}(1+\SNR{})$ to compute the \emph{analytical throughput} of a link under bandwidth $\BW$ and (HD) link SNR $\SNR{}$. If the BS is only HD-capable, the network throughput in a UL-DL network when the UL and DL share the channel in a TDMA manner with equal fraction of time is given by
%%
\begin{align}
\label{eq:net-ul-dl-tput-hd}
\DataRate{\textrm{UL-DL}}^{\textrm{HD}} = \frac{\BW}{2}\cdot\log_{2}\left(1+\SNRUL\right) + \frac{\BW}{2}\cdot\log_{2}\left(1+\SNRDL\right),
\end{align}
%%
where $\SNRUL$ and $\SNRDL$ are the UL and DL SNRs, respectively. If the BS is FD-capable, the UL and DL can be simultaneously activated with an analytical network throughput of
%%
\begin{align}
\label{eq:net-ul-dl-tput-fd}
% \hspace*{-12pt}
\DataRate{\textrm{UL-DL}}^{\textrm{FD}} = \BW\cdot\log_{2}(1+\frac{\SNRUL}{1+\XINR}) + \BW\cdot\log_{2}(1+\frac{\SNRDL}{1+\IUI}),
\end{align}
%%
where: (i) $(\frac{\SNRDL}{1+\IUI})$ is the signal-to-interference-plus-noise ratio (SINR) at the DL HD user, and (ii) $\XINR$ is the residual self-interference-to-noise ratio (XINR) at the FD BS. We set $\XINR=1$ when computing the analytical throughput. Namely, the residual SI power is no higher than the RX noise floor (which can be achieved by the FDE-based FD radio, see Section~\ref{ssec:exp-node}). The \emph{analytical FD gain} is then defined as the ratio $(\DataRate{\textrm{UL-DL}}^{\textrm{FD}}/\DataRate{\textrm{UL-DL}}^{\textrm{HD}})$. Note that the FD gain depends on the coupling between $\SNRUL$, $\SNRDL$, and $\IUI$, which depend on the BS/user locations, their TX power levels, etc. 

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[$\SNRUL={10}\thinspace\textrm{dB}$]{
\label{fig::exp-net-ul-dl-gain-10db}
\includegraphics[height=1.35in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_10db.eps}
}
\subfloat[$\SNRUL={15}\thinspace\textrm{dB}$]{
\label{fig::exp-net-ul-dl-gain-15db}
\includegraphics[height=1.35in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_15db.eps}
}
\subfloat[$\SNRUL={20}\thinspace\textrm{dB}$]{
\label{fig::exp-net-ul-dl-gain-20db}
\includegraphics[height=1.35in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_20db.eps}
}
\vspace{-0.5\baselineskip}
\caption{Analytical (colored surface) and experimental (filled circles) network throughput gain for UL-DL networks consisting of one FD BS and two HD users with varying UL and DL SNR values, and inter-user interference (IUI) levels: (a) $\SNRUL={10}\thinspace\textrm{dB}$, (b) $\SNRUL={15}\thinspace\textrm{dB}$, and (c) $\SNRUL={20}\thinspace\textrm{dB}$. The baseline is the network throughput when the BS is HD.}
\label{fig:exp-net-ul-dl-gain}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%% table begins
\begin{table}[!t]
\caption{Average FD Gain in UL-DL Networks with IUI.}
\label{table:exp-net-ul-dl-gain}
\vspace{-\baselineskip}
\footnotesize
\begin{center}
% \begin{tabular}{| p{0.1\columnwidth} | p{0.2\columnwidth} | p{0.1\columnwidth} | p{0.2\columnwidth} |}
\begin{tabular}{|c|c|c|}
\hline
UL SNR, $\SNRUL$ & Analytical FD Gain & Experimental FD Gain \\
\hline
{10}\thinspace{dB} & 1.30$\times$ & 1.25$\times$ \\
\hline
{15}\thinspace{dB} & 1.23$\times$ & 1.16$\times$ \\
\hline
{20}\thinspace{dB} & 1.22$\times$ & 1.14$\times$ \\
\hline
\end{tabular}
\end{center}
\vspace{-2\baselineskip}
\end{table}
%% table ends

%%
%%
\noindent\textbf{Experimental FD gain}.
The experimental setup is depicted in Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-ul-dl}, where the TX power levels of the BS and user 1 are set to be {10}\thinspace{dBm} and $-${10}\thinspace{dBm}, respectively. We fix the location of the BS and consider different UL SNR values of $\SNRUL = 10/15/20\thinspace\textrm{dB}$ by placing user 1 at three different locations. For each value of $\SNRUL$, user 2 is placed at 10 different locations, resulting in varying $\SNRDL$ and $\IUI$ values.

Fig.~\ref{fig:exp-net-ul-dl-gain} shows the analytical (colored surface) and experimental (filled circles) FD gain, where the analytical gain is extracted using {\eqref{eq:net-ul-dl-tput-hd}} and {\eqref{eq:net-ul-dl-tput-fd}}, and the experimental gain is computed using the measured UL and DL throughput. It can be seen that smaller values of $\SNRUL$ and lower ratios between $\SNRDL$ and $\IUI$ lead to higher throughput gains in both analysis and experiments. The average analytical and experimental FD gains are summarized in Table~\ref{table:exp-net-ul-dl-gain}. Due to practical reasons such as the link SNR difference and its impact on link PRR (see Section~\ref{ssec:exp-snr-prr-relationship}), the experimental FD gain is within 93\% of the analytical FD gain. The results confirm the analysis in~\cite{marasevic2017resource} and demonstrate the practical FD gain achieved in wideband UL-DL networks without any changes in the current network stack (i.e., only bringing FD capability to the BS). Moreover, performance improvements are expected through advanced power control and scheduling schemes.


%%%%%
%%%%%
\subsubsection{Heterogeneous 3-Node Networks}
\label{sssec:exp-net-two-users}

We consider heterogeneous HD-FD networks with 3 nodes: one FD BS and two users that can operate in either HD or FD mode (see an example experimental setup in Figs.~\ref{fig:intro}\subref{fig:intro-fd-net} and~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-two-users}). All 3 nodes have the same {0}\thinspace{dBm} TX power so that each user has symmetric UL and DL SNR values of $\SNR{i}$ ($i=1,2$).
% \footnote{To better illustrate the results, we consider symmetric UL and DL SNR values while the link SNRs are different across users. The case with asymmetric UL and DL SNR values can also be evaluated.}
We place user 1 at 5 different locations and place user 2 at 10 different locations for each location of user 1, resulting in a total number of 50 pairs of $(\SNR{1},\SNR{2})$.


%%
%%
\noindent\textbf{Analytical FD gain}.
We set the users to share the channel in a TDMA manner. The analytical network throughput in a 3-node network when zero, one, and two users are FD-capable is respectively given by
%%
\begin{align}
& \hspace*{-10pt}
\DataRate{}^{\textrm{HD}} = \frac{\BW}{2}\cdot\log_{2}\left(1+\SNR{1}\right) + \frac{\BW}{2}\cdot\log_{2}\left(1+\SNR{2}\right), \label{eq:net-two-users-tput-hd} \\
& \hspace*{-10pt}
\DataRate{\textrm{User}~i~\textrm{FD}}^{\textrm{HD-FD}} = \BW\cdot\log_{2}(1+\frac{\SNR{i}}{1+\XINR}) + \frac{\BW}{2}\cdot\log_{2}(1+\SNR{\overline{i}}),\ \label{eq:net-two-users-tput-hd-fd} \\
& \hspace*{-10pt}
\DataRate{}^{\textrm{FD}} = \BW\log_{2}\cdot(1+\frac{\SNR{1}}{1+\XINR}) + \BW\log_{2}\cdot(1+\frac{\SNR{2}}{1+\XINR}), \label{eq:net-two-users-tput-fd}
\end{align}
%%
where $\XINR=1$ is set (similar to Section~\ref{sssec:exp-net-ul-dl}). We consider both FD gains of $(\DataRate{\textrm{User}~i~\textrm{FD}}^{\textrm{HD-FD}}/\DataRate{}^{\textrm{HD}})$ (i.e., user $i$ is FD and user $\overline{i} \ne i$ is HD), and $(\DataRate{}^{\textrm{FD}}/\DataRate{}^{\textrm{HD}})$ (i.e., both users are FD). 


%%
%%
\noindent\textbf{Experimental FD gain}.
For each pair of $(\SNR{1},\SNR{2})$, experimental FD gain is measured in three cases: (i) only user 1 is FD, (ii) only user 2 is FD, and (iii) both users are FD. Fig.~\ref{fig:exp-net-two-users} shows the analytical (colored surface) and experimental (filled circles) FD gain for each case. We exclude the results with $\SNR{i}<{3}\thinspace\textrm{dB}$ since the packets cannot be decoded, resulting in a throughput of zero (see Fig.~\ref{fig:exp-prr-vs-snr}).

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat[Only user 1 FD]{
\label{fig:exp-net-two-users-user1-fd}
\includegraphics[height=1.35in]{./figs/exp/net_two_users/exp_user1_fd_gain_experimental.eps}
}
\subfloat[Only user 2 FD]{
\label{fig:exp-net-two-users-user2-fd}
\includegraphics[height=1.35in]{./figs/exp/net_two_users/exp_user2_fd_gain_experimental.eps}
}
\subfloat[Both users FD]{
\label{fig:exp-net-two-users-both-fd}
\includegraphics[height=1.35in]{./figs/exp/net_two_users/exp_both_fd_gain_experimental.eps}
}
\vspace{-0.5\baselineskip}
\caption{Analytical (colored surface) and experimental (filled circles) network throughput gain for 3-node networks consisting of one FD BS and two users with varying link SNR values: (a) only user 1 is FD, (b) only user 2 is FD, and (c) both users are FD. The baseline is the network throughput when both users are HD.}
\label{fig:exp-net-two-users}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends

% %% figure begins
% \begin{figure}[!t]
% \centering
% % \vspace{-\baselineskip}
% \includegraphics[width=0.8\columnwidth]{./figs/exp/net_two_users/exp_two_users_fairness.eps}
% \vspace{-0.5\baselineskip}
% \caption{Measured Jain's fairness index (JFI) in 3-node networks when both users are HD and FD with varying $(\SNR{1},\SNR{2})$.}
% \label{fig:exp-net-two-users-fairness}
% \vspace{-\baselineskip}
% \end{figure}
% %% figure ends

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-\baselineskip}
\subfloat[User 1 $\SNR{1}={15}\thinspace\textrm{dB}$]{
\label{fig:exp-net-two-users-fairness-snr1-15db}
\includegraphics[height=1.5in]{./figs/exp/net_two_users/exp_two_users_fairness_snr1_15db.eps}
}
\hspace{-10pt}
\subfloat[User 1 $\SNR{1}={20}\thinspace\textrm{dB}$]{
\label{fig:exp-net-two-users-fairness-snr1-20db}
\includegraphics[height=1.5in]{./figs/exp/net_two_users/exp_two_users_fairness_snr1_20db.eps}
}
\hspace{-10pt}
\subfloat[User 1 $\SNR{1}={25}\thinspace\textrm{dB}$]{
\label{fig:exp-net-two-users-fairness-snr1-25db}
\includegraphics[height=1.5in]{./figs/exp/net_two_users/exp_two_users_fairness_snr1_25db.eps}
}
\vspace{-0.5\baselineskip}
\caption{Measured Jain's fairness index (JFI) in 3-node networks where both users are HD, User 1 is FD, and both users are FD, with varying $(\SNR{1},\SNR{2})$.}
\label{fig:exp-net-two-users-fairness}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends

The results show that with small link SNR values, the experimental FD gain is lower than the analytical value due to the inability to decode the packets. On the other hand, with sufficient link SNR values, the experimental FD gain exceeds the analytical FD gain. This is because setting $\XINR=1$ in {\eqref{eq:net-two-users-tput-hd-fd}} and {\eqref{eq:net-two-users-tput-fd}} results in a {3}\thinspace{dB} SNR loss in the analytical FD link SNR, and thereby in a lower throughput. However, in practice, the packets can be decoded with a link PRR of 1 with sufficient link SNRs, resulting in exact twice number of packets being successfully sent over an FD link. Moreover, the FD gain is more significant when enabling FD capability for users with higher link SNR values.

% 0.047/0.036/0.055
Another important metric we consider is the fairness between users, which is measured by the Jain's fairness index (JFI). In the considered 3-node networks, the JFI ranges between 0.5 (worst case) and 1 (best case). Fig.~\ref{fig:exp-net-two-users-fairness} shows the measured JFI when both users operate in HD mode, user 1 operates in FD mode, and both users operate in FD mode. with varying user SNR values $(\SNR{1},\SNR{2})$.
The results show that introducing FD capability to both users results in an average degradation in the network JFI of only 5.6/4.4/7.4\% for $\SNR{1} = {15/20/25}\thinspace\textrm{dB}$ (averaged across varying $\SNR{2}$), while the average network FD gains are 1.32/1.58/1.73$\times$ (see Fig.~\ref{fig:exp-net-two-users}), respectively. In addition, the JFI increases with more balanced user SNR values, which is as expected. For example, under the same value of $\SNR{1}$, increased value of $\SNR{2}$ (with $\SNR{2}<\SNR{1}$) leads to improved JFI, whose value approaches to 1 as $\SNR{2}$ approaches $\SNR{1}$.
% Moreover, unbalanced $\SNR{1}$ and $\SNR{2}$ can result in even more degraded fairness performance in the case when both users have different capabilities (i.e., user 1 is FD-capable while user 2 is HD-capable).
% Another important metric we consider is the fairness between users, which is measured by the Jain's fairness index (JFI). In the considered 3-node networks, the JFI ranges between 1/2 (worst case) and 1 (best case). Fig.~\ref{fig:exp-net-two-users-fairness} shows the measured JFI when both users operate in HD or FD mode. The results show that introducing FD capability results in an average degradation in the network JFI of only $5.6\%/4.4\%/7.4\%$ for $\SNR{1} = 15/20/25\thinspace\SI{}{dB}$, while the average network FD gains are $1.32\times$/$1.58\times$/$1.73\times$, respectively. In addition, the JFI increases with higher and more balanced user SNR values, which is as expected.


%%%%%
%%%%%
\subsubsection{Heterogeneous 4-Node Networks}
\label{sssec:exp-net-three-users}

We experimentally study 4-node networks consisting of an FD BS and three users with {10}\thinspace{dBm}d TX power (see an example experimental setup in Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-three-users}).
% This is limited by the fact that only three FDE PCB cancellers are fabricated, which support one FD BS and at most two FD users.
The experimental setup is similar to that described in Section~\ref{sssec:exp-net-two-users}. 100 experiments are conducts where the 3 users are placed at different locations with different user SNR values. For each experiment, the network throughput is measured in three cases where: (i) zero, (ii) one, and (iii) two users are FD-capable.

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-\baselineskip}
\includegraphics[width=0.85\columnwidth]{./figs/exp/net_three_users/exp_three_users_gain_experimental.eps}
\vspace{-0.5\baselineskip}
\caption{CDF of the experimental network throughput in 4-node networks when zero, one, or two users are FD-capable.}
\label{fig:exp-net-three-users}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-\baselineskip}
\includegraphics[width=0.85\columnwidth]{./figs/exp/net_three_users/exp_three_users_fairness_experimental.eps}
\vspace{-0.5\baselineskip}
\caption{CDF of the measured Jain's fairness index (JFI) in 4-node networks when zero, one, or two users are FD-capable.}
\label{fig:exp-net-three-users-fairness}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-\baselineskip}
\includegraphics[width=0.85\columnwidth]{./figs/exp/net_three_users/exp_three_users_analysis_vs_experimental.eps}
\vspace{-0.5\baselineskip}
\caption{CDF of the analytical and experimental network throughput gains in 4-node networks when one or two users are FD-capable.}
\label{fig:exp-net-three-users-analysis-vs-exp}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

Fig.~\ref{fig:exp-net-three-users} shows the CDF of the network throughput of the three cases, where the measured link SNR varies between {5--45}\thinspace{dB}.Overall, the median network throughput is increased by 1.25/1.52$\times$ when one/two FD users become FD-capable.
%
Fig.~\ref{fig:exp-net-three-users-fairness} plots the CDF of the corresponding JFI, where although introducing FD-capable users results in lower values of the experimental JFI, the median JFI values degrade by only 0.06 and 0.10 with one and two FD users, respectively. Moreover, Fig.~\ref{fig:exp-net-three-users-analysis-vs-exp} shows the CDF of both the analytical and experimental network throughput gains in 4-node networks when one or two users are FD-capable. In particular, the median analytical and experimental network throughput gains have a difference of only 4\% and 3\% when one and two users are FD-capable.
% Overall, median network FD gains of 1.25$\times$ and 1.52$\times$ are achieved in cases with one and two FD users, respectively.
% These trends and the results show that in a real-world environment, the total network throughput increases as more users become FD-capable, and the improvement is more significant with higher user SNR values. Note that we only apply a TDMA scheme and a more advanced MAC layer (e.g.,~\cite{kim2013janus}) has the potential to improve the FD gain.
These trends and results show that in a real-world environment, the total network throughput increases as more users become FD-capable, and the improvement is more significant with higher user SNR values. Note that we only apply a TDMA scheme and a more advanced MAC layer (e.g.,~\cite{kim2013janus, chen2018hybrid}) has the potential to improve the FD gain and fairness performance.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:

==> tex/experiments_20180807.tex <==
%%
In this section, we discuss the integration of the PCB canceller described in Section~\ref{sec:impl} with an SDR testbed. Then, we present extensive experimental evaluation of the FDE-based FD radio at the node, link, and network levels.

%%%%%
%%%%%
\subsection{Implementation and Testbed}
\label{ssec:exp-testbed}

\noindent\textbf{FDE-based FD Radio and the SDR Testbed}.
Figs.~\ref{fig:intro}\subref{fig:intro-fd-radio} and~\ref{fig:intro}\subref{fig:intro-fd-net} depict our FDE-based FD radio design and the SDR testbed. A $698$--$\SI{960}{MHz}$ swivel blade antenna and a coaxial circulator with operating frequency range $860$--$\SI{960}{MHz}$ are used as the antenna interface. We use the NI USRP-2942 SDR with carrier frequency at $\SI{900}{MHz}$, which is the same as the operating frequency of the antenna interface and the PCB canceller with 2 FDE taps.\footnote{As mentioned in Section~\ref{ssec:impl-pcb}, our PCB canceller design can be easily extended to other operating frequencies.} The USRP has a measured noise floor of $-\SI{85}{dBm}$ at a fixed receiver gain setting.\footnote{This USRP receiver noise floor is limited by the environmental interference at around $\SI{900}{MHz}$ frequency. The USRP has a true noise floor of around $-\SI{95}{dBm}$ at the same receiver gain setting, when not connected to an antenna.}

We implemented a full OFDM-based PHY layer using NI LabVIEW on a host PC. A real-time RF bandwidth of $\BW=\SI{20}{MHz}$ is used through our experiments. The baseband complex (IQ) samples are streamed between the USRP and the host PC through a high-speed PCI-Express interface. The OFDM symbol size is 64 samples (subcarriers) with a cyclic-prefix ratio of 0.25 (16 samples). Throughout the evaluation, $\{f_k\}_{k=1}^{K=52}$ is used to represent the center frequency of the 52 non-zero subcarriers. The OFDM PHY layer supports various modulation and coding schemes (MCSs) with constellations from BPSK to 64QAM and coding rates of 1/2, 2/3, and 3/4, resulting in a highest (HD) data rate of $\SI{54}{Mbps}$.
% Unless mentioned otherwise, we cycle through all MCSs in the experiments and record the maximal achieved data rate.
The digital SIC algorithm with a highest non-linearity order of 7 is also implemented in LabVIEW to further suppress the residual SI signal after RF SIC.\footnote{The digital SIC algorithm is based on Volterra series and a least-square problem, which is similar to that presented in~\cite{bharadia2013full}. We omit the details here due to limited space.}

In total, our testbed consists of 3 FDE-based FD radios, whose performance is experimentally evaluated at the node, link, and network levels. Regular USRPs (without the PCB canceller) are also included in scenarios where additional HD users are needed.

%%
%%
\noindent\textbf{Optimized PCB Canceller Configuration}.
We implement the optimized PCB canceller configuration scheme on the host PC and the canceller is configured by a SUB-20 controller through the USB interface. To achieve computational efficiency, the PCB canceller response {\eqref{eq:pcb-tf-calibrated}} (which is independent of the environment) is pre-computed and stored. The detailed steps of the canceller configuration are as follows.
%%
\begin{enumerate}[topsep=0pt,itemsep=-3pt,leftmargin=*]
\item[1.]
Measure the real-time antenna interface response, $\AntTF(f_k)$, using a preamble (2 OFDM symbols) by dividing the received preamble by the known transmitted preamble in the frequency domain;
\item[2.]
Solve for an initial PCB canceller configuration using optimization {\OptProblemPCB} based on the measured $\AntTF(f_k)$ and the canceller model {\eqref{eq:pcb-tf-calibrated}} (see Section~\ref{ssec:impl-opt}). The returned configuration parameters are rounded to their closest possible values based on hardware resolutions (see Section~\ref{ssec:impl-pcb});
\item[3.]
Perform a finer-grained local search and record the optimal canceller configuration (usually \texttt{\char`\~}10 iterations).
\end{enumerate}
%%
In our design, the optimized PCB canceller configuration can be obtained in less than $\SI{10}{ms}$ on a regular PC with quad-core Intel i7 CPU via a non-optimized MATLAB solver.\footnote{Assuming that the canceller needs to be configured once per second, this is only a $1\%$ overhead. We note that an FPGA-based implementation can significantly improve the performance of the canceller configuration scheme and is left for future work.}

%%
%%


%%%%%
%%%%%
\subsection{Node-Level: Microbenchmarks}
\label{ssec:exp-node}

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[]{
\label{fig:exp-usrp-algo-iq}
\includegraphics[width=0.47\columnwidth]{./figs/exp/exp_usrp_algo_iq.eps}
}
\hfill
\subfloat[]{
\label{fig:exp-usrp-algo-res}
\includegraphics[width=0.47\columnwidth]{./figs/exp/exp_usrp_algo_res.eps}
}
\vspace{-0.5\baselineskip}
\caption{(a) Real and imaginary parts of the optimized PCB canceller response, $\PCBTF(f_k)$, vs. real-time SI channel measurements, $\AntTF(f_k)$, and (b) modeled and measured RX signal power after RF SIC at $\SI{10}{dBm}$ TX power. An average $\SI{52}{dB}$ RF SIC across $\SI{20}{MHz}$ is achieved in the experiments.}
\label{fig:exp-usrp-algo}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%
\noindent\textbf{Optimized PCB Canceller Response and RF SIC}.
We set up an FDE-based FD radio running the optimized PCB canceller configuration scheme and record the canceller configuration, measured $\AntTF(f_k)$, and measured residual SI power after RF SIC. The recorded canceller configuration is then used to compute the PCB canceller response using {\eqref{eq:pcb-tf-calibrated}}.

Fig.~\ref{fig:exp-usrp-algo}\subref{fig:exp-usrp-algo-iq} shows an example of the optimized PCB canceller response, $\PCBTF(f_k)$, and the measured antenna interface response, $\AntTF(f_k)$, in real and imaginary parts (or I and Q). It can be seen that $\PCBTF(f_k)$ closely matches with $\AntTF(f_k)$ with maximal amplitude and phase differences of only $\SI{0.5}{dB}$ and $\SI{2.5}{\degree}$, respectively. This confirms the accuracy of the PCB canceller model and the performance of the optimized canceller configuration. Fig.~\ref{fig:exp-usrp-algo}\subref{fig:exp-usrp-algo-res} shows the modeled (computed by subtracting the modeled canceller response from the measured $\AntTF(f_k)$) and measured RX signal power after RF SIC at $\SI{10}{dBm}$ TX power. The results show that the FDE-based FD radio achieves an average $\SI{52}{dB}$ RF SIC across $\SI{20}{MHz}$ bandwidth, from which $\SI{20}{dB}$ is obtained from the antenna interface isolation. Similar performance is observed in various experiments throughout the experimental evaluation.
% Note that the profile of RF SIC is similar to that presented in the sensitivity analysis of the FDE-based cancellers (see Section~\ref{sec:sensitivity}).

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-.5\baselineskip}
\includegraphics[width=0.7\columnwidth]{./figs/exp/exp_usrp_sic.eps}
\vspace{-0.5\baselineskip}
\caption{Power spectrum of the received signal after SIC in the RF and digital domains with $\SI{10}{dBm}$ average TX power, $\SI{20}{MHz}$ bandwidth, and $-\SI{85}{dBm}$ receiver noise floor.}
\label{fig:eval-usrp-spec-20mhz}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%
%%
\noindent\textbf{Overall SIC}.
We measure the overall SIC achieved by the FDE-based FD radio including the digital SIC in the same setting as described above, and the results are presented in Fig.~\ref{fig:eval-usrp-spec-20mhz}. It can be seen that the FDE-based FD radio achieves an average $\SI{95}{dB}$ overall SIC across $\SI{20}{MHz}$, from which $\SI{52}{dB}$ and $\SI{43}{dB}$ are obtained in the RF and digital domains, respectively. Recall from Section~\ref{ssec:exp-testbed} that the USRP has noise floor of $\SI{-85}{dBm}$, the FDE-based RF radio supports a maximal average TX power of $\SI{10}{dBm}$ (where the peak TX power can go as high as $\SI{20}{dBm}$). We use TX power levels lower than or equal to $\SI{10}{dBm}$ throughout the experiments, where all the SI can be canceled to below the RX noise floor.


%%
%%
\subsection{Link-Level: SNR-PRR Relationship}
\label{ssec:exp-snr-prr-relationship}
We now evaluate the relationship between link SNR and link packet reception ratio (PRR). We setup up a link with two FDE-based FD radios at a fixed distance of 5 meters with equal TX power. We set an FD radio to operate in HD mode by turning on only its transmitter or receiver, since we would like to evaluate it performance with the existence of the PCB canceller. The following experiments are conducted for all possible MCSs and varying TX power level of the radios. In each experiment, both FD radios send a sequence of 50 OFDM streams in both HD and FD modes, each containing 20 OFDM packets with length 800 Bytes. The packets are sent over the link simultaneously in FD mode and in alternating directions in HD mode (i.e., the two radios take turns and transmit to each other).

We consider two metrics. The \emph{HD (resp.\ FD) link SNR} is measured as the ratio between the average RX signal power in both directions and the RX noise floor when both radios operate in HD (resp. FD) mode. The \emph{HD (resp.\ FD) link PRR} is computed as the fraction of packets successfully sent over the HD (resp. FD) link in each experiment. We observe from the experiments that the HD and FD link SNR and PRR values in both link directions are similar. Similar experiments and results were presented in~\cite{zhou2016basic} for HD links.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[Code rate 1/2]{
\label{fig:exp-prr-vs-snr-1-2}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_prr_vs_snr_1_2.eps}
}
\hfill
\subfloat[Code rate 3/4]{
\label{fig:exp-prr-vs-snr-3-4}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_prr_vs_snr_3_4.eps}
}
\vspace{-0.5\baselineskip}
\caption{HD and FD link packet reception ratio (PRR) with varying HD link SNR and modulation and coding schemes (MCSs).}
\label{fig:exp-prr-vs-snr}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

Fig.~\ref{fig:exp-prr-vs-snr} shows the relationship between link PRR values and HD link SNR values with varying MCSs. The results show that with sufficient link SNR values (e.g., $\SI{8}{dB}$ for BPSK-1/2 and $\SI{28}{dB}$ for 64QAM-3/4), the FDE-based FD radio achieves a link PRR of $100\%$. With insufficient link SNR values, the average FD link PRR is $6.5\%$ lower than the HD link PRR across varying MCSs. This degradation is caused by the link SNR difference when the radios operate in HD or FD mode, which is described later in Section~\ref{ssec:exp-link}. Since packets are sent simultaneously in both directions on an FD link, this average PRR degradation is equivalent to an average FD link throughput gain of $1.87\times$ under the same MCS.


%%%%%
%%%%%
\subsection{Link-Level: SNR Difference and FD Gain}
\label{ssec:exp-link}

%% figure begins
\begin{figure}[!t]
\centering
% \vspace{-0.5\baselineskip}
\subfloat[LOS deployment and an FD radio in a hallway]{
\label{fig:exp-map-los}
\includegraphics[width=1\columnwidth]{./figs/exp/link/exp_los_setup.pdf}
} \\
\vspace{-0.5\baselineskip}
% \hspace{6pt}
\subfloat[NLOS deployment and an FD radio in a lab environment]{
\label{fig:exp-map-nlos}
\includegraphics[width=1\columnwidth]{./figs/exp/link/exp_nlos_setup.pdf}
}
\vspace{-0.5\baselineskip}
\caption{(a) Line-of-sight (LOS), and (b) non-line-of-sight (NLOS) deployments, and the measured HD link SNR values (dB).}
\label{fig:exp-map}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%
%%
\noindent\textbf{Experimental Setup}.
To thoroughly evaluate the link level FD throughput gain achieved by our FD radio design, we conduct experiments with two FD radios with $\SI{10}{dBm}$ TX power, one emulating a base station (BS) and one emulating a user. We consider both line-of-sight (LOS) and non-line-of-sight (NLOS) experiments as shown in Fig.~\ref{fig:exp-map}. In the LOS setting, the BS is placed at the end of a hallway and the user is moved away from the BS at stepsizes of 5 meters up to a distance of 40 meters. In the NLOS setting, the BS is placed in a lab environment with regular furniture and the user is placed at various locations (offices, labs, and corridors). The measured HD link SNR values are also included in Fig.~\ref{fig:exp-map}. Following the methodology of~\cite{bharadia2013full}, for each user location, we measure the \emph{link SNR difference}, which is defined as the absolute difference between the average HD and FD link SNR values. Throughout the experiments, link SNR values between $0$ -- $\SI{50}{dB}$ are observed.


%%
%%
\noindent\textbf{Difference in HD and FD Link SNR Values}.
Fig.~\ref{fig:exp-link-snr-loss} shows the measured link SNR difference as a function of the HD link SNR (i.e., for different user locations) in the LOS and NLOS experiments, respectively, with 64QAM-3/4 MCS. For the LOS experiments, the average link SNR difference is $\SI{0.6}{dB}$ with a standard deviation of $\SI{0.16}{dB}$. For the NLOS experiments, the average link SNR difference is $\SI{0.63}{dB}$ with a standard deviation of $\SI{0.31}{dB}$. The SNR difference has a higher variance in the NLOS experiments, due to the complicated environments (e.g., wooden desks and chairs, metal doors and bookshelves, etc.). In both cases, the link SNR difference is minimal and uncorrelated with user locations, showing the robustness of the FDE-based FD radio.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[LOS Experiment]{
\label{fig:exp-link-snr-loss-los}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_los_snr_loss.eps}
}
\hfill
\subfloat[NLOS Experiment]{
\label{fig:exp-link-snr-loss-nlos}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_nlos_snr_loss.eps}
}
\vspace{-0.5\baselineskip}
\caption{Difference between HD and FD link SNR values in the (a) LOS, and (b) NLOS experiments, with $\SI{10}{dBm}$ TX power and 64QAM-3/4 MCS.}
\label{fig:exp-link-snr-loss}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%
%%
\noindent\textbf{Impact of Constellations}.
Fig.~\ref{fig:exp-constellation} shows the measured link SNR difference and its CDF with varying constellations and 3/4 coding rate. It can be seen that the link SNR difference has a mean of $\SI{0.58}{dB}$ and a standard deviation of $\SI{0.4}{dB}$, both of which are uncorrelated with the constellations.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[]{
\label{fig:exp-constellation-snr-loss}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/snr_loss_vs_constellation_err.eps}
}
\hfill
\subfloat[]{
\label{fig:exp-constellation-tput-gain}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/snr_loss_vs_constellation_cdf.eps}
}
\vspace{-0.5\baselineskip}
\caption{Difference between HD and FD link SNR values with $\SI{10}{dBm}$ TX power under varying constellations: (a) mean and standard deviation, and (b) CDF.}
\label{fig:exp-constellation}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%
%%
\noindent\textbf{FD Link Throughput and Gain}.
For each user location in the LOS and NLOS experiments, the HD (resp.\ FD) link throughput is measured as the highest average data rate across all MCSs achieved by the link when both nodes operate in HD (resp.\ FD) mode . The FD gain is computed as the ratio between FD and HD throughput values. Recall that the maximal HD data rate is $\SI{54}{Mbps}$, an FD link data rate of $\SI{108}{Mbps}$ can be achieved with an FD link PRR of 1.

Fig.~\ref{fig:exp-link-tput} shows the average HD and FD link throughput with varying 16QAM-3/4 and 16QAM-3/4 MCSs, where each point represents the average throughput across 1,000 packets. The results show that with sufficient link SNR (e.g., $\SI{30}{dB}$ for 64QAM-3/4 MCS), the FDE-based FD radios achieve an \emph{exact} link throughput gain of $2\times$ with an HD/FD link PRR of 1. Namely, in cases in which the data rate is limited by the MCS, enabling FD communication results in an \emph{exact} throughput gain of $2\times$. With medium link SNR values, where the link PRR less than 1, the average FD link throughput gains across different MCSs are $1.91\times$ and $1.85\times$ for the LOS and NLOS experiments, respectively.


%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[LOS Experiment]{
\label{fig:exp-link-tput-los}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_los_tput_3_4.eps}
}
\hfill
\subfloat[NLOS Experiment]{
\label{fig:exp-link-tput-nlos}
\includegraphics[width=0.47\columnwidth]{./figs/exp/link/exp_nlos_tput_3_4.eps}
}
\vspace{-0.5\baselineskip}
\caption{HD and FD link throughput in the (a) LOS, and (b) NLOS experiments, with $\SI{10}{dBm}$ TX power and 16QAM-3/4 and 64QAM-3/4 MCSs.}
\label{fig:exp-link-tput}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%%%%
%%%%%
\subsection{Network-Level FD Gain}
\label{ssec:exp-net}
We now experimentally evaluate the network-level throughput gain introduced by FD-capable BS and users. The users can significanlty benefit from the FDE-based FD radio suitable for hand-held devices. We compare experimental results to the analysis (e.g.,~\cite{marasevic2017resource}) and demonstrate practical FD gain in different network settings. Specifically, we consider two types of networks as depicted in Fig.~\ref{fig:exp-net-setup}: (i) \emph{UL-DL networks} with one FD BS and two HD users with inter-user interference (IUI), and (ii) \emph{heterogeneous HD-FD networks} with HD and FD users. Due to hardware limitations, we apply a TDMA setting where each (HD or FD) user takes turn to be activated for the same period of time.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[]{
\label{fig:exp-net-setup-ul-dl}
\includegraphics[width=0.32\columnwidth]{./figs/exp/net_ul_dl/exp_ul_dl_setup.pdf}
}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:exp-net-setup-two-users}
\includegraphics[width=0.32\columnwidth]{./figs/exp/net_two_users/exp_two_users_setup.pdf}
}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:exp-net-setup-three-users}
\includegraphics[width=0.32\columnwidth]{./figs/exp/net_three_users/exp_three_users_setup.pdf}
}
\vspace{-0.5\baselineskip}
\caption{An example experimental setup for: (a) the UL-DL networks with varying $\SNRUL$ and $\SNRDL$, (b) heterogeneous 3-node network with one FD BS and 2 FD users, and (c) heterogeneous 4-node networks with one FD BS, 2 FD users, and one HD user.}
\label{fig:exp-net-setup}
\vspace{-\baselineskip}
\end{figure}
%% figure ends


%%%%%
%%%%%
\subsubsection{UL-DL Networks with IUI}
\label{sssec:exp-net-ul-dl}
We first consider UL-DL networks consisting of one FD BS and two HD users (indexed 1 and 2). Without loss of generality, in this setting, user 1 transmits on the UL to the BS, and the BS transmits to user 2 on the DL (see Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-ul-dl}).

%%
%%
\noindent\textbf{Analytical FD gain}.
We use Shannon's capacity formula $\DataRate{}(\SNR{}) = \BW \cdot \log_{2}(1+\SNR{})$ to compute the \emph{analytical throughput} of a link under bandwidth $\BW$ and link SNR $\SNR{}$. If the BS is only HD-capable, the network throughput in a UL-DL network when the UL and DL share the channel in a TDMA manner with equal fraction of time is given by
%%
\begin{align}
\label{eq:net-ul-dl-tput-hd}
\textstyle
\DataRate{\textrm{UL-DL}}^{\textrm{HD}} = \frac{\BW}{2}\log\left(1+\SNRUL\right) + \frac{\BW}{2}\log\left(1+\SNRDL\right),
\end{align}
%%
where $\SNRUL$ and $\SNRDL$ are the UL and DL SNRs, respectively.

If the BS is FD-capable, the UL and DL can be simultaneously activated with an analytical network throughput of
%%
\begin{align}
\label{eq:net-ul-dl-tput-fd}
\textstyle
\DataRate{\textrm{UL-DL}}^{\textrm{FD}} = \BW\log\left(1+\frac{\SNRUL}{1+\XINR}\right) + \BW\log\left(1+\frac{\SNRDL}{1+\IUI}\right),
\end{align}
%%
where: (i) $\frac{\SNRDL}{1+\IUI}$ is the signal-to-interference-plus-noise ratio (SINR) at the DL HD user, and (ii) $\XINR$ is the residual self-interference-to-noise ratio (XINR) at the FD BS. We set $\XINR=1$ when computing the analytical throughput. Namely, the residual SI power is no higher than the RX noise floor (which can be achieved by the FDE-based FD radio, see Section~\ref{ssec:exp-node}). The \emph{analytical FD gain} is then defined as the ratio $\left(\DataRate{\textrm{UL-DL}}^{\textrm{FD}}/\DataRate{\textrm{UL-DL}}^{\textrm{HD}}\right)$. Note that the FD gain depends on the coupling between $\SNRUL$, $\SNRDL$, and $\IUI$, which depend on the BS/user locations, their TX power, etc. 

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[$\SNRUL=\SI{10}{dB}$]{
\label{fig::exp-net-ul-dl-gain-10db}
\includegraphics[height=1.25in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_10db.eps}
}
\subfloat[$\SNRUL=\SI{15}{dB}$]{
\label{fig::exp-net-ul-dl-gain-15db}
\includegraphics[height=1.25in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_15db.eps}
}
\subfloat[$\SNRUL=\SI{20}{dB}$]{
\label{fig::exp-net-ul-dl-gain-20db}
\includegraphics[height=1.25in]{./figs/exp/net_ul_dl/exp_ul_dl_gain_20db.eps}
}
\vspace{-0.5\baselineskip}
\caption{Analytical (colored surface) and experimental (filled circles) network throughput gain for UL-DL networks consisting of one FD BS and two HD users with varying UL and DL SNR values, and inter-user interference (IUI) levels: (a) $\SNRUL=\SI{10}{dB}$, (b) $\SNRUL=\SI{15}{dB}$, and (c) $\SNRUL=\SI{20}{dB}$. The baseline is the network throughput when the BS is HD.}
\label{fig:exp-net-ul-dl-gain}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%
%%
\noindent\textbf{Experimental FD gain}.
The experimental setup is depicted in Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-ul-dl}, where the TX power levels of the BS and user 1 are set to be $\SI{10}{dBm}$ and $\SI{-10}{dBm}$, respectively. We fix the location of the BS and consider different UL SNR values of $\SNRUL = 10/15/20\thinspace\SI{}{dB}$ by placing user 1 at three different locations. For each value of $\SNRUL$, user 2 is placed at 10 different locations, resulting in varying $\SNRDL$ and $\IUI$ values.

%% table begins
\begin{table}[!t]
\caption{Average FD Gain in UL-DL Networks with IUI.}
\label{table:exp-net-ul-dl-gain}
\vspace{-1.5\baselineskip}
\scriptsize
\begin{center}
% \begin{tabular}{| p{0.1\columnwidth} | p{0.2\columnwidth} | p{0.1\columnwidth} | p{0.2\columnwidth} |}
\begin{tabular}{|c|c|c|}
\hline
UL SNR, $\SNRUL$ & Analytical FD Gain & Experimental FD Gain \\
\hline
$\SI{10}{dB}$ & $1.30\times$ & $1.25\times$ \\
\hline
$\SI{15}{dB}$ & $1.23\times$ & $1.16\times$ \\
\hline
$\SI{20}{dB}$ & $1.22\times$ & $1.14\times$ \\
\hline
\end{tabular}
\end{center}
\vspace{-2\baselineskip}
\end{table}
%% table ends

Fig.~\ref{fig:exp-net-ul-dl-gain} shows the analytical (colored surface) and experimental (filled circles) FD gain, where the analytical gain is extracted using {\eqref{eq:net-ul-dl-tput-hd}} and {\eqref{eq:net-ul-dl-tput-fd}}, and the experimental gain is computed using the measured UL and DL throughput. It can be seen that smaller values of $\SNRUL$ and lower ratios between $\SNRDL$ and $\IUI$ lead to higher throughput gains in both analysis and experiments. The average analytical and experimental FD gains are summarized in Table~\ref{table:exp-net-ul-dl-gain}. Due to practical reasons such as the link SNR difference and its impact on link PRR (see Section~\ref{ssec:exp-snr-prr-relationship}), the experimental FD gain is $7\%$ lower than the analytical FD gain. The results confirm the analysis in~\cite{marasevic2017resource} and demonstrate the practical FD gain achieved in wideband UL-DL networks without any changes in the current network stack (i.e., only bringing FD capability to the BS). Moreover, performance improvements are expected through advanced power control and scheduling schemes.


%%%%%
%%%%%
\subsubsection{Heterogeneous 3-Node Networks}
\label{sssec:exp-net-two-users}

We consider heterogeneous HD-FD networks with 3 nodes: one FD BS and two users that can operate in either HD or FD mode (see an example experimental setup in Figs.\ref{fig:intro}\subref{fig:intro-fd-net} and~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-two-users}). All 3 nodes have the same $\SI{0}{dBm}$ TX power so that each user has symmetric UL and DL SNR values of $\SNR{i}$ ($i=1,2$).
% \footnote{To better illustrate the results, we consider symmetric UL and DL SNR values while the link SNRs are different across users. The case with asymmetric UL and DL SNR values can also be evaluated.}
We place user 1 at 5 different locations and place user 2 at 10 different locations for each location of user 1, resulting in a total number of 50 pairs of $(\SNR{1},\SNR{2})$.


%%
%%
\noindent\textbf{Analytical FD gain}.
We set the users to share the channel in a TDMA manner. The analytical network throughput in a 3-node network when zero, one, and two users are FD-capable is respectively given by
%%
\begin{align}
& \textstyle \DataRate{}^{\textrm{HD}} = \frac{\BW}{2}\log\left(1+\SNR{1}\right) + \frac{\BW}{2}\log\left(1+\SNR{2}\right), \label{eq:net-two-users-tput-hd} \\
& \textstyle \DataRate{\textrm{User}~i~\textrm{FD}}^{\textrm{HD-FD}} = \BW\log\left(1+\frac{\SNR{i}}{1+\XINR}\right) + \frac{\BW}{2}\log\left(1+\SNR{\bar{i}}\right),\ \label{eq:net-two-users-tput-hd-fd} \\
& \textstyle \DataRate{}^{\textrm{FD}} = \BW\log\left(1+\frac{\SNR{1}}{1+\XINR}\right) + \BW\log\left(1+\frac{\SNR{2}}{1+\XINR}\right), \label{eq:net-two-users-tput-fd}
\end{align}
%%
where $\XINR=1$ is set (similar to Section~\ref{sssec:exp-net-ul-dl}). We consider both FD gains of $\left(\DataRate{\textrm{User}~i~\textrm{FD}}^{\textrm{HD-FD}}/\DataRate{}^{\textrm{HD}}\right)$ (i.e., user $i$ is FD and user $\bar{i} \ne i$ is HD), and $\left(\DataRate{}^{\textrm{FD}}/\DataRate{}^{\textrm{HD}}\right)$ (i.e., both users are FD). 


%%
%%
\noindent\textbf{Experimental FD gain}.
For each pair of $(\SNR{1},\SNR{2})$, experimental FD gain is measured in three cases: (i) only user 1 is FD, (ii) only user 2 is FD, and (iii) both users are FD. Fig.~\ref{fig:exp-net-two-users} shows the analytical (colored surface) and experimental (filled circles) FD gain for each case. We exclude the results with $\SNR{i}<\SI{3}{dB}$ since the packets cannot be decoded, resulting in a throughput of zero (see Fig.~\ref{fig:exp-prr-vs-snr}).

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-0.5\baselineskip}
\subfloat[Only user 1 FD]{
\label{fig:exp-net-two-users-user1-fd}
\includegraphics[height=1.25in]{./figs/exp/net_two_users/exp_user1_fd_gain_experimental.eps}
}
\subfloat[Only user 2 FD]{
\label{fig:exp-net-two-users-user2-fd}
\includegraphics[height=1.25in]{./figs/exp/net_two_users/exp_user2_fd_gain_experimental.eps}
}
\subfloat[Both users FD]{
\label{fig:exp-net-two-users-both-fd}
\includegraphics[height=1.25in]{./figs/exp/net_two_users/exp_both_fd_gain_experimental.eps}
}
\vspace{-0.5\baselineskip}
\caption{Analytical (colored surface) and experimental (filled circles) network throughput gain for 3-node networks consisting of one FD BS and two users with varying link SNR values: (a) only user 1 is FD, (b) only user 2 is FD, and (c) both users are FD. The baseline is the network throughput when both users are HD.}
\label{fig:exp-net-two-users}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends

%% figure begins
\begin{figure}[!t]
\centering
\includegraphics[width=0.8\columnwidth]{./figs/exp/net_two_users/exp_two_users_fairness.eps}
\vspace{-0.5\baselineskip}
\caption{Measured Jain's fairness index (JFI) in 3-node networks when both users are HD and FD with varying $(\SNR{1},\SNR{2})$.}
\label{fig:exp-net-two-users-fairness}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

The results show that with small link SNR values, the experimental FD gain is lower than the analytical value due to the inability to decode the packets. On the other hand, with sufficient link SNR values, the experimental FD gain exceeds the analytical FD gain. This is because setting $\XINR=1$ in {\eqref{eq:net-two-users-tput-hd-fd}} and {\eqref{eq:net-two-users-tput-fd}} results in a $\SI{3}{dB}$ SNR loss in the analytical FD link SNR, and thereby in a lower throughput. However, in practice, the packets can be decoded with a link PRR of 1 with sufficient link SNRs, resulting in exact twice number of packets being successfully sent over an FD link. Moreover, the FD gain is more significant when enabling FD capability for users with higher link SNR values.

% 0.047/0.036/0.055
Another important metric we consider is the fairness between users, which is measured by the Jain's fairness index (JFI). In the considered 3-node networks, the JFI ranges between 1/2 (worst case) and 1 (best case). Fig.~\ref{fig:exp-net-two-users-fairness} shows the measured JFI when both users operate in HD or FD mode. The results show that introducing FD capability results in an average degradation in the network JFI of only $5.6\%/4.4\%/7.4\%$ for $\SNR{1} = 15/20/25\thinspace\SI{}{dB}$, while the average network FD gains are $1.32\times$/$1.58\times$/$1.73\times$, respectively. In addition, the JFI increases with higher and more balanced user SNR values, which is as expected.


%%%%%
%%%%%
\subsubsection{Heterogeneous 4-Node Networks}
\label{sssec:exp-net-three-users}

We experimentally study 4-node networks consisting of an FD BS and three users with $\SI{10}{dBm}$ TX power (see an example experimental setup in Fig.~\ref{fig:exp-net-setup}\subref{fig:exp-net-setup-three-users}).
% This is limited by the fact that only three FDE PCB cancellers are fabricated, which support one FD BS and at most two FD users.
The experimental setup is similar to that described in Section~\ref{sssec:exp-net-two-users}. 100 experiments are conducts where the 3 users are placed at different locations with different user SNR values. For each experiment, the network throughput is measured in three cases where: (i) zero, (ii) one, and (iii) two users are FD-capable.

Fig.~\ref{fig:exp-net-three-users} shows the CDF of the network throughput of the three cases, where the measured link SNR varies between $5$--$\SI{45}{dB}$. Overall, median network FD gains of $1.25\times$ and $1.52\times$ are achieved in cases with one and two FD users, respectively. The trend shows that in a real-world environment, the total network throughput increases as more users become FD-capable, and the improvement is more significant with higher user SNR values. Note that we only apply a TDMA scheme and a more advanced MAC layer design has the potential to improve the FD gain in these networks.

%% figure begins
\begin{figure}[!t]
\centering
\includegraphics[width=0.8\columnwidth]{./figs/exp/net_three_users/exp_three_users_gain_experimental.eps}
\vspace{-0.5\baselineskip}
\caption{Experimental network throughput gain for 4-node networks when zero, one, or two users are FD-capable, with $\SI{10}{dBm}$ TX power and varying user locations.}
\label{fig:exp-net-three-users}
\vspace{-\baselineskip}
\end{figure}
%% figure ends

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:

==> tex/intro_20180805.tex <==
Full-duplex (FD) wireless -- simultaneous transmission and reception on the same frequency channel -- can significantly improve spectrum efficiency at the physical (PHY) layer and provide many other benefits at the higher layers~\cite{sabharwal2014band,krishnaswamy2016spectrum}. The main challenge associated with FD is the extremely strong self-interference (SI) signal that needs to be suppressed, requiring $90$-$\SI{110}{dB}$ of self-interference cancellation (SIC). 

% However, as the transmitted signal is many orders of magnitude stronger than the useful signal at the input of the receiver, it is extremely challenging to recover the useful signal and enable such a communication. In particular, the self-interfering (SI) signal needs to be suppressed by billions of times, requiring $90$-$\SI{110}{dB}$ of self-interference cancellation (SIC). 

%%
\begin{figure}[!t]
\centering
\subfloat[]{
\label{fig:intro-pcb}
\includegraphics[height=1.18in]{./figs/testbed/testbed_fde_canc.pdf}}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:intro-fd-radio}
\includegraphics[height=1.18in]{./figs/testbed/testbed_fd_radio.pdf}}
\\ \vspace{-.75\baselineskip}
\subfloat[]{
\label{fig:intro-fd-link}
\includegraphics[width=0.85\columnwidth]{./figs/testbed/testbed_fd_link.png}}
\vspace{-\baselineskip}
\caption{(a) Our frequency-domain equalization- (FDE-) based wideband RF canceller implemented using discrete components on a PCB, (b) our implemented FDE-based FD radio, and (c) \memoTC{replace figure by a network.}}
\label{fig:intro}
\vspace{-\baselineskip}
\end{figure}
%%

Recent work leveraging off-the-shelf components and software-defined radios (SDRs) has established the feasibility of FD wireless through SI suppression at the antenna interface, and SIC in analog/RF and digital domains~\cite{choi2010achieving,duarte2010full,khojastepour2011case,bharadia2013full,korpi2016full}. However, existing approaches to achieve wideband RF SIC (e.g.,~\cite{bharadia2013full, korpi2016full}) rely on RF cancellers with transmission-line delays. Such delay lines cannot be realized in small-form-factor devices and/or integrated circuit (IC) implementations, due to the required lengthy for generating nanosecond-scale time delays and the lossy nature of the silicon substrate.\footnote{For instance, obtaining a nanosecond delay in silicon typically requires a $\SI{15}{cm}$-long delay line.}

A \emph{compact IC-based} design is necessary for supporting FD in hand-held devices (e.g., handsets and tablets). Recently, the first IC-based implementations of wideband FD transceivers have emerged~\cite{yang2015wideband,Zhou_WBSIC_JSSC15}. Recent advances in the RFIC community have demonstrated the practicality to achieve wideband RF SIC in an IC implementation based on the technique of frequency-domain equalization (FDE)~\cite{Zhou_WBSIC_JSSC15}. In contrast to the delay line-based approaches (which are essentially performing time-domain equalization), the FDE-based RF canceller utilizes tunable, reconfigurable, high quality factor $2^{\textrm{nd}}$-order bandpass filters (BPFs) with amplitude and phase controls to emulate the frequency-selective antenna interface. In general, tunable, high quality factor BPFs are perhaps as hard to be implemented on an IC as nanosecond-scale delay lines, but $N$-path filters represent an exciting advance that has enabled their implementation in nanoscale CMOS over the past few years~\cite{ghaffari2011tunable,reiskarimian2016analysis}.

% recent advances in the RFIC community have demonstrated the practicality to achieve wideband RF SIC in an IC implementation based on the frequency-domain equalization (FDE) of the antenna interface using widely tunable, high quality factor $2^{\textrm{nd}}$-order BPFs with amplitude and phase controls~\cite{Zhou_WBSIC_JSSC15}.
% In contrast to the delay line-based approaches (which are essentially performing time-domain equalization), recent advances in the RFIC community have demonstrated the practicality to achieve wideband RF SIC in an IC implementation based on the frequency-domain equalization (FDE) of the antenna interface using widely tunable, high quality factor $2^{\textrm{nd}}$-order BPFs with amplitude and phase controls~\cite{Zhou_WBSIC_JSSC15}.
% Recent advances in the implementation of tunable, reconfigurable, high quality factor RF BPFs in nanoscale CMOS, namely N-path filters, enable the design of a compact RF canceller that can emulate a frequency-selective antenna interface without using bulky delay lines~\cite{Zhou_WBSIC_JSSC15, reiskarimian2016analysis}.

While major advances have been made at the IC level, there is still a need to understand the fundamental limits of the achievable RF SIC based on technique of FDE and to develop optimized configuration for this new type of RF canceller to achieve optimal RF SIC. It is also important to to evaluate the performance of such compact FD radios in different network settings in real-world environment. \emph{The focus on this paper is on the implementation, optimization, and experimentation of the FDE-based RF canceller that is suitable for wideband compact FD nodes}.
 

% The fundamental challenge associated with achieving wideband RF SIC is due to the frequency selectivity of the antenna interface. Although there has been extensive bench-top implementations of FD transceivers supporting practical levels of SIC across sufficient bandwidth (see ~\cite{bharadia2013full, korpi2016full} and the references in~\cite{sabharwal2014band}), the underlying approaches to achieve SIC at RF (referred to as \emph{RF SIC}) suffer from large radio dimensions that are unsuitable for compact/small-form-factor devices (e.g., laptops and cell phones).

% These approaches to achieve wideband RF SIC are based on transmission-line delays, which are fundamentally impractical to be realized in small-form-factor devices and/or Integrated Circuit (IC) implementations. This is due to the lengthy and bulky transmission-lines required for generating nanosecond-scale true time delays and the lossy nature of the silicon substrate.

% In~\cite{fd_demo_mobihoc16}, we demonstrated an FD radio implementation using a conventional frequency-flat amplitude- and phase-based RF canceller that emulates its RFIC canceller counterpart presented in~\cite{Zhou_NCSIC_JSSC14}. However, this conventional RF canceller can only emulate the antenna interface response at a single frequency point, resulting in a narrowband RF SIC.

% Recent advances in the implementation of tunable, reconfigurable, high quality factor RF BPFs in nanoscale CMOS, namely N-path filters, enable the design of a compact RF canceller that can emulate a frequency-selective antenna interface without using bulky delay lines~\cite{Zhou_WBSIC_JSSC15, reiskarimian2016analysis}. This new approach is based on frequency-domain equalization (FDE) of the antenna interface using reconfigurable RF bandpass filters (BPFs).
% our work focuses on the design and implementation of wideband compact RF cancellers. Our approach is based on the frequency-domain equalization (FDE) of the antenna interface using reconfigurable RF bandpass filters (BPFs). Recent advances in the implementation of tunable, reconfigurable, high quality factor RF BPFs in nanoscale CMOS, namely N-path filters, enable the design of a compact RF canceller that can emulate a frequency-selective antenna interface without using bulky delay lines~\cite{Zhou_WBSIC_JSSC15, reiskarimian2016analysis}. In general, tunable, high quality factor filters are perhaps as hard to be implemented on an IC as nanosecond-scale delay lines, but N-path filters represent an exciting advance that has enabled their implementation over the past few years~\cite{ghaffari2011tunable,reiskarimian2016analysis}. Recent advances in the RFIC community have demonstrated the practicality to realize widely tunable high quality factor $2^{\textrm{nd}}$-order BPFs with amplitude and phase controls~\cite{Zhou_WBSIC_JSSC15}.
% Therefore, an RF canceller consisting of multiple FDE taps (BPFs) can channelize the signal bandwidth and emulate the antenna interface. However, there is a lack in both the optimal configuration of the FDE-based canceller and the system-level FD gain introduced by it. \emph{The focus on this paper is on the modeling, optimization, and experimentation of FDE-based wideband RF cancellers that are suitable for compact implementations}.
 
Since while interfacing an RFIC canceller to an SDR presents numerous technical challenges, in this work, we design and implement the FDE-based RF canceller using discrete components on a printed circuit board (PCB), see Fig.~\ref{fig:intro}\subref{fig:intro-pcb} (we refer to it as the \emph{PCB canceller}). The FDE-based PCB canceller can largely facilitate the evaluation of the canceller configuration scheme and the experiments using an SDR platform, as well as to build a network with multiple FDE-based FD nodes.
% In this work, we design and implement the FDE-based RF canceller using discrete components on a printed circuit board (PCB), see Fig.~\ref{fig:intro}\subref{fig:intro-pcb} (we refer to it as the \emph{PCB canceller}).
Moreover, the PCB canceller is more robust and stable to be integrated with the open-access ORBIT~\cite{orbit} and COSMOS~\cite{COSMOS} testbeds to allow the broader community to experiment with wideband compact FD wireless, as we plan to do.\footnote{A narrowband RF canceller has been integrated with the ORBIT testbed~\cite{flexicon_orbit_gen1}.} We present a realistic model of the PCB canceller and its configuration scheme based on an optimization problem. The PCB canceller model is experimentally validated based on measurements and is shown to have high accuracy.

% We present a generalized model for an FDE-based RF canceller and consider two specific models: (i) an \emph{ideal FDE-based canceller} model using $2^{\textrm{nd}}$-order RF BPFs that accurately captures the characteristics of the RFIC canceller~\cite{Zhou_WBSIC_JSSC15}, and (ii) a \emph{FDE-based PCB canceller} model based on an FDE-based RF canceller implemented on a printed circuit board (PCB) in this work. % Figs.~\ref{fig:intro}\subref{fig:intro-fd-radio}and~\ref{fig:intro}\subref{fig:intro-pcb} depict our implemented FD radio equipped with an PCB-based FDE RF canceller that emulates its RFIC counterpart in~\cite{Zhou_WBSIC_JSSC15}, and Fig.~\ref{fig:intro}\subref{fig:intro-fd-link} shows an FD wireless link that we demonstrated in~\cite{fd_demo_infocom17}.
% Figs.~\ref{fig:intro}\subref{fig:intro-fd-radio} and~\ref{fig:intro}\subref{fig:intro-pcb} depict our implemented FD radio equipped with an PCB-based FDE RF canceller implemented using discrete components.

% The PCB canceller also supports higher TX power handling when compared to the RFIC canceller.

% In order to obtain good RF SIC performance using FDE-based cancellers, we formulate optimization problems with practical constraints for the specific models. In all cases, the objective is to use the FDE-based cancellers to best emulate the antenna interface. Although the non-convex and non-linear nature of the problems results in analytical intractability, we show that the optimization problems can still be numerically solved efficiently. Moreover, in practice, it is unnecessary to find the globally optimal canceller configuration as long as the obtained optimized solution can provide sufficient amount of wideband RF SIC. We also show that when the FDE-based canceller is configured using the solutions to these optimization problems, it performs better than when configured using the iterative configuration algorithm proposed in~\cite{Zhou_WBSIC_JSSC15}.

% We then experimentally validate the PCB canceller model and use them for performance evaluation with the optimized canceller configuration. In particular, the RFIC canceller is numerically evaluated in cases with and without practical hardware constraints. Furthermore, the trade-offs between the RF SIC performance (e.g., desired RF SIC bandwidth) and various configuration parameters (e.g., number of FDE taps) are evaluated. Numerical results show that even under practical constraints, an RFIC canceller with 4 FDE taps is capable of achieving an average $\SI{50}{dB}$ RF SIC across up to $\SI{80}{MHz}$ bandwidth.

We implement an FDE-based FD radio by integrating the PCB canceller with an NI USRP SDR platform, as depicted in Fig.~\ref{fig:intro}\subref{fig:intro-fd-radio}. We experimentally evaluate the performance of the FDE-based FD radio with the canceller configuration scheme, which allows efficient tuning of the PCB canceller to adapt to environmental changes. The FDE-based FD radio achieves $\SI{95}{dB}$ overall SIC across $\SI{20}{MHz}$ real-time bandwidth, enabling an FD link budget of $\SI{10}{dBm}$ average TX power level and $-\SI{85}{dBm}$ RX noise floor. In particular, $\SI{52}{dB}$ SIC is achieved in the RF domain, from which $\SI{20}{dB}$ is obtained from the antenna interface isolation.

We also evaluate the performance and robustness of the FDE-based FD radio at the link-level in the context of packet reception ratio (PRR) and FD throughput gain, in both line-of-sight (LOS) and non-line-of-sight (NLOS) settings. The results show that the FDE-based FD radio achieves an average FD link throughput gain of 1.85$\times$--1.91$\times$, while the link SNR difference when the radio operates in HD and FD modes is only less than $\SI{1}{dB}$.
\memoTC{also add 1(c) of the network}

We extensively evaluate the network-level FD gain in two types of networks, and compare to and confirm the analytical results: (i) \emph{UL-DL networks} consisting of one FD base station (BS) and two half-duplex (HD) users with inter-user interference (IUI), and (ii) \emph{heterogeneous HD-FD networks} consisting of one FD BS and co-existing HD and FD users. For UL-DL networks, we show experimentally that the throughput gain is between  1.14$\times$--1.25$\times$ compared to 1.22$\times$--1.3$\times$ predicted by analysis. We discuss the relationship with UL and DL SNR values, as well as the IUI levels. For heterogeneous HD-FD networks, we demonstrate through experiments the impact of different user SNR values on the throughout, as well as the relationship between the network throughput gain and the number of FD users in the network. For example, in a 4-node network consisting of one FD BS and 3 users with various user locations and SNR values, median experimental FD gains of 1.25$\times$ and 1.52$\times$ can be achieved when one and two users become FD-capable, respectively. To the best of our knowledge, this is the first experimental study of FD gains in such networks. The results can serve as the fundamental building blocks for developing more advanced and efficient MAC layers. The results also demonstrate the performance of compact FD radio designs suitable for hand-held devices, which can be realized through the FDE-based approach.

Finally, we perform sensitivity analysis of the FDE-based cancellers with varying design parameters, and compare the performance between the RFIC and PCB implementations. We show that  optimized canceller configuration is shown to outperform the heuristic canceller configuration in the RFIC implementation~\cite{Zhou_WBSIC_JSSC15} by an order of magnitude in terms of the achieved RF SIC;

%%
%% Contributions
% To summarize, the main contributions of the paper are three-fold:
% \begin{enumerate}[topsep=0pt,itemsep=0pt]%[topsep=0pt, leftmargin=*]
% \item[(i)]
% We present a general FDE-based RF canceller model for achieving wideband RF SIC in compact devices. In addition, two specific models are considered and validated based on our practical implementations of an RFIC canceller and a PCB canceller;
% \item[(ii)]
% We propose an optimization framework for efficiently obtaining optimized FDE-based canceller configuration and use it for performance evaluation of the FDE-based cancellers;
% \item[(iii)]
% We numerically evaluate the RFIC canceller model and the trade-offs between various design parameters. We experimentally evaluate the PCB canceller using an SDR testbed.
% \end{enumerate}

To summarize, the main contributions of the paper are:
\begin{enumerate}[topsep=0pt,itemsep=-5pt]%[topsep=0pt, leftmargin=*]
\item[(i)]
We present the design, implementation, modeling validation, and a canceller configuration scheme of the FDE-based PCB canceller, which can be used to evaluate the performance of FDE-based approach suitable for achieving wideband RF SIC compact nodes;
\item[(ii)]
We experimentally evaluate our FDE-based FD radio with the PCB canceller and the optimized canceller configuration. 
\item[(iii)]
We experimentally evaluate the throughput gain introduced by FD in various network settings with different user capabilities (i.e., HD or FD) and user SNR values.\memoTC{also say something about the sensitivity analysis that we analyze and evaluate the fundamentals for the FDE-based approach?}
\end{enumerate}

The rest of the paper is organized as follows. Section~\ref{sec:related} reviews related work. In Section~\ref{sec:background}, we introduce FD background and the problem formulation, as well as RF canceller designs. We present the design, implementation, and model of the FDE-based PCB canceller, as well as the optimal canceller configuration scheme in Section~\ref{sec:impl}. The performance of the FDE-based FD radio is experimentally evaluated at the node, link, and network levels in Sections~\ref{sec:exp}. In Section~\ref{sec:sensitivity}, we perform sensitivity analysis of the FDE-based cancellers and compare the RFIC and PCB implementations. We conclude and discuss future directions in Section~\ref{sec:conclusion}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/pcb_validation.tex <==
%%
%%
% In this section, we experimentally validate both the PCB BPF model {\eqref{eq:pcb-bpf-tf}} and the PCB canceller model {\eqref{eq:pcb-tf-calibrated}}.
% We first perform measurements to validate both the PCB BPF {\eqref{eq:pcb-bpf-tf}} and the PCB canceller {\eqref{eq:pcb-tf-calibrated}} models.
% Then, we perform system-level evaluation of our FD radio design with optimized PCB canceller configuration in an SDR testbed. We also perform model-based evaluation of the PCB canceller with a larger number of FDE taps, $\NumTap$.


%%%%%
%%%%%
% \subsubsection*{Validation of the PCB BPF}
\noindent\textbf{Validation of the PCB BPF}.
We first experimentally validate the PCB BPF model, $\BPFTapTF{i}(f_k)$, given by {\eqref{eq:pcb-bpf-tf}}. The ground truth is obtained by measuring the frequency response (using S-Parameters measurements) of the PCB BPF using a test structure, which contains only the BPF, to avoid the effects of other components on the PCB. The measurements are conducted with varying $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ configurations and the result of each configuration is averaged over 20 measurement instances.\footnote{We drop the subscript $i$, since both PCB BPFs behave identically.} The BPF center frequency is measured as the frequency with the highest BPF amplitude, and the BPF quality factor is computed as the ratio between the center frequency and the {3}\thinspace{dB} bandwidth around the center frequency.
% Due to practical implementation losses, we use multi-dimensional curve-fitting to better tune parameters $L_1 = \SI{1.85}{nH}$ and $L_2 = \SI{3.28}{nH}$ (see Fig.~\ref{fig:impl-fde}).

The PCB BPF has a \emph{fixed} quality factor of 2.7, achieved by using only the RLC resonance tank. By setting $\PCBTapQFCapNoidx = \PCBTapQFCapMax$ and $\PCBTapQFCapNoidx = \PCBTapQFCapMin$ (see Section~\ref{ssec:impl-pcb}), the measured lowest and highest achievable BPF quality factors are 9.2 and 17.8, respectively. This shows an improvement in the PCB BPF quality factor tuning range of 3.4$\times$--6.6$\times$, achieved by introducing the impedance transformation networks. Similarly, by setting $\PCBTapCFCapNoidx = \PCBTapCFCapMax$ and $\PCBTapCFCapNoidx = \PCBTapCFCapMin$, the PCB BPF has a center frequency tuning range of {18}\thinspace{MHz}.

%% table begins
\begin{table}[!t]
\caption{Four $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ configurations used in the validations.}
\label{table:set-cap}
\vspace{-\baselineskip}
\scriptsize
\begin{center}
% \begin{tabular}{| p{0.1\columnwidth} | p{0.2\columnwidth} | p{0.1\columnwidth} | p{0.2\columnwidth} |}
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{|c|c|c|}
\hline
& Highest Q-Factor & Lowest Q-Factor \\
\hline
Highest Center Freq. & Set 1: $(\PCBTapCFCapMin, \PCBTapQFCapMin)$ & Set 3: $(\PCBTapCFCapMin, \PCBTapQFCapMax)$ \\
\hline
Lowest Center Freq. & Set 2: $(\PCBTapCFCapMax, \PCBTapQFCapMin)$ & Set 4: $(\PCBTapCFCapMax, \PCBTapQFCapMax)$ \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\end{center}
\vspace{-\baselineskip}
\end{table}
%% table ends

Fig.~\ref{fig:eval-pcb-bpf} presents the modeled and measured amplitude and phase responses of the PCB BPF with 4 different $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ configurations (see Table~\ref{table:set-cap}) which cover the entire tuning range of the BPF center frequency and quality factor.
Table~\ref{table:accuracy-bpf} summarizes the maximum differences between the measured and modeled amplitude and phase of the PCB BPF in the range of {850--950}\thinspace{MHz}.
In particular, the PCB BPF model {\eqref{eq:pcb-bpf-tf}} matches very closely with the measurements at the highest BPF quality factor value, where the maximum differences between the measured and modeled amplitude and phase in Set 1/2 are {0.6/0.8}\thinspace{dB} and {7.4}$^{\circ}$/{5.0}$^{\circ}$, respectively.
At the lowest BPF quality factor value, the differences in Set 3/4 are {1.2/1.2}\thinspace{dB} and {13.8}$^{\circ}$/{15.1}$^{\circ}$, respectively, still showing the validity of the PCB BPF model.
The same level of accuracy of the PCB BPF model {\eqref{eq:pcb-bpf-tf}} is also observed for other $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ configurations within their tuning ranges.
% The results show that the PCB BPF model {\eqref{eq:pcb-bpf-tf}} matches very closely with the measurements at the highest BPF quality factor value (Sets 1 and 2). In particular, the PCB BPF model {\eqref{eq:pcb-bpf-tf}} matches very closely with the measurements at the highest BPF quality factor value (Sets 1 and 2), where the maximum differences in amplitude and phase are {0.5}\thinspace{dB} and {7}$^{\circ}$, respectively.
% \remove{At the lowest BPF quality factor value (Sets 3 and 4), the differences are {1.2}\thinspace{dB} and {15}$^{\circ}$, thereby showing the validity of the PCB BPF model. The same level of accuracy of the PCB BPF model {\eqref{eq:pcb-bpf-tf}} is also observed for other $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ configurations within their tuning ranges.}

%%
%%
% \subsection{Validation of the PCB Canceller}
% \label{ssec:pcb-validation-fde}

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat{
\label{fig:eval-pcb-bpf-amp}
\includegraphics[width=0.47\columnwidth]{./figs/model/model_bpf_amp.eps}
}
\hfill
\subfloat{
\label{fig:eval-pcb-bpf-phase}
\includegraphics[width=0.47\columnwidth]{./figs/model/model_bpf_phase.eps}
}
\vspace{-0.5\baselineskip}
\caption{Modeled and measured amplitude and phase responses of the implemented PCB BPF with varying $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ indicated in Table~\ref{table:set-cap}.}
\label{fig:eval-pcb-bpf}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends


%%%%%
%%%%%
% \subsubsection*{Validation of the PCB Canceller}
\noindent\textbf{Validation of the PCB canceller}.
We use the same experiments as in the PCB BPF validation to validate the PCB canceller model with 2 FDE taps, $\PCBTF(f_k)$, given by {\eqref{eq:pcb-tf-calibrated}}. We consider two cases for controlled measurements: (i) only one FDE tap is active, and (ii) both FDE taps are active. Note that the programmable attenuators have a maximal attenuation of only {15.5}\thinspace{dB} (see Section~\ref{ssec:impl-pcb}) and at this maximal attenuation, signals can still leak through the FDE tap, resulting in inseparable behaviors between the two FDE taps.

%% table begins
\begin{table}[!t]
\caption{Accuracy of the PCB BPF model with varying $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ indicated in Table~\ref{table:set-cap}.}
\label{table:accuracy-bpf}
\vspace{-\baselineskip}
\scriptsize
\begin{center}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{|c|c|c|c|c|}
\hline
& Set 1 & Set 2 & Set 3 & Set 4 \\
\hline
Max Difference in Amplitude & {0.6}\thinspace{dB} & {0.8}\thinspace{dB} & {1.2}\thinspace{dB}  & {1.2}\thinspace{dB} \\
\hline
Max Difference in Phase & {7.4}$^{\circ}$ & {5.0}$^{\circ}$ & {13.8}$^{\circ}$ & {15.1}$^{\circ}$ \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\end{center}
\vspace{-\baselineskip}
\end{table}
%% table ends

To minimize the effect of the second FDE tap, we set the 1$^{\textrm{st}}$ FDE tap at its highest amplitude (i.e., lowest attenuation value of $\PCBTapAmp{1}$) with varying values of $(\PCBTapCFCap{1}, \PCBTapQFCap{1})$ while setting the 2$^{\textrm{nd}}$ FDE tap with the lowest amplitude (i.e., highest attenuation value of $\PCBTapAmp{2}$). Fig.~\ref{fig:eval-pcb} shows the modeled and measured amplitude and phase responses of the PCB canceller in this case, i.e., only the 1$^{\textrm{st}}$ FDE tap is active. The corresponding maximum differences are summarized in Table~\ref{table:accuracy-fde}. The results show that at the highest BPF quality factor value, the maximum differences in amplitude and phase for Set 1/2 are {1.0/0.9}\thinspace{dB} and {2.2}$^{\circ}$/{7.6}$^{\circ}$, respectively. At the lowest BPF quality factor value, the maximum differences for Set 3/4 are {1.7/1.5}\thinspace{dB} and {7.2}$^{\circ}$/{11.4}$^{\circ}$, respectively, still validating the PCB canceller model. Table~\ref{table:accuracy-fde} also shows similar results in the case where only the 2$^{\textrm{nd}}$ FDE tap is active by setting highest attenuation value of $\PCBTapAmp{1}$ and lowest attenuation value of $\PCBTapAmp{2}$.
The measurements are repeated with different $\{\PCBTapAmp{i}, \PCBTapPhase{i}, \PCBTapCFCap{i}, \PCBTapQFCap{i}\}$ settings for $i=1,2$, and all the results demonstrate the same level of accuracy of the PCB canceller model {\eqref{eq:pcb-tf-calibrated}} (see Fig.~\ref{fig:exp-usrp-algo} for an example).

% At the highest BPF quality factor value (Sets 1 and 2), the maximum differences between the modeled and measured amplitude and phase are {0.9}\thinspace{dB} and {8}$^{\circ}$, respectively. At the lowest BPF quality factor value (Sets 3 and 4), the errors are {1.5}\thinspace{dB} and {12}$^{\circ}$, while still validating the PCB canceller model. We obtain similar results in the case where only the second FDE tap is active by setting highest attenuation value of $\PCBTapAmp{1}$ and lowest attenuation value of $\PCBTapAmp{2}$. The measurements are repeated with different $\{\PCBTapAmp{i}, \PCBTapPhase{i}, \PCBTapCFCap{i}, \PCBTapQFCap{i}\}$ settings for $i=1,2$, and all the results demonstrate the same level of accuracy of the PCB canceller model {\eqref{eq:pcb-tf-calibrated}}.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat{
\label{fig:eval-pcb-amp}
\includegraphics[width=0.47\columnwidth]{./figs/model/model_fde_amp.eps}
}
\hfill
\subfloat{
\label{fig:eval-pcb-phase}
\includegraphics[width=0.47\columnwidth]{./figs/model/model_fde_phase.eps}
}
\vspace{-0.5\baselineskip}
\caption{Modeled and measured amplitude and phase responses of the PCB canceller, where only the 1$^{\textrm{st}}$ FDE tap is active, with varying $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ indicated in Table~\ref{table:set-cap}.}
\label{fig:eval-pcb}
\vspace{-0.5\baselineskip}
\end{figure}
%% figure ends

%% table begins
\begin{table}[!t]
\caption{Accuracy of the PCB canceller model, where only the 1$^{\textrm{st}}$ or 2$^{\textrm{nd}}$ FDE tap is active, with varying $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ indicated in Table~\ref{table:set-cap}.}
\label{table:accuracy-fde}
\vspace{-\baselineskip}
\scriptsize
\begin{center}
\renewcommand{\arraystretch}{1.0}
\begin{tabular}{|c|c|c|c|c|}
\hline
& Set 1 & Set 2 & Set 3 & Set 4 \\
\hline
Max Difference in Amplitude (1$^{\textrm{st}}$ tap) & {1.0}\thinspace{dB} & {0.9}\thinspace{dB} & {1.7}\thinspace{dB} & {1.5}\thinspace{dB} \\
\hline
Max Difference in Phase (1$^{\textrm{st}}$ tap) & {2.2}$^{\circ}$ & {7.6}$^{\circ}$ & {7.2}$^{\circ}$ & {11.4}$^{\circ}$ \\
\hline
Max Difference in Amplitude (2$^{\textrm{nd}}$ tap) & {1.6}\thinspace{dB} & {1.6}\thinspace{dB} & {2.5}\thinspace{dB} & {2.2}\thinspace{dB} \\
\hline
Max Difference in Phase (2$^{\textrm{nd}}$ tap) & {6.4}$^{\circ}$ & {5.1}$^{\circ}$ & {11.8}$^{\circ}$ & {9.7}$^{\circ}$ \\
\hline
\end{tabular}
\renewcommand{\arraystretch}{1}
\end{center}
\vspace{-\baselineskip}
\end{table}
%% table ends

% %% table begins
% \begin{table}[!t]
% \caption{\revise{Accuracy of the PCB canceller model, where only the 2$^{\textrm{nd}}$ FDE tap is active, with varying $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$.}}
% \label{table:accuracy-fde-2nd-tap}
% \vspace{-\baselineskip}
% \scriptsize
% \begin{center}
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% & Set 1 & Set 2 & Set 3 & Set 4 \\
% \hline
% Max Difference in Amplitude & {1.6}\thinspace{dB} & {1.6}\thinspace{dB} & {2.5}\thinspace{dB} & {2.2}\thinspace{dB} \\
% \hline
% Max Difference in Phase & {6.4}$^{\circ}$ & {5.1}$^{\circ}$ & {11.8}$^{\circ}$ & {9.7}$^{\circ}$ \\
% \hline
% \end{tabular}
% \renewcommand{\arraystretch}{1}
% \end{center}
% \vspace{-\baselineskip}
% \end{table}
% %% table ends


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/removed.tex <==
\subsection{A Heuristic Iterative Approach}
Because of the high-complexity of Algorithm~\ref{algo:opt-joint}, we also present a more efficient iterative approach to optimize for the FDE canceller parameters. The idea of this approach (as described in Algorithm~\ref{algo:opt-iterative}) iteratively emulates the SI channel response, $\SIChnlTF(f)$, at different desired SIC frequency points $\{\IterSICFreq{i}\}_{i=1}^{N}$ using $N$ FDE taps by treating the residual SI channel response from the previous iteration as the new SI channel. Note that this iterative approach is not optimal since including the $i$-th FDE tap will also affect the residual SI channel response from the $(i-1)$-th iteration.

From the SI channel response, $\SIChnlTF(f)$, it is not hard to compute the amplitude, phase, slope of amplitude, and slope of phase by solving the following equations:
%%
\begin{align}
|\FDEChnlTF{i}(f)| & = \frac{\Amp{i}}{\sqrt{1+\QFactor{i}K_i(f)}} = |\SIChnlTF(\IterSICFreq{i})|\\
\angle\FDEChnlTF{i}(f) & = \tan^{-1} (\QFactor{i}K_i(f)) - \Phase{i} = \angle \SIChnlTF(\IterSICFreq{i}) \\
\frac{\textrm{d} |\FDEChnlTF{i}(f)|}{\textrm{d} f} & = \frac{\textrm{d} |\SIChnlTF(f)|}{\textrm{d} f} \Big|_{f = \IterSICFreq{i}} \\
\frac{\textrm{d} \angle\FDEChnlTF{i}(f)}{\textrm{d} f} & = \frac{\textrm{d} \angle\SIChnlTF(f)}{\textrm{d} f} \Big|_{f = \IterSICFreq{i}}
\end{align}
%%
From the FDE tap model {\eqref{eq:fde-tap-tf}}, the amplitude, phase, slope of amplitude, and slope of phase of the $i$-th FDE tap at 

%% Iterative optimization
\begin{algorithm}[!h]
\caption{Iterative Algorithm}
\label{algo:opt-iterative}
\begin{algorithmic}[1]
% input
\State
Input:
Desired center frequency matching points of the $N$ FDE taps, $\IterSICFreqVec = [\IterSICFreq{i},\cdots,\IterSICFreq{N}]$, and the desired self-interference cancellation frequency range $[f_{\rm min}, f_{\rm max}]$. Initialize $\ResSIChnlTF{0}(f) = \SIChnlTF(f)$.
% solve opt
\For{$i = 1,\cdots,N$}
\State Find the configurations for the $i$-th FDE tap by using equations [CITE EQ];
\State Compute the residual SI channel response: $\ResSIChnlTF{i}(f) \leftarrow \ResSIChnlTF{i-1}(f) - \FDEChnlTF{i}(f|\Amp{i},\Phase{i},\CenterFreq{i},\QFactor{i})$;
\EndFor
% return
\State
Return the configuration for all the $N$ FDE channels.
\end{algorithmic}
\normalsize
\end{algorithm}
%%



In this section, we describe our adaptive tuning algorithm based on the FDE-based canceller.

We denote $\FDEChnlTF{i}(j\omega) = H_i(j\omega) e^{-j\omega\tau_i} \cdot H_i^{\rm BPF}(j\omega)$ as the frequency response of the $i$-th FDE channel containing one attenuator, one phase shifter, and one BPF. Recall from the above model, for simplicity, we also include the constant gain and group delay into $\FDEChnlTF{i}(j\omega)$. For brevity, we use the vector form to denote the tunable parameters for all the FDE channels, i.e., $\CapCFvec = [\CapCF{i}]_{i=1}^{N}$, $\CapQFvec = [\CapQF{i}]_{i=1}^{N}$, $\Attvec = [\Att{i}]_{i=1}^{N}$, and $\PSvec = [\PS{i}]_{i=1}^{N}$.


%%
%%
\subsection{Joint Optimization}
\label{ssec:algo-joint}

Ideally, we would like to solve for the configuration for the $N$ parallel FDE channels to best emulate the self-interference channel, $\SIChnlTFvec(f)$, i.e., 
%%
\begin{align}
\min:\ || \SIChnlTFvec(f) - \sum_{i=1}^{N} \FDEChnlTFvec{i}(f) ||_2^2.
\end{align}
%%
Unlike the conventional frequency flat amplitude- and phase-based RF canceller [CITE MOBIHOC'16 DEMO] which can only emulate $\SIChnlTFvec(f)$ at a single frequency point, the key idea here is to use the FDE channels to emulate the SI channel $\SIChnlTFvec(f)$ across the desired bandwidth. Essentially, the objective allows the FDE canceller to not only match with $\SIChnlTFvec(f)$ (in both amplitude and phase) across the desired bandwidth, but more importantly, match with the group delay. This is critical since the group delay is essentially the negative of the derivative of the phase, which cannot be obtained by just looking at a single frequency point.

%% Joint optimization
\begin{algorithm}[!h]
\caption{Joint Optimization}
\label{algo:joint}
\begin{algorithmic}[1]
% input
\State
Input:
$C_i \in [C_{\rm min}, C_{\rm max}],\ Q_i \in [Q_{\rm min}, Q_{\rm max}],\ A_i \in [-\SI{50}{dB}, \SI{0}{dB}],\ \phi_i \in [-\pi, \pi],$ and the desired self-interference cancellation frequency range $[f_{\rm min}, f_{\rm max}]$.
% solve opt
\State
Solve the following optimization problem using a gradient descent method:
\begin{align}
\min_{C_i,\ Q_i,\ A_i,\ \phi_i,\ \forall i=1,\cdots,N}\ || \SIChnlTFvec(f) - \sum_{i=1}^{N} \FDEChnlTFvec{i}(f) ||_2^2.
\end{align}
% return
\State
Return the configurations $C$, $Q$, $A$, and $\phi$.
\end{algorithmic}
\normalsize
\end{algorithm}
%%

\memoTC{Say something about the complexity? It might be hard since we are using numerical gradient descent based on measured SI channel response.}
Note that Algorithm~\ref{algo:joint} is a multi-dimensional optimization problem in which, except for the frequency $f$, the $i$-th FDE channel has four variables:  $\FDEChnlTF{i}(f) = \FDEChnlTF{i}(f | C_i, Q_i, A_i, \phi_i)$. Based on the measured discrete SI channel response (e.g., the response of the antenna interface), one can solve for the optimum configurations using a numerical gradient descent.


%%
%%
\subsection{A Heuristic Iterative Approach}
\label{ssec:algo-iterative}
Because of the high-complexity of Algorithm~\ref{algo:joint}, we also proposed a more efficient iterative approach to optimize for the FDE channels. Essentially, this approach iteratively (as described in Algorithm~\ref{algo:iterative}) emulates the SI channel response, $\SIChnlTF(f)$ at several frequency points $\{f_i\}_{i=1}^{N}$ using $N$ FDE channels by treating the residual SI channel response from the previous iteration as the new SI channel. Note that this approach does not involve matching the group delay but, as we will show below, it can still achieve relatively good SIC performance in a much simpler fashion.

%% Iterative optimization
\begin{algorithm}[!h]
\caption{Iterative Algorithm}
\label{algo:iterative}
\begin{algorithmic}[1]
% input
\State
Input:
$C_i \in [C_{\rm min}, C_{\rm max}],\ Q_i \in [Q_{\rm min}, Q_{\rm max}],\ A_i \in [-\SI{50}{dB}, \SI{0}{dB}],\ \phi_i \in [-\pi, \pi],$ and the desired self-interference cancellation frequency range $[f_{\rm min}, f_{\rm max}]$. Set $\ResSIChnlTFvec{0}(f) = \SIChnlTFvec(f)$.
% solve opt
\For{$i = 1,\cdots,N$}
\State Find the configurations for the $i$-th FDE channel, $(C_i,Q_i,A_i,\phi_i)$, that minimizes $|| \ResSIChnlTF{i-1}(f_i) - \FDEChnlTF{i}(f_i) ||_2$;
\State Compute the residual self-interference channel response: $\ResSIChnlTFvec{i}(f) \leftarrow \ResSIChnlTFvec{i-1}(f) - \FDEChnlTFvec{i}(f|C_i,Q_i,A_i,\phi_i)$;
\EndFor
% return
\State
Return the configuration for all the $N$ FDE channels.
\end{algorithmic}
\normalsize
\end{algorithm}
%%

\memoTC{Talk about the monotonicity property of the FDE transfer function w.r.t. center frequency and group delay.}
This iterative approach is not optimal since the $i$-th FDE channel will also affect the residual SI channel response from the $(i-1)$-th iteration, $\ResSIChnlTFvec{i-1}(f)$. 

% \memoTC{Talk about the monotonicity property of the FDE transfer function w.r.t. center frequency and group delay.}


==> tex/removed_BPF.tex <==

Since the core of our implementation is the reconfigurable RF bandpass filters (BPFs), we give a detailed description of both the BPF model and the implementation using discrete components.

As depicted in Fig.[CONCEPT], the implemented RF canceller includes two filter paths, each of which is implemented using off-the-shelf components and consists of a BPF, an attenuator, and a phase shifter. We implement the BPF as an LC filter on a printed-circuit board (PCB), whose diagram is depicted in Fig.[DIAGRAM]. When compared to the N-path filter which consumes certain amount of DC power used in our integrated FD radio in [CITE JIN JSSC'15], a discrete-component-based passive LC BPF has zero DC power consumption.

\memoTC{say something like our non-optimized BPF implementation using off-the-shelf components is around 2cm x 4cm per BPF, but the implementation is scalable to >2 SIC channels as the expense of increasing tuning complexity and power consumption?}

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\includegraphics[width=0.8\columnwidth]{./figs/diagram/CancellerSchematic.png}
\vspace{-0.5\baselineskip}
\caption{Block diagram of te FDE-based RF canceller and the LC bandpass filger (BPF) using discrete components on a PCB. \memoTC{Need to update the schematic}}
\label{fig:FDE-schematic}
\vspace{-\baselineskip}
\end{figure}
%%


%%
%% - implementation of BPF
\subsection{BPF Implementation}
\memoTC{Mahmood - please write some more details about why the impedance matching networks are important...}
The LC BPF is optimized around $\SI{875}{MHz}$ operation frequency. The quality factor of th BPF is determined by its source and load impedance. In order to achieve high quality factors, impedance transforming networks including transmission lines (TLs) and digitally tunable capacitors ($C_{2}$ and $C_{3}$) are used. Due to the symmetry of the BPF, we set $C_{2}=C_{3}$. By controlling the tunable capacitors inside the impedance transformation networks, the BPF quality factor can be adjusted. Then center frequency of the BPF can be adjusted through the digitally tunable capacitor ($C_{1}$) in the middle LC filter.

%%
%% - modeling the BPF
\subsection{Modeling the BPF}
\memoTC{The details below can probably go into the appendix to avoid confusing the readers.}
In order to understand the performance of the BPF, a solid mathematical model is needed. We first derive the transfer function (TF) $\BPFTF(j\omega)$ using transmission (ABCD) matrix theory.\footnote{We use subscripts $A$, $B$, $C$, and $D$ to denote the entries in the $2 \times 2$ matrix.}
%%
\begin{align}
\begin{bmatrix}
V_{\rm in} \\ I_{\rm in}
\end{bmatrix}
& =
\begin{bmatrix}
1 & 0 \\ Y_{2} & 1
\end{bmatrix}
\mathbf{M}^{\rm TL}(j\omega)
\begin{bmatrix}
1 & 0 \\ Y_{1} & 1
\end{bmatrix}
\mathbf{M}^{\rm TL}(j\omega)
\begin{bmatrix}
1 & 0 \\ Y_{3} & 1
\end{bmatrix}
\begin{bmatrix}
V_{\rm out} \\ I_{\rm out}
\end{bmatrix}
\\
& \triangleq
\begin{bmatrix}
M_{A}^{\rm BPF}(j\omega) & M_{B}^{\rm BPF}(j\omega) \\
M_{B}^{\rm BPF}(j\omega) & M_{D}^{\rm BPF}(j\omega)
\end{bmatrix}
\begin{bmatrix}
V_{\rm out} \\ I_{\rm out}
\end{bmatrix}
\triangleq \mathbf{M}^{\rm BPF}(j\omega)
\begin{bmatrix}
V_{\rm out} \\ I_{\rm out}
\end{bmatrix}
\end{align}
%%
in which
%%
\begin{align}
\mathbf{M}^{\rm TL}(j\omega) & = 
\begin{bmatrix}
\cos{(\beta l)} & jZ_{0}\sin{(\beta l)} \\
j\sin{(\beta l)}/Z_{0} & \cos{(\beta l)} \\
\end{bmatrix}
\triangleq
\begin{bmatrix}
a & bZ_{0} \\
b/Z_{0} & a \\
\end{bmatrix}
\end{align}
%%
is the transmission matrix of a TL with length $l$. In addition,
%%
\begin{align}
Y_{k} & = 1/R_{k} + jC_{k}\omega + \frac{1}{jL_{k}\omega},\ (k = 1,2,3)
\end{align}
%%
is the equivalent admittance parameter of the corresponding block. Therefore, the transfer function $\BPFTF(j\omega)$ is given by
%%
\begin{align}
\label{eqn:BPF-TF}
\BPFTF(j\omega) & = \frac{V_{\rm out}(j\omega)}{V_{\rm in}(j\omega)} = \frac{1}{R_{s}} \cdot \frac{V_{\rm out}(j\omega)}{I_{\rm in}(j\omega)} = \frac{1}{R_{s}} \cdot \frac{1}{M_{C}^{\rm BPF}(j\omega)} \nonumber \\
& = \frac{1}{R_{s}} \cdot \big[ a^2Y_1 + 2(a^2+b^2)Y_2 + abZ_0(2Y_1Y_2+Y_2^2) \nonumber \\
& \qquad\qquad + b^2Y_1Y_2^2Z_0^2 + 2ab/Z_{0} \big]^{-1}
\end{align}
%%
and the corresponding magnitude response, phase response, and group delay of the BPF is given by
%%
\begin{align}
|\BPFTF(j\omega)| & = R_{s}^{-1} |M_{C}^{\rm BPF}(j\omega)|^{-1}, \\ \angle\BPFTF(j\omega) & = \angle (1 / M_{C}^{\rm BPF}(j\omega) ), \\
\textrm{GD}(\BPFTF(j\omega)) & = - \partial \angle\BPFTF(j\omega) / \partial \omega
\end{align}
%%
Note that a much more accurate model can also be derived by considering all the extra transmission lines existing in the actual implementation. However, as we will show in the validation section below, this model already provides a very good accuracy when modeling the magnitude, phase, and group delay of the BPF.


%%
%% - model validation
\subsection{BPF Model Validation}
We use experimental measurements to verify the BPF model derived above. We measure the S-Parameters (SPs) on the implemented BPF (see Fig.[BPF TEST STRUCTURE]) across a $\SI{100}{MHz}$ bandwidth around the $\SI{875}{MHz}$ center frequency, with a step size of $\SI{0.2}{MHz}$ (e.g., $500$ measurement points). The measurements are conducted using different digitally programmed $C_{1}$ and $C_{2} (= C_{3})$ values. Because of practical and possible implementation losses, we use multi-dimensional curve-fitting to find the best values of $L_{1} = \SI{1.85}{nH}$ and $L_{2} = \SI{3.28}{nH}$.

We evaluate the derived BPF model {\eqref{eqn:BPF-TF}} at both the highest and lowest tunable BPF quality factor by setting $C_{2} = C_{2}^{\rm min} (= C_{3}^{\rm min})$ and $C_{2} = C_{2}^{\rm max} (= C_{3}^{\rm max})$, respectively. Figs.~\ref{fig:BPF-model-C2min} and~\ref{fig:BPF-model-C2max} present both the magnitude and phase responses in {\eqref{eqn:BPF-TF}} from measurements (solid lines) and the model. As suggested by the figures, our model matches with the measurement results very well with high BPF quality factor. In particular, across the $\SI{100}{MHz}$ bandwidth of interest, the maximum differences of the measured and modeled magnitude and phase responses are $\SI{0.5}{dB}$ (an equivalent modeling error of $5.9\%$) and $\SI{7}{deg}$.

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat[]{
\label{fig:BPF-model-mag-C2min}
\includegraphics[width=0.33\columnwidth]{./figs/BPF_model_mag_fixed_C2min.eps}
}
\hspace{-18pt} \hfill
\subfloat[]{
\label{fig:BPF-model-ph-C2min}
\includegraphics[width=0.33\columnwidth]{./figs/BPF_model_ph_fixed_C2min.eps}
}
\hspace{-18pt} \hfill
\subfloat[]{
\label{fig:BPF-model-gd-C2min}
\includegraphics[width=0.33\columnwidth]{./figs/BPF_model_gd_fixed_C2min.eps}
}
\vspace{-0.5\baselineskip}
\caption{Measured and modeled (a) magnitude, (b) phase, and (c) group delay of the BPF with impedance transformation network, $|\BPFTF(j\omega)|$, with $C_{2} = C_{2}^{\rm min}$ (highest BPF quality factor).}
\label{fig:BPF-model-C2min}
\vspace{-\baselineskip}
\end{figure}
%%

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat[]{
\label{fig:BPF-model-mag-C2max}
\includegraphics[width=0.33\columnwidth]{./figs/BPF_model_mag_fixed_C2max.eps}
}
\hspace{-18pt} \hfill
\subfloat[]{
\label{fig:BPF-model-ph-C2max}
\includegraphics[width=0.33\columnwidth]{./figs/BPF_model_ph_fixed_C2max.eps}
}
\hspace{-18pt} \hfill
\subfloat[]{
\label{fig:BPF-model-gd-C2max}
\includegraphics[width=0.33\columnwidth]{./figs/BPF_model_gd_fixed_C2max.eps}
}
\vspace{-0.5\baselineskip}
\caption{Measured and modeled (a) magnitude, (b) phase, and (c) group delay of the BPF with impedance transformation network, $|\BPFTF(j\omega)|$, with $C_{2} = C_{2}^{\rm max}$ (lowest BPF quality factor).}
\label{fig:BPF-model-C2max}
\vspace{-\baselineskip}
\end{figure}
%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/removed_eval_pcb.tex <==
%%
%%
We now experimentally evaluate the PCB canceller performance based on the realistic model {\eqref{eq:pcb-tf-calibrated}} described in Section~\ref{ssec:impl-pcb}. We first perform measurements to validate both the PCB BPF {\eqref{eq:pcb-bpf-tf}} and the PCB canceller {\eqref{eq:pcb-tf-calibrated}} models. Then, we perform system-level evaluation of our FD radio design with optimized PCB canceller configuration in an SDR testbed. We also perform model-based evaluation of the PCB canceller with a larger number of FDE taps, $\NumTap$.

%%%%%
%%%%%
\subsection{Validation of PCB Canceller}
\label{ssec:eval-pcb-validation}

\subsubsection{Validation of the PCB BPF}
We first validate the PCB BPF model, $\BPFTapTF{i}(f_k)$, given by {\eqref{eq:pcb-bpf-tf}}, where the ground truth is obtained by measuring the S-Parameters of the PCB BPF using a test structure (see Fig.~\ref{fig:diagram-pcb}) to avoid the effects of other components on the PCB. The measurements are conducted with varying programmed values of $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ and the results are averaged over $20$ measurements.\footnote{We drop the subscript of $i$ since both PCB BPFs behave identically.}
% Due to practical implementation losses, we use multi-dimensional curve-fitting to better tune parameters $L_1 = \SI{1.85}{nH}$ and $L_2 = \SI{3.28}{nH}$ (see Fig.~\ref{fig:impl-fde}).

Fig.~\ref{fig:eval-pcb-bpf} presents the amplitude and phase of the PCB BPF using both measurements and the model {\eqref{eq:pcb-bpf-tf}} with $4$ sets of selected $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ as indicated in Table~\ref{table:set-cap} covering the entire tuning range of the BPF center frequency and quality factor. We consider both the highest and lowest achievable BPF quality factors by respectively setting $\PCBTapQFCapNoidx = \PCBTapQFCapMin$ and $\PCBTapQFCapNoidx = \PCBTapQFCapMax$ (see Section~\ref{ssec:impl-pcb}). The measured PCB BPF quality factor has a tuning range between $9.2$ and $17.8$. Comparing to the \emph{fixed} quality factor of $2.7$ achieved by using only the $RLC$ resonance tank, introducing the impedance transformation networks provides improves the quality factor tuning range by $3.4 - 6.6\times$. In addition, the PCB BPF has a center frequency tuning range of $\SI{18}{MHz}$. Fig.~\ref{fig:eval-pcb-bpf} shows that the PCB BPF model {\eqref{eq:pcb-bpf-tf}} matches very closely with the measurement results at high BPF quality factor value (top row). In particular, the maximum differences between the measured and modeled amplitude and phase are $\SI{0.5}{dB}$ ($5.9\%$) and $\SI{7}{deg}$, respectively. At the lowest BPF quality factor value (bottom row), these errors increase to $\SI{1.2}{dB}$ ($14.8\%$) and $\SI{15}{deg}$, while still validating the PCB BPF model. The measurements are repeated for different values of $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ within their configuration ranges and the same level of accuracy of the model {\eqref{eq:pcb-bpf-tf}} is observed.

%%
\begin{figure}[!t]
\centering
\subfloat{
\label{fig:eval-pcb-bpf-amp}
\includegraphics[width=0.45\columnwidth]{./figs/model/model_bpf_amp.eps}
}
\hspace{6pt}
\subfloat{
\label{fig:eval-pcb-bpf-phase}
\includegraphics[width=0.45\columnwidth]{./figs/model/model_bpf_phase.eps}
}
\caption{Measured and modeled amplitude and phase of the implemented PCB BPF without amplitude and phase controls under different $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ as indicated in Table~\ref{table:set-cap}.}
\label{fig:eval-pcb-bpf}
\end{figure}
%%

%% begin of table
\begin{table}[!t]
\caption{Selected sets of parameters $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$}
\label{table:set-cap}
\vspace{-\baselineskip}
\footnotesize
\begin{center}
% \begin{tabular}{| p{0.1\columnwidth} | p{0.2\columnwidth} | p{0.1\columnwidth} | p{0.2\columnwidth} |}
\begin{tabular}{|c|c|c|}
\hline
& High Q-Factor & Low Q-Factor \\
\hline
High Center Freq. & Set 1: $(\PCBTapCFCapMin, \PCBTapQFCapMin)$ & Set 3: $(\PCBTapCFCapMin, \PCBTapQFCapMax)$ \\
\hline
Low Center Freq. & Set 2: $(\PCBTapCFCapMax, \PCBTapQFCapMin)$ & Set 4: $(\PCBTapCFCapMax, \PCBTapQFCapMax)$ \\
\hline
\end{tabular}
\end{center}
\vspace{-1\baselineskip}
\end{table}
%% end of table


%%
%%
\subsubsection{Validation of the PCB Canceller}
We now turn to the validation of the PCB canceller model, $\PCBTF(f_k)$, given by {\eqref{eq:pcb-tf-calibrated}} with two FDE taps. Note that the attenuators used have a maximal attenuation value of only $\SI{16}{dB}$ (see Section~\ref{ssec:impl-pcb}) and even at this maximal attenuation, signals can still leak through the FDE tap, resulting in inseparable behaviors between the two FDE taps.

In order to validate the PCB canceller model {\eqref{eq:pcb-tf-calibrated}}, we measure the frequency response of the PCB canceller by setting the first FDE tap at its highest amplitude (i.e., lowest attenuation value of $\PCBTapAmp{1}$) with varying values of $(\PCBTapCFCap{1}, \PCBTapQFCap{1})$ while setting the second FDE tap with the highest attenuation value $\PCBTapAmp{2}$ (e.g., to minimize the effect of the second FDE tap). Fig.~\ref{fig:eval-pcb} shows the amplitude and phase of the PCB canceller using measurements and the model {\eqref{eq:pcb-tf-calibrated}} in such a setting. We obtain similar behaviors results when turning on only the second FDE tap. We then repeat the measurements by setting different values of $\{\PCBTapAmp{i}, \PCBTapPhase{i}, \PCBTapCFCap{i}, \PCBTapQFCap{i}\}$, and the all the measurements validate the PCB canceller model {\eqref{eq:pcb-tf-calibrated}}.


%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-pcb-amp}
\includegraphics[width=0.45\columnwidth]{./figs/model/model_fde_amp.eps}
}
\hspace{6pt}
\subfloat{
\label{fig:eval-pcb-phase}
\includegraphics[width=0.45\columnwidth]{./figs/model/model_fde_phase.eps}
}
\caption{Measured and modeled amplitude and phase of the PCB canceller with one FDE tap on and the other tap at minimal amplitude under different $(\PCBTapCFCapNoidx, \PCBTapQFCapNoidx)$ as indicated in Table~\ref{table:set-cap}.}
\label{fig:eval-pcb}
\end{figure}
%%




%%%%%
%%%%% BEGINNING OF EXP

\subsection{Experimental Evaluation}
\label{ssec:eval-pcb-exp}

After validating the PCB canceller model {\eqref{eq:pcb-tf-calibrated}}, we experimentally evaluate its performance with optimized canceller configuration (see Section~\ref{ssec:algo-opt}) in an SDR testbed.

%%
% \begin{figure}[!t]
% \centering
% \includegraphics[width=\columnwidth]{./figs/exp/exp_labview.png}
% \vspace{-0.5\baselineskip}
% \caption{The implemented full-duplex radio prototype consisting on an antenna, a circulator, an FDE canceller with two FDE taps, and a USRP SDR.}
% \label{fig:impl-fd-radio}
% \vspace{-\baselineskip}
% \end{figure}
%%

\subsubsection{SDR Testbed}
Figs.~\ref{fig:intro}\subref{fig:intro-fd-radio} and~\ref{fig:intro}\subref{fig:intro-fd-link} depict our FD radio design and the testbed. We use the NI USRP-2942 SDR with carrier frequency at $\SI{900}{MHz}$, which is the same as the operating frequency of the antenna, the circulator, and the PCB canceller. As described in Section~\ref{ssec:impl-pcb}, our FDE-based canceller design can be easily extended to other operating frequencies. We implemented a full OFDM-based WiFi- (802.11a/g-) like PHY layer
% \footnote{Since our FDE-based RF canceller was designed around $\SI{900}{MHz}$ we shift the WiFi-like OFDM PHY to be centered at the same operating frequency.}
with a maximal real-time RF bandwidth of $\SI{20}{MHz}$. The OFDM symbol size is $64$ samples (subcarriers) with a cyclic-prefix ratio of $0.25$ ($16$ samples). The OFDM PHY layer supports constellations from BPSK to $64$-QAM with coding rates of $1/2$, $2/3$, and $3/4$. The baseband complex (IQ) samples are streamed between the USRP-2942 and the host PC through a high-speed PCI-Express interface. The optimization of the PCB canceller is implemented on the host PC and the canceller is configured via a SUB-20 controller. The digital SIC algorithm is also implemented on the host PC to further suppress the residual SI signal after RF SIC, where we set the highest non-linearity order to be $7$.\footnote{The digital SIC algorithm is based on Volterra series and a least-square problem, which is similar to that presented in~\cite{bharadia2013full}. We omit the details here due to limited space.}


%%
%%
\subsubsection{Evaluation of RF SIC and the Optimized Canceller Configuration}
To perform the PCB canceller configuration optimization, the antenna interface response, $\AntTF(f_k)$, is first measured using two long training symbols (LTSs) as specified in the 802.11a/g standards. In particular, $\AntTF(f_k)$ is computed by dividing the received LTS symbols by the known transmitted LTS in the frequency domain. Then, the computed (complex) values of $\AntTF(f_k)$ and the PCB canceller model {\eqref{eq:pcb-tf-calibrated}} are used for obtaining the PCB canceller configuration, where $\OptProblemPCB$ is first solved by a non-linear optimization solver to obtain an initial PCB canceller configuration (see Section~\ref{ssec:algo-opt}), followed by a finer-grained, fast local search to achieve the true-optimal RF SIC performance. In our design, a non-optimized solver can return the solution to $\OptProblemPCB$ in less than $\SI{10}{ms}$, where the PCB canceller model {\eqref{eq:pcb-tf-calibrated}} is pre-computed and stored for computational efficiency. Note that this is only a $1\%$ overhead is the PCB canceller needs to be tuned once every second.

\textbf{FDE Canceller Model and Configuration}.
Fig.~\ref{fig:exp-usrp-algo} shows the process of PCB canceller configuration in our FD radio design.
% As Fig.~\ref{fig:exp-usrp-algo} suggests, with the returned PCB canceller configuration obtained by solving $\OptProblemPCB$, the PCB canceller has a similar frequency response in practice (obtained through measurements) when compared to that predicted by the model {\eqref{eq:pcb-tf-calibrated}}.
As Fig.~\ref{fig:exp-usrp-algo} suggests, with the canceller model {\eqref{eq:pcb-tf-calibrated}} and the configuration obtained by solving $\OptProblemPCB$, the PCB canceller closely matches with $\AntTF(f_k)$ with only less than $\SI{0.5}{dB}$ and $\SI{2.5}{deg}$ differences in amplitude and phase, respectively. This confirms both the accuracy of the PCB canceller model and the efficiency of the canceller configuration. Throughout out experiments, an average $\SI{52}{dB}$ RF SIC is achieved across $\SI{20}{MHz}$ bandwidth, from which $\SI{20}{dB}$ comes from the antenna interface isolation.

\textbf{Overall SIC}.
Fig.~\ref{fig:eval-usrp-spec-20mhz} presents the overall SIC achieved by our FD radio design, where the USRP has a measured noise floor of $-\SI{85}{dBm}$ at a fixed receiver gain.\footnote{This USRP receiver noise floor is limited by the environmental interference at $\SI{900}{MHz}$ frequency. The USRP has a true noise floor of around $-\SI{95}{dBm}$ at the same receiver gain setting, when not connected to an antenna.} An average $\SI{95}{dB}$ overall SIC is achieved in our experiments, from which $\SI{52}{dB}$ is obtained at RF through the antenna isolation and the PCB canceller, and $\SI{43}{dB}$ is obtained by the digital SIC. Therefore, an average TX power of up to $\SI{10}{dBm}$ can be supported. Note that in this case, the \emph{peak} TX power can go as high as $\SI{20}{dBm}$. We also believe that by adding more FDE taps and optimizing the PCB canceller implementation have the potential to further enhance the performance of RF SIC.


%% amplitude and phase
% \begin{figure}[!t]
% \centering
% \subfloat{
% \label{fig:exp-usrp-algo-amp}
% \includegraphics[width=0.5\columnwidth]{./figs/exp/exp_usrp_algo_amp.eps}}
% \hspace{-12pt}\hfill
% \subfloat{
% \label{fig:exp-usrp-algo-phase}
% \includegraphics[width=0.5\columnwidth]{./figs/exp/exp_usrp_algo_phase.eps}}
% \vspace{-0.5\baselineskip}
% \caption{Performance the PCB canceller configuration optimization based on real-time antenna interface measurements. The canceller model {\eqref{eq:pcb-tf-calibrated}} accurately follows the SI channel response with amplitude and phase errors of less than $\SI{0.5}{dB}$ and $\SI{2.5}{deg}$.}
% \label{fig:exp-usrp-algo}
% \vspace{-\baselineskip}
% \end{figure}
%%

%% amplitude and phase
\begin{figure}[!t]
\centering
\subfloat{
\label{fig:exp-usrp-algo-phase}
\includegraphics[width=0.45\columnwidth]{./figs/exp/exp_usrp_algo_iq.eps}}
\hspace{6pt}
\subfloat{
\label{fig:exp-usrp-algo-amp}
\includegraphics[width=0.45\columnwidth]{./figs/exp/exp_usrp_algo_res.eps}}
\caption{(Left) Optimized PCB canceller configuration based on real-time SI channel measurements, and (right) the measured and modeled RX signal after RF SIC. The accurate PCB canceller model {\eqref{eq:pcb-tf-calibrated}} results in an average $\SI{52}{dB}$ RF SIC across $\SI{20}{MHz}$.}
\label{fig:exp-usrp-algo}
\end{figure}
%%

%%
\begin{figure}[!t]
\centering
% \includegraphics[width=0.9\columnwidth]{./figs/exp/exp_usrp_spec_20mhz_annotated.eps}
\includegraphics[width=0.6\columnwidth]{./figs/exp/exp_usrp_sic.eps}
\caption{Power spectrum of the received signal after RF and digital SIC with $\SI{10}{dBm}$ average TX power and $-\SI{85}{dBm}$ RX noise floor. \memoTC{put a node picture on the side?}}
\label{fig:eval-usrp-spec-20mhz}
\end{figure}
%%





%% FD gain

%%
% \begin{figure}[!t]
% \centering
% \vspace{-\baselineskip}
% \subfloat{
% \label{fig:eval-pcb-fd-gain-0dbm}
% \includegraphics[width=0.4\columnwidth]{./figs/exp/exp_fd_gain_0dbm_annotated.eps}
% }
% % \hspace{-6pt} \hfill
% \subfloat{
% \label{fig:eval-pcb-fd-gain-10dbm}
% \includegraphics[width=0.4\columnwidth]{./figs/exp/exp_fd_gain_10dbm_annotated.eps}
% }
% \vspace{-0.5\baselineskip}
% \caption{CDF of an FD link throughput when operating in HD and FD mode with $\SI{0}{dBm}$ and $\SI{10}{dBm}$ average TX power. The medians of FD throughput gain are $1.77\times$ and $1.81\times$, respectively.}
% \label{fig:eval-pcb-fd-gain}
% \vspace{-\baselineskip}
% \end{figure}
%%


%%
\begin{figure*}[!t]
\centering
\subfloat{
\label{fig:eval-pcb-snr-loss-err}
\includegraphics[width=0.8\columnwidth]{./figs/exp/link/snr_loss_pos_map.jpg}
}
\hspace{6pt}
\subfloat{
\label{fig:eval-pcb-snr-loss-cdf}
\includegraphics[width=0.5\columnwidth]{./figs/exp/link/snr_loss_vs_dist_err.eps}
}
\hspace{6pt}
\subfloat{
\label{fig:eval-pcb-snr-loss-cdf}
\includegraphics[width=0.5\columnwidth]{./figs/exp/link/fd_gain_vs_dist_cdf.eps}
}
\caption{(Left) Floor plan for the FD/HD link SNR measurements, (middle) SNR loss with varying HD link SNR values, and (right) CDF of FD throughput gain with varying HD link SNR values with $\SI{0}{dBm}$ average TX power, 64QAM constellation, and $\SI{20}{MHz}$ bandwidth.}
\label{fig:eval-pcb-snr-loss}
\end{figure*}
%%




%%
\begin{figure}[!t]
\centering
\subfloat{
\label{fig:eval-pcb-snr-loss-err}
\includegraphics[width=0.45\columnwidth]{./figs/exp/link/snr_loss_vs_mod_cdf.eps}
}
\hspace{6pt}
\subfloat{
\label{fig:eval-pcb-snr-loss-cdf}
\includegraphics[width=0.45\columnwidth]{./figs/exp/link/snr_loss_vs_mod_err.eps}
}
\caption{(Left) CDF of SNR loss, and (right) SNR loss in FD mode with different modulation schemes at $\SI{10}{dBm}$ average TX power.}
\label{fig:eval-pcb-snr-loss}
\end{figure}
%%



%%
%%
\subsubsection{Evaluation of FD Gain}
\label{ssec:eval-pcb-model-based-sim}
We also experimentally evaluate the (PHY layer) throughput gain achieved by our FD radio design compared to that when it operates in HD mode. The experiments are conducted as follows. We set up a wireless link with two FD radios that send a sequence $1000$ WiFi packets in both FD mode and HD mode. We set an FD radio to operate in HD mode by turning on only its transmitter or receiver, since we would like to evaluate it performance with the existence of the circulator and PCB canceller. We repeat the experiments in a lab environment with regular furniture and cycle through all modulation schemes at average TX power levels of $\SI{0}{dBm}$ and $\SI{10}{dBm}$. The \emph{link signal-to-noise ratio (SNR)} is then computed as the ratio between the RX signal power level and the USRP receiver noise floor ($-\SI{85}{dBm}$).

Fig.~\ref{fig:eval-pcb-fd-gain} presents the CDF of the experimental link throughput when two FD radios operate in HD mode and FD mode with $\SI{0}{dBm}$ and $\SI{10}{dBm}$ average TX power. The measured link SNR in all cases varies between $0$-$\SI{15}{dB}$. Fig.~\ref{fig:eval-pcb-fd-gain} shows that medians of experimental FD throughput gains are $1.77\times$ for $\SI{0}{dBm}$ TX power level and $1.81\times$ for $\SI{10}{dBm}$ TX power level, respectively. This slightly differs from the a theoretical FD gain of $2\times$ due to the minimal (around $\SI{1}{dB}$) loss in the link SNR when the radios operate in FD mode.



%%%%% END OF EXP
%%%%%




%%
%%
\subsection{Model-based Evaluation}

Since the PCB canceller only has $2$ FDE taps and the USRP can only operate at a maximal bandwidth of $\SI{20}{MHz}$, we also perform model-based simulation to evaluate the performance of a PCB canceller with varying number of FDE taps and desired RF SIC bandwidth, using the validated PCB canceller model {\eqref{eq:pcb-tf-calibrated}}.

The evaluation is performed using the same approach as described in Section~\ref{sec:eval-rfic}. Fig.~\ref{fig:eval-pcb} presents the RF SIC of the PCB canceller with $\NumTap \in \{2,4\}$ and $\{40,80\}\thinspace\SI{}{MHz}$. We consider both cases with and without the quantization constraints, which come from the PCB canceller implementation described in Section~\ref{ssec:impl-pcb}. As Fig.~\ref{fig:eval-pcb-sim} illustrates, the PCB canceller with $2$ FDE taps can still achieve an average amount of $\SI{40}{dB}$ and $\SI{35}{dB}$ RF SIC across $\SI{40}{MHz}$ and $\SI{80}{MHz}$ bandwidths, even under practical quantization constraints. Moreover, a PCB canceller of $4$ taps has the potential to achieve $\SI{65}{dB}$ and $\SI{50}{dB}$ RF SIC across $\SI{40}{MHz}$ and $\SI{80}{MHz}$, respectively. Therefore, we believe that the RF SIC performance can be further enhanced for the PCB canceller if more FDE taps are included.

%%
\begin{figure}[!t]
\centering
\subfloat{
\label{fig:eval-pcb-sim-bw-40mhz}
\includegraphics[width=0.45\columnwidth]{./figs/sim/sim_pcb_bw_40mhz.eps}
}
\hspace{6pt}
\subfloat{
\label{fig:eval-pcb-sim-bw-80mhz}
\includegraphics[width=0.45\columnwidth]{./figs/sim/sim_pcb_bw_80mhz.eps}
}
\caption{TX/RX isolation of the antenna interface and with the PCB canceller with varying number of FDE taps, $\NumTap \in \{2,4\}$, and desired RF SIC bandwidth of $\{40,80\}\thinspace\SI{}{MHz}$.}
\label{fig:eval-pcb-sim}
\end{figure}
%%




%%
%%
\subsection{Throughput Gain in Heterogeneous Networks}
Now we turn to the evaluation of the network throughput gain with varying number of FD and HD users. Due to the software limitations, it is challenging to implement a full MAC layer. However, we can still evaluate the throughput gain in such heterogeneous networks using a simple TDD MAC layer where every node (FD or HD) takes turn and performs transmission and/or reception.

\textbf{Setup}. We consider a network consisting of one FD AP, $2$ FD users\footnote{We are limited by the number of FDE cancellers fabricated.}, and $2$ HD users, where the users are placed as different locations in a lab environment.

%%
\begin{figure}[!t]
\centering
\subfloat{
\label{fig:eval-pcb-snr-loss-err}
\includegraphics[width=0.45\columnwidth]{./figs/exp/net/exp_two_users_net_tput.eps}
}
\hspace{6pt}
\subfloat{
\label{fig:eval-pcb-snr-loss-cdf}
\includegraphics[width=0.45\columnwidth]{./figs/exp/net/exp_two_users_fairness.eps}
}
\caption{Throughput and fairness of a 2-user network.}
\label{fig:eval-pcb-snr-loss}
\end{figure}
%%



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/removed_exp.tex <==
In this section, we experimentally evaluate the performance of both the PCB RF SI canceller with $\NumTap=2$ FDE taps and the proposed tuning algorithm. 

%%
%%
\subsection{SDR Platform and Testbed}
\label{ssec:exp-setup}

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\includegraphics[width=0.6\columnwidth]{./figs/eval/impl_fd_radio.png}
\vspace{-0.5\baselineskip}
\caption{The implemented full-duplex radio prototype consisting on an antenna, a circulator, an FDE canceller with two FDE taps, and a USRP SDR.}
\label{fig:impl-fd-radio}
\vspace{-\baselineskip}
\end{figure}
%%

Fig.~\ref{fig:impl-fd-radio} shows our implemented single-antenna full-duplex radio prototype equipped with the FDE-based PCB RF SI canceller described in Section~\ref{ssec:model-pcb}.

We use the NI USRP-2942 software defined radio platform with carrier frequency set to be $\SI{900}{MHz}$.\memoTC{mention that can also work at other frequencies.} We implemented a full OFDM-based WiFi-like PHY layer\footnote{Since our FDE-based RF canceller was designed around $\SI{900}{MHz}$ we shift the WiFi-like OFDM PHY to be centered at the same operating frequency.} that can be configured to operate at a maximal $\SI{20}{MHz}$ RF real-time bandwidth. The OFDM symbol size is set to be $64$ samples (subcarriers) with a cyclic-prefix ratio of $0.25$ (i.e., $16$ samples). We support constellations from BPSK to $64$-QAM with coding rates of $1/2$, $2/3$, and $3/4$. The baseband complex (IQ) samples are streamed between the host PC and the USRP-2942 through a PCI-e interface. The tuning algorithm is implemented on the host PC and the PCB canceller is configured through a SUB-20 controller. A digital SIC algorithm based on Volterra series and a least-square problem (similar to that in~\cite{bharadia2013full}) is also implemented on the host PC, where we set the highest non-linearity order to be $7$.


%%
%%
\subsection{SI Channel Measurements and Tuning Algorithm Implementation}
In our experiments, the frequency domain response of the SI channel, $\SIChnlTF(f)$, is measured using the two long training frames (LTFs) in the 802.11a/b/g standards, each of which contains one OFDM consisting of $64$ samples in the frequency domain. In particular, the (complex) SI channel response is obtained by dividing the received LTF symbols on the $52$ data subcarriers by the known transmitted symbols. This SI channel response is then passed into the tuning algorithm, where Algorithm~\ref{algo:opt-joint} is first used to compute an initial near-optimal canceller configurations followed by a finer-grained local search to achieve the optimal RF SIC performance.

Fig.~\ref{fig:exp-usrp-algo} shows an example of the measured SI channel response across $52$ OFDM subcarriers and the simulated and experimental RF SIC, respectively. The inherent delay introduce by USRP is calibrated out and the measure SI channel group delay is around $\SI{10}{ns}$. As Fig.~\ref{fig:exp-usrp-algo} illustrates, the configurations returned by the algorithm and a simple local search generate a PCB canceller response that is very close to the SI channel response, resulting in an average amount of $\SI{50}{dB}$ RF SIC across the considered bandwidth.


%%
%%
\subsection{RF SIC Evaluation}

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\includegraphics[width=0.49\columnwidth]{./figs/eval/eval_usrp_algo_amp.eps}}
\hspace{-6pt}\hfill
\subfloat{
\includegraphics[width=0.49\columnwidth]{./figs/eval/eval_usrp_algo_phase.eps}}
% \hspace{-6pt}\hfill
% \subfloat{
% \includegraphics[width=0.33\columnwidth]{./figs/eval/eval_usrp_algo_gd.eps}}
\vspace{-0.5\baselineskip}
\caption{An example of the FDE canceller configurations returned by the joint optimization algorithm based on SI channel response measured by USRP on the OFDM channels ($52$ data subcarriers and $1$ null-subcarrier spanning $\SI{16.6}{MHz}$ occupied bandwidth) and the developed realistic FDE canceller model. }
\label{fig:exp-usrp-algo}
\vspace{-\baselineskip}
\end{figure}
%%

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\includegraphics[width=0.8\columnwidth]{./figs/eval/eval_usrp_spec_20mhz.eps}
\vspace{-0.5\baselineskip}
\caption{Power spectrum of the transmitted signal and the received signal after RF and digital SIC, respectively, from which $\SI{50}{dB}$ RF SIC is achieved across $\SI{20}{MHz}$ RF bandwidth. A total amount of $\SI{95}{dB}$ SIC is achieved across the antenna, RF, and digital domains, supporting $+\SI{10}{dBm}$ average TX power level and $-\SI{85}{dBm}$ receiver noise floor.}
\label{fig:eval-usrp-spec-20mhz}
\vspace{-\baselineskip}
\end{figure}
%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/removed_impl.tex <==
In this section, we describe the detailed implementation of our FDE-based RF SI canceller using reconfigurable BPFs with amplitude and phase control. Then, we present the mathematical model of the discrete-component-based implementation, which is used for the tuning algorithm.

%%
%% - implementation of BPF
\subsection{FDE/BPF Implementation}
\memoTC{Mahmood - please write some more details about why the impedance matching networks are important... Also talk about power divider/combiner and couplers. For the diagram, please put $C_1$ in the middle LC tank and the same $C_2$ in the impedance tuning networks.}

As depicted in Fig.[CONCEPT], the implemented FDE-based RF SI canceller includes two FDE taps, each of which is implemented using off-the-shelf components and consists of a BPF, a programmable attenuator, and a programmable phase shifter. The BPF is implemented as an LC filter on a printed-circuit board (PCB), whose diagram is depicted in Fig.[DIAGRAM]. When compared to the N-path filter which consumes certain amount of DC power used in our integrated FD radio in [CITE JIN JSSC'15], a discrete-component-based passive LC BPF has zero DC power consumption.
\memoTC{say something like our non-optimized BPF implementation using off-the-shelf components is around 2cm x 4cm per BPF, but the implementation is scalable to >2 SIC channels at the expense of increasing tuning complexity and power consumption?}

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat[]{
\label{fig:impl-fde-diagram}
\includegraphics[width=0.48\columnwidth]{./figs/diagram/CancellerSchematic.png}
}
\hspace{-6pt} \hfill
\subfloat[]{
\label{fig:impl-fde-canc}
\includegraphics[width=0.48\columnwidth]{./figs/eval/impl_fde_canc.png}
}
\vspace{-0.5\baselineskip}
\caption{The implemented FDE-based RF SI canceller containing two FDE taps: (a) block diagram, and (b) circuit implementation using using discrete components on a printed circuit board. \memoTC{Mahmood - Need to update the diagram figure.}}
\label{fig:impl-fde}
\vspace{-\baselineskip}
\end{figure}
%%

The LC BPF is optimized around $\SI{900}{MHz}$ operating frequency.\footnote{In this implementation, we select $\SI{900}{MHz}$ operating frequency \memoTC{WHY} but this approached can be easily extended to other frequencies (e.g., at $\SI{2.4/5}{GHz}$).} The center frequency of the BPF can be adjusted through the digitally tunable capacitor ($C_{1}$) in the middle LC filter. The quality factor of the BPF is determined by its source and load impedance. In order to achieve high quality factors, impedance transforming networks including transmission lines (TLs) and digitally tunable capacitors ($C_{2}$) are used. By controlling the tunable capacitors inside the impedance transformation networks, the BPF quality factor can be adjusted.


%%
%% - modeling the BPF
\subsection{Modeling the BPF}
\memoTC{Some of the math details below can probably go into the appendix to avoid confusing the readers...}
In practical implementations \memoTC{or efficient/good implementations?}, the center frequency, $\CenterFreq{i}$, and the quality factor, $\QFactor{i}$, in the $i$-th ideal FDE tap (see {\eqref{eq:fde-tap-tf}}) \emph{can not be tuned directly}. As described before, $\CenterFreq{i}$ and $\QFactor{i}$ are adjusted through the digitally tunable capacitor, $C_1$ and $C_2$ (see [FIG DIAGRAM]). In order to understand the relationship between the values of $C_1$ and $C_2$ and the resultant center frequency and quality factor, a solid mathematical model is needed. This is essential for efficient and practical tuning algorithms on realistic hardware. We first derive the transfer function (TF) $\BPFTF(j\omega)$ using transmission (ABCD) matrix theory.\footnote{We use subscripts $A$, $B$, $C$, and $D$ to denote the entries in the $2 \times 2$ matrix.}
%%
\begin{align}
\begin{bmatrix}
V_{\rm in} \\ I_{\rm in}
\end{bmatrix}
& =
\begin{bmatrix}
1 & 0 \\ Y_2 & 1
\end{bmatrix}
\mathbf{M}^{\rm TL}(f)
\begin{bmatrix}
1 & 0 \\ Y_1 & 1
\end{bmatrix}
\mathbf{M}^{\rm TL}(f)
\begin{bmatrix}
1 & 0 \\ Y_2 & 1
\end{bmatrix}
\begin{bmatrix}
V_{\rm out} \\ I_{\rm out}
\end{bmatrix}
\\
& \triangleq
\begin{bmatrix}
M_{A}^{\rm BPF}(f) & M_{B}^{\rm BPF}(f) \\
M_{B}^{\rm BPF}(f) & M_{D}^{\rm BPF}(f)
\end{bmatrix}
\begin{bmatrix}
V_{\rm out} \\ I_{\rm out}
\end{bmatrix}
\triangleq \mathbf{M}^{\rm BPF}(f)
\begin{bmatrix}
V_{\rm out} \\ I_{\rm out}
\end{bmatrix}
\end{align}
%%
in which
%%
\begin{align}
\mathbf{M}^{\rm TL}(f) & = 
\begin{bmatrix}
\cos{(\beta l)} & jZ_{0}\sin{(\beta l)} \\
j\sin{(\beta l)}/Z_{0} & \cos{(\beta l)} \\
\end{bmatrix}
\triangleq
\begin{bmatrix}
a & bZ_{0} \\
b/Z_{0} & a \\
\end{bmatrix}
\end{align}
%%
is the transmission matrix of a transmission line with length $l$ and \memoTC{and $\beta$ and $Z_0$ being???}, and
%%
\begin{align}
Y_k(f) & = 1/R_k + jC_k2\pi f + 1/(jL_k2\pi f),\ k = 1,2
\end{align}
%%
is the equivalent admittance of the corresponding block. Therefore, the transfer function of the implemented FDE tap, $\BPFImplTF{}(f)$, can be computed as
%%
\begin{align}
\label{eq:impl-bpf-tf}
& \BPFImplTF{}(f) = \frac{V_{\rm out}(f)}{V_{\rm in}(f)} = \frac{1}{R_s} \cdot \frac{V_{\rm out}(f)}{I_{\rm in}(f)} = \frac{1}{R_s} \cdot \frac{1}{M_C^{\rm BPF}(f)} \nonumber \\
& \quad = R_s^{-1} \Big[ a^2Y_1(f) + 2(a^2+b^2)Y_2(f) + 2abZ_02Y_1(f)Y_2(f) \nonumber \\
& \qquad + abZ_0(Y_2(f))^2 + b^2Y_1(f)(Y_2(f))^2Z_0^2 + 2ab/Z_0 \Big]^{-1},
\end{align}
%%
and the corresponding magnitude response, phase response, and group delay of the BPF is given by
%%
\begin{align}
|\BPFImplTF{}(f)| & = R_s^{-1} |M_C^{\rm BPF}(f)|^{-1}, \\
\angle\BPFImplTF{}(f) & = \angle (1 / M_C^{\rm BPF}(f) ), \\
\tau(\BPFImplTF{}(f)) & = - \frac{\partial \angle\BPFImplTF{}(f)}{\partial f}.
\end{align}
%%
Note that a much more accurate model can also be derived by considering all the extra components existing in the actual implementation. However, as we will show below, this model already provides a very good accuracy when modeling the magnitude, phase, and group delay of the BPF.


%%
%% - model the FDE tap
\subsection{Modeling the FDE Tap}
Based on the realistic BPF transfer function {\eqref{eq:impl-bpf-tf}}, one FDE tap can be then modeled by adding  amplitude and phase controls to {\eqref{eq:impl-bpf-tf}}, i.e., the transfer function of an implemented FDE tap is given by
%%
\begin{align}
\label{eq:impl-fde-tf}
\FDEImplTF{i}(f) & = \Amp{i} e^{j\Phase{i}} \cdot \BPFImplTF{i}(f),\ i=1,2.
\end{align}
%%

Due to the existence of other components before and after the FDE taps (e.g., couplers and power divider/combiner, etc.), the signals traveling on the PCB may experience some extra attenuation and group delay. By looking at the S-Parameter datasheet of each component, it is observed that the attenuation and group delay are almost constant. By adding this (small) constant attenuation and group delay into {\eqref{impl-fde-tf}}, we can get a very accurate model of an implemented FDE tap. Then, the entire FDE canceller with two FDE taps has an equivalent transfer function of $\FDEImplTF{}(f) = \FDEImplTF{1}(f) + \FDEImplTF{2}(f)$.


%%
%% - model validation
\subsection{Validating the Models}
\subsubsection{BPF Model Validation}
We first perform experimental measurements to verify the BPF model derived above. We measure the S-Parameters \memoTC{maybe transfer function?} of the implemented BPF using a test structure to avoid the effect from other components (see Fig.[BPF TEST STRUCTURE]) across a $\SI{100}{MHz}$ bandwidth from $\SI{850}{MHz}$ to $\SI{950}{MHz}$. The measurements are conducted using varying programmed values of $C_c$ and $C_Q$ and the results are averaged over $20$ measurements. Due to practical implementation losses, we use multi-dimensional curve-fitting to better tune parameters $L_1 = \SI{1.85}{nH}$ and $L_2 = \SI{3.28}{nH}$.

Fig.~\ref{impl-model-bpf} present the measured (solid lines) and modeled (using {\eqref{eq:impl-bpf-tf}}) magnitude/phase responses and group delay of the implemented BPF. We consider both the highest and lowest tunable BPF quality factor by setting $C_Q = C_Q^{\rm min}$ and $C_Q = C_Q^{\rm max}$, respectively, corresponding to a tunable range of the BPF quality factor between $9.2$ and $17.8$. As Fig.~\ref{impl-model-bpf} suggest, our BPF model {\eqref{eq:impl-bpf-tf}} matches with the measurement results very closely at high BPF quality factor values. In particular, the maximum differences between the measured and modeled magnitude and phase responses are $\SI{0.5}{dB}$ (or $5.9\%$ in linear scale) and $\SI{7}{deg}$, respectively.

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:BPF-model-mag-C2min}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_amp_vary_Cc_fixed_Cq_min.eps}
}
\hspace{-8pt} \hfill
\subfloat{
\label{fig:BPF-model-ph-C2min}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_phase_vary_Cc_fixed_Cq_min.eps}
}
\hspace{-8pt} \hfill
\subfloat{
\label{fig:BPF-model-gd-C2min}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_gd_vary_Cc_fixed_Cq_min.eps}
}
\\ \vspace{-1.5\baselineskip}
%%
\subfloat{
\label{fig:BPF-model-mag-C2max}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_amp_vary_Cc_fixed_Cq_max.eps}
}
\hspace{-8pt} \hfill
\subfloat{
\label{fig:BPF-model-ph-C2max}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_phase_vary_Cc_fixed_Cq_max.eps}
}
\hspace{-8pt} \hfill
\subfloat{
\label{fig:BPF-model-gd-C2max}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_gd_vary_Cc_fixed_Cq_max.eps}
}
%%
\vspace{-0.5\baselineskip}
\caption{Measured and modeled magnitude, phase, and group delay of the implemented bandpass filter (BPF) response, $\BPFImplTF{}(f)$, with the highest BPF quality factor, $C_Q = C_Q^{\rm min}$ (top row) and the lowest BPF quality factor, $C_Q = C_Q^{\rm max}$ (bottow row), respectively.}
\label{fig:impl-model-bpf}
\vspace{-\baselineskip}
\end{figure}
%%

%%
% \begin{figure}[!t]
% \centering
% % \vspace{-0.75\baselineskip}
% \subfloat[]{
% \label{fig:BPF-model-mag-C2max}
% \includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_amp_vary_Cc_fixed_Cq_max.eps}
% }
% \hspace{-8pt} \hfill
% \subfloat[]{
% \label{fig:BPF-model-ph-C2max}
% \includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_phase_vary_Cc_fixed_Cq_max.eps}
% }
% \hspace{-8pt} \hfill
% \subfloat[]{
% \label{fig:BPF-model-gd-C2max}
% \includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_gd_vary_Cc_fixed_Cq_max.eps}
% }
% \vspace{-0.5\baselineskip}
% \caption{Measured and modeled: (a) magnitude, (b) phase, and (c) group delay of the implemented bandpass filter (BPF) response, $\BPFImplTF{}(f)$, with $C_2 = C_2^{\rm max}$ (i.e., lowest BPF quality factor).}
% \label{fig:BPF-model-C2max}
% \vspace{-\baselineskip}
% \end{figure}
%%

%%
\subsubsection{FDE Tap Model Validation}

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat[]{
\label{fig:BPF-model-mag-C2max}
\includegraphics[height=0.9in]{./figs/model/model_fde_amp.eps}
}
\hspace{-8pt} \hfill
\subfloat[]{
\label{fig:BPF-model-ph-C2max}
\includegraphics[height=0.9in]{./figs/model/model_fde_phase.eps}
}
\hspace{-8pt} \hfill
\subfloat[]{
\label{fig:BPF-model-gd-C2max}
\includegraphics[height=0.9in]{./figs/model/model_fde_gd.eps}
}
\vspace{-0.5\baselineskip}
\caption{Measured and modeled: (a) magnitude, (b) phase, and (c) group delay of the implemented FDE tap with varying combinations of $C_c$ and $C_Q$.}
\label{fig:impl-model-fde}
\vspace{-\baselineskip}
\end{figure}
%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/removed_validation.tex <==
In this section, we use model- and measurement-based simulations to evaluate both the RFIC and PCB RF SI canceller implementations. Throughout our evaluation, we use a \emph{real, practical} antenna interface response, $\SIChnlTF(f)$, measured using a $698$-$\SI{960}{MHz}$ swivel blade antenna with a coaxial circulator at frequency range $860$-$\SI{960}{MHz}$.


%%
%%
\subsection{Evaluation of the RFIC Canceller}
\label{ssec:eval-rfic}

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-rfic-sic-20mhz}
\includegraphics[width=0.49\columnwidth]{./figs/sim/sim_2nd_order_filter_bw_20mhz.eps}
}
\hspace{-10pt} \hfill
\subfloat{
\label{fig:eval-rfic-sic-bw-40mhz}
\includegraphics[width=0.49\columnwidth]{./figs/sim/sim_2nd_order_filter_bw_40mhz.eps}
}
\\ \vspace{-\baselineskip}
%%
\subfloat{
\label{fig:eval-rfic-sic-bw-60mhz}
\includegraphics[width=0.49\columnwidth]{./figs/sim/sim_2nd_order_filter_bw_60mhz.eps}
}
\hspace{-10pt} \hfill
\subfloat{
\label{fig:eval-rfic-sic-bw-80mhz}
\includegraphics[width=0.49\columnwidth]{./figs/sim/sim_2nd_order_filter_bw_80mhz.eps}
}
\vspace{-0.5\baselineskip}
\caption{Residual SI power level (reference to the original TX power lever) before and after the simulate RF SIC using varying number of filter taps, $\NumTap \in \{1,2,3,4\}$, and different desired RF SIC bandwidth of $\{20,40,60,80\}\thinspace\SI{}{MHz}$ as indicated by the range between the red dashed lines.}
\label{fig:eval-rfic-sic}
\vspace{-\baselineskip}
\end{figure}
%%

Our RFIC implementation in~\cite{Zhou_WBSIC_JSSC15} has only $\NumTap=2$ filter taps, achieving an average amount of $\SI{40}{dB}$ RF SIC across $\SI{27}{MHz}$ bandwidth. Since the model {\eqref{eq:rfic-tf}} matches with the implementation very closely \memoTC{Mahmood/Jin - maybe say more here about why this is true?} and can be scaled up to more filter taps, we perform simulation based on the model in {\eqref{eq:rfic-tf}} together with the proposed Algorithm~\ref{algo:opt-joint}.

%%
\subsubsection{The Ideal Case}
To evaluate and validate our concept of FDE, we simulated RF SIC with varying number of filter taps of $\NumTap \in \{1,2,3,4\}$ and desired RF SIC bandwidth of $\BW \in \{20,40,60,80\}\thinspace\SI{}{MHz}$. Fig.~\ref{fig:eval-rfic} presents the the amplitude responses of both the antenna interface (SI channel) and the residual SI power level after RF SIC. The power levels shown are referred to the circulator TX input \memoTC{double-confirm this}. The configurations the filter taps are obtained by solving the optimization problem {\eqref{eq:opt-joint-obj}} with the following constraints: $\Amp{i} \in [-40, -10]\thinspace\SI{}{dB}$, $\Phase{i} \in [-\pi, \pi]$, $\CenterFreq{i} \in [875, 925]\thinspace\SI{}{MHz}$, and $\QFactor{i} \in [1, 50]$, $\forall i$. These constraints are practically selected (e.g., without allowing extreme high quality factors, etc.) such that the values can be easily achieved in an RFIC implementation.

As Fig.~\ref{fig:eval-rfic-sic} shows, a larger number of $2$nd-order filter taps can significantly enhance the RF SIC bandwidth. In particular, under the same desired SIC bandwidth, a larger number of filter taps results in better average RF SIC as expected. For the case with only $\NumTap=2$ filter taps, an average value of $\SI{58}{dB}$ SIC can be achieved across $\SI{20}{MHz}$ bandwidth, but this value decreases to $\SI{47}{dB}$ with $\SI{40}{MHz}$ bandwidth. For the case with $\NumTap=4$ filter taps, an average amount of more than $\SI{56}{dB}$ RF SIC can be achieved for all considered SIC bandwidth up to $\SI{80}{MHz}$.
% Fig.~\ref{fig:theory-sim-varying-bw} also shows that the RF SIC performance does not degrade for $N=2,3$ FDE taps when the desired SIC bandwidth is increased, illustrating that $2$ or $3$ ideal FDE taps are robust to medium SIC bandwidth requirements.
Fig.~\ref{fig:eval-rfic-sic} also shows that in some scenarios, adding more filter taps does not help increase the amount of RF SIC. For example, since $\NumTap=3$ already achieves very good SIC across $\SI{20}{MHz}$ bandwidth, adding a fourth filter tap will only introduce minimal performance improvements. We would also like to note that the center frequency range of the $2$nd-order filters was constrained to be within a $\SI{50}{MHz}$ range, and performance improvements are expect by relaxing this constraint.


%%
\subsubsection{The Practical Case with Quantization Constraints}
In practice, the values of $\Amp{i}$, $\Phase{i}$, $\CenterFreq{i}$, and $\QFactor{i}$ can not be arbitrarily selected from a continuous range, and are often programmed at discrete values given the resolution of the hardware components. We evaluate the effect of quantization constraints in the following settings. For $\Amp{i}$, a $\SI{0.25}{dB}$ resolution is added to the constraint range of $\Amp{i} \in [-40, -10]\thinspace\SI{}{dB}$. For $\Phase{i} \in [-\pi, \pi]$, $\CenterFreq{i} \in [875, 925]\thinspace\SI{}{MHz}$, and $\QFactor{i} \in [1, 50]$, an $8$-bit resolution constraint was introduced, which is equivalent to $2^8=256$ discrete values with equal spacing within the given range. The quantized configurations of the filter taps are obtained by rounding the configurations returned in the continuous case above to their closest quantized values.

Fig.~\ref{fig:eval-rfic-sic-quantized} presents the the amplitude responses of both the antenna interface (SI channel) and the residual SI power after RF SIC for $\NumTap \in \{1,2,3,4\}$ and $\BW \in \{40, 80\}\thinspace\SI{}{MHz}$. The results for $\BW \in \{20, 60\}\thinspace\SI{}{MHz}$ are similar and thus omitted here. Comparing Fig.~\ref{fig:eval-rfic-sic-quantized} with (the right column of) Fig.~\ref{fig:eval-rfic-sic} shows that adding practical quantization constraint will slightly reduce the amount of RF SIC achieved across the desired bandwidth. In particular, the effect of quantized configurations is the most significant for the case with $\NumTap=4$ filter taps. This is because as more filter taps are available, more flexibility exists due to a larger number of variables that can be controlled. As a results, the performance of RF SIC becomes more sensitive to the coupling between the individual response of each filter tap. However, as Fig.~\ref{fig:eval-rfic-sic-quantized} suggests, even with the existence of such practical quantization constraints, $\NumTap=4$ filter taps can still achieve an average of $\SI{50}{dB}$ RF SIC across a $\SI{80}{MHz}$ bandwidth. Again, by relaxing the constraints (e.g., by using components with higher resolutions), performance improvements can reveal.

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-rfic-sic-quantized-bw-40mhz}
\includegraphics[width=0.49\columnwidth]{./figs/sim/sim_2nd_order_filter_bw_40mhz_quantized.eps}
}
\hspace{-10pt} \hfill
\subfloat{
\label{fig:eval-rfic-sic-quantized-bw-80mhz}
\includegraphics[width=0.49\columnwidth]{./figs/sim/sim_2nd_order_filter_bw_80mhz_quantized.eps}
}
\vspace{-0.5\baselineskip}
\caption{Residual SI power level (reference to the original TX power lever) before and after the simulate RF SIC with practical quantization constraints using varying number of filter taps, $\NumTap \in \{1,2,3,4\}$, and different desired RF SIC bandwidth of $\{40,80\}\thinspace\SI{}{MHz}$.}
\label{fig:eval-rfic-sic-quantized}
\vspace{-\baselineskip}
\end{figure}
%%


%%
%%
\subsection{Evaluation of the PCB Canceller}
\label{ssec:eval-pcb}
Now we turn to the evaluation of the PCB RF SI Canceller. We first perform experimental measurements to verify the BPF model derived in Section~\ref{ssec:model-pcb}, and then perform model-based simulation to evaluate the RF SIC performance.

\subsubsection{Validating the BPF Model, $\BPFTapTF{i}(f)$}
We first measure the S-Parameters (or equivalently, the transfer function) of the implemented BPF using a test structure to avoid the effects of other components on the PCB (see Fig.[BPF TEST STRUCTURE]). The measurements are conducted using varying programmed values of $\CapCF{}$ and $\CapQF{}$ and the results are averaged over $20$ measurements.
% Due to practical implementation losses, we use multi-dimensional curve-fitting to better tune parameters $L_1 = \SI{1.85}{nH}$ and $L_2 = \SI{3.28}{nH}$ (see Fig.~\ref{fig:impl-fde}).

Fig.~\ref{fig:eval-pcb-bpf} presents the amplitude, phase, and group delay of the BPF using both measurements and the model {\eqref{eq:pcb-bpf-tf}}. We consider both the highest and lowest tunable BPF quality factor by setting $\CapQF{} = \CapQF{}^{\rm min}$ and $\CapQF{} = \CapQF{}^{\rm max}$, respectively, corresponding to a tunable range of the BPF quality factor between $9.2$ and $17.8$. Note that without the impedance transforming networks, the quality factor of the center $LC$ resonance tank is \emph{fixed at only $2.7$}. Therefore, the impedance transformation networks provide a improved quality factor tuning range by $3.4 - 6.6\times$. Fig.~\ref{fig:eval-pcb-bpf} shows that our BPF model {\eqref{eq:pcb-bpf-tf}} matches very closely with the measurements at high BPF quality factor values (top row). In particular, the maximum differences between the measured and modeled magnitude and phase responses are $\SI{0.5}{dB}$ (or $5.9\%$) and $\SI{7}{deg}$, respectively. At the lowest BPF quality factor values, these errors increase to $\SI{1.2}{dB}$ (or $14.8\%$) and $\SI{15}{deg}$ (bottom row), while still showing a validated BPF model.

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-pcb-bpf-amp-CQmin}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_amp_CQmin.eps}
}
\hspace{-8pt} \hfill
\subfloat{
\label{fig:eval-pcb-bpf-phase-CQmin}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_phase_CQmin.eps}
}
\hspace{-8pt} \hfill
\subfloat{
\label{fig:eval-pcb-bpf-gd-CQmin}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_gd_CQmin.eps}
}
\\ \vspace{-1\baselineskip}
%%
\subfloat{
\label{fig:eval-pcb-bpf-amp-CQmax}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_amp_CQmax.eps}
}
\hspace{-8pt} \hfill
\subfloat{
\label{fig:eval-pcb-bpf-phase-CQmax}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_phase_CQmax.eps}
}
\hspace{-8pt} \hfill
\subfloat{
\label{fig:eval-pcb-bpf-gd-CQmax}
\includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_gd_CQmax.eps}
}
%%
\vspace{-0.5\baselineskip}
\caption{Measured and modeled magnitude, phase, and group delay of one implemented bandpass filter response (w/o amplitude and phase controls), with the highest quality factor value, $C_Q = C_Q^{\rm min}$ (top row) and the lowest quality factor value, $C_Q = C_Q^{\rm max}$ (bottow row), respectively.}
\label{fig:eval-pcb-bpf}
\vspace{-\baselineskip}
\end{figure}
%%

%%
% \begin{figure}[!t]
% \centering
% % \vspace{-0.75\baselineskip}
% \subfloat[]{
% \label{fig:BPF-model-mag-C2max}
% \includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_amp_vary_Cc_fixed_Cq_max.eps}
% }
% \hspace{-8pt} \hfill
% \subfloat[]{
% \label{fig:BPF-model-ph-C2max}
% \includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_phase_vary_Cc_fixed_Cq_max.eps}
% }
% \hspace{-8pt} \hfill
% \subfloat[]{
% \label{fig:BPF-model-gd-C2max}
% \includegraphics[width=0.33\columnwidth]{./figs/model/model_bpf_gd_vary_Cc_fixed_Cq_max.eps}
% }
% \vspace{-0.5\baselineskip}
% \caption{Measured and modeled: (a) magnitude, (b) phase, and (c) group delay of the implemented bandpass filter (BPF) response, $\BPFImplTF{}(f)$, with $C_2 = C_2^{\rm max}$ (i.e., lowest BPF quality factor).}
% \label{fig:BPF-model-C2max}
% \vspace{-\baselineskip}
% \end{figure}
%%

%%
\subsubsection{Validating the PCB Canceller Model, $\PCBTF(f)$}
The implemented PCB canceller presented in Section~\ref{ssec:model-pcb-impl} consists of $\NumTap=2$ BPF taps, as well as other components (e.g., power splitter/combiner and couplers, etc.). Therefore, a comprehensive model of the entire PCB canceller taking into account all the remaining components is needed to serve as the input to the tuning algorithm. We carefully measure the effect of other components and set $\Amp{0} = -\SI{4.1}{dB}$ and $\tau_0 = \SI{4.2}{ns}$ in {\eqref{eq:pcb-tf-calibrated}}. Note that the attenuators used have a maximal attenuation value of $\SI{16}{dB}$. Therefore, even at this maximal attenuation, signals can still travel through the BPF, making the entire response of the PCB canceller inseparable between the two FDE taps.

In order to validate our model, we measure the first BPF tap at its lowest attenuation value with varying values of $(\CapCF{}, \CapQF{})$ while setting the second tap with the highest attenuation value. The resultant amplitude, phase, and group delay from both measurements and the proposed model {\eqref{eq:pcb-tf-calibrated}} are presented in Fig.~\ref{fig:eval-pcb}. We also observe similar behaviors when turning on only the second tap. Since the attenuations are mostly independent, we use a ``weighted'' sum response for modeling $\PCBTF(f)$, where the weights are the independent attenuation values on each tap. \memoTC{need to further clarify here.}

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-pcb-amp}
\includegraphics[width=0.29\columnwidth]{./figs/model/model_fde_amp.eps}
}
\hspace{-12pt} \hfill
\subfloat{
\label{fig:eval-pcb-phase}
\includegraphics[width=0.29\columnwidth]{./figs/model/model_fde_phase.eps}
}
% \\ \vspace{-\baselineskip}
%%
\hspace{-12pt} \hfill
\subfloat{
\label{fig:eval-pcb-gd}
\includegraphics[width=0.435\columnwidth]{./figs/model/model_fde_gd.eps}
}
\vspace{-0.5\baselineskip}
\caption{Measured and modeled: (a) magnitude, (b) phase, and (c) group delay of the entire implemented PCB canceller with $\NumTap=2$ filter taps with varying combinations of $C_c$ and $C_Q$.}
\label{fig:eval-pcb}
\vspace{-\baselineskip}
\end{figure}
%%


%%
%%
\subsubsection{Model-based Numerical Evaluation}

Since our implemented PCB canceller only has $\NumTap=2$ FDE taps, we also perform model-based simulation to evaluate the performance of the PCB canceller with varying number of taps and desired RF SIC bandwidth, using the model developed above. The case with $\NumTap=2$ and $B=\SI{20}{MHz}$ is also experimentally evaluated in Section~\ref{sec:exp}.

We follow the same approaches in Section~\ref{ssec:eval-rfic}. Fig.~\ref{fig:eval-pcb-sic} presents the RF SIC of the PCB canceller with $\NumTap \in \{2,4\}$ and $B = \{40,80\} \SI{}{MHz}$, using our validated PCB canceller model presented above. We consider both cases with and without the adding the quantization constraints. As Fig.~\ref{fig:eval-pcb-sic} illustrates, the PCB canceller with $\NumTap=2$ FDE taps can achieve an average amount of $\SI{40}{dB}$ and $\SI{35}{dB}$ RF SIC across $\SI{40}{MHz}$ and $\SI{80}{MHz}$ bandwidth, respectively, even with the existence of practical quantization constraints. In addition, the PCB canceller achieves $\SI{50}{dB}$ RF SIC across $\SI{20}{MHz}$ in real-world experiments, as will be described in Section~\ref{sec:exp}. \memoTC{some concluding remarks here?}

%%
\begin{figure}[!t]
\centering
% \vspace{-0.75\baselineskip}
\subfloat{
\label{fig:eval-pcb-sic-bw-40mhz}
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_6th_order_filter_bw_40mhz.eps}
}
\hspace{-6pt} \hfill
\subfloat{
\label{fig:eval-pcb-sic-bw-80mhz}
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_6th_order_filter_bw_80mhz.eps}
}
\vspace{-0.5\baselineskip}
\caption{Residual SI power level (reference to the original TX power lever) before and after the simulate RF SIC with practical quantization constraints using varying number of filter taps, $\NumTap \in \{2,4\}$, and different desired RF SIC bandwidth of $\{40,80\} \SI{}{MHz}$.}
\label{fig:eval-pcb-sic}
\vspace{-\baselineskip}
\end{figure}
%%


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:


==> tex/sensitivity.tex <==
%%
%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat{
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_rfic_bw_20mhz_ideal.eps}
}
\subfloat{
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_pcb_bw_20mhz_ideal.eps}
}
\vspace{-0.5\baselineskip}
\\
\subfloat{
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_rfic_bw_40mhz_ideal.eps}
}
\subfloat{
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_pcb_bw_40mhz_ideal.eps}
}
\vspace{-0.5\baselineskip}
\\
\setcounter{subfigure}{0}
\subfloat[RFIC Canceller]{
\label{fig:sim-ideal-rfic}
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_rfic_bw_80mhz_ideal.eps}
}
\subfloat[PCB Canceller]{
\label{fig:sim-ideal-pcb}
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_pcb_bw_80mhz_ideal.eps}
}
% \vspace{-0.5\baselineskip}
\caption{TX/RX isolation of the antenna interface (black curve) and with the RFIC and PCB cancellers with varying number of FDE taps, $\NumTap$, and desired RF SIC bandwidth, $\BW$, \emph{in the ideal case}.}
\label{fig:sim-ideal}
\vspace{-\baselineskip}
\end{figure}
%% figure ends
%%
%%
In this section, we numerically evaluate and compare the performance of the FDE-based RFIC~\cite{Zhou_WBSIC_JSSC15} and PCB cancellers \emph{based on measurements and validated models}. We confirm that the PCB canceller emulates its RFIC counterpart and show that the optimized canceller configuration scheme can significantly improve the performance of the RFIC canceller. We also evaluate the performance of FDE-based cancellers with respect to the number of FDE taps, $\NumTap$, and desired RF SIC bandwidth, $\BW$, and discuss various design tradeoffs.

\subsection{Setup}
We use a real, practical antenna interface response, $\AntTF(f_k)$, measured in the same setting as described in Section~\ref{ssec:exp-testbed}, and consider $\NumTap \in \{1,2,3,4\}$ and $\BW \in \{20,40,80\}\thinspace\textrm{MHz}$. We only report the RF SIC performance with up to 4 FDE taps since, as we will show, this case can achieve sufficient RF SIC up to {80}\thinspace{MHz} bandwidth.\footnote{We select typical values of $20/40/80\thinspace\textrm{MHz}$ as the desired RF SIC bandwidth, since the circulator has a frequency range of {100}\thinspace{MHz}.}

We use {\eqref{eq:rfic-tf}} to both model and evaluate the RFIC canceller with configuration parameters $\{\ICTapAmp{i}, \ICTapPhase{i}, \ICTapCF{i}, \ICTapQF{i}\}$, since it is shown that a 2$^{\textrm{nd}}$-order BPF can accurately model the FDE $N$-path filter~\cite{Zhou_WBSIC_JSSC15}. Similar to {\OptProblemPCB} (see Section~\ref{ssec:impl-opt}), the optimized RFIC canceller configuration can be obtained by solving {\OptProblemIC} with $\ICTF(f_k)$ given by {\eqref{eq:rfic-tf}}.
%%
\begin{align*}
\OptProblemIC\ & \min: \littlesum_{k=1}^{\NumChnl} \NormTwo{\ICResTF(f_k)} = \littlesum_{k=1}^{\NumChnl} \NormTwo{ \AntTF(f_k) - \ICTF(f_k) }^2 \\
\textrm{s.t.:}\ & \ICTapAmp{i} \in [\ICTapAmpMin, \ICTapAmpMax],\ \ICTapPhase{i} \in [-\pi, \pi], \\
& \ICTapCF{i} \in [\ICTapCFMin, \ICTapCFMax],\ \ICTapQF{i} \in [\ICTapQFMin, \ICTapQFMax],\ \forall i.
\end{align*}
%%

\noindent Note that in~\cite{Zhou_WBSIC_JSSC15}, there is no optimization of the RFIC canceller configuration, and the canceller is configured based on a heuristic approach. As we will show, the optimized canceller scheme outperforms the heuristic approach by an order of magnitude in terms of the amount of RF SIC achieved.

%% figure begins
\begin{figure}[!t]
\centering
\vspace{-\baselineskip}
\subfloat{
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_rfic_bw_20mhz_quan.eps}
}
\subfloat{
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_pcb_bw_20mhz_quan.eps}
}
\vspace{-0.5\baselineskip}
\\ 
\subfloat{
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_rfic_bw_40mhz_quan.eps}
}
\subfloat{
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_pcb_bw_40mhz_quan.eps}
}
\vspace{-0.5\baselineskip}
\\ 
\setcounter{subfigure}{0}
\subfloat[RFIC Canceller]{
\label{fig:sim-quan-rfic}
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_rfic_bw_80mhz_quan.eps}
}
\subfloat[PCB Canceller]{
\label{fig:sim-quan-pcb}
\includegraphics[width=0.48\columnwidth]{./figs/sim/sim_pcb_bw_80mhz_quan.eps}
}
% \vspace{-0.5\baselineskip}
\caption{TX/RX isolation of the antenna interface (black curve) and with the RFIC and PCB cancellers with varying number of FDE taps, $\NumTap$, and desired RF SIC bandwidth, $\BW$, \emph{under practical quantization constraints}.}
\label{fig:sim-quan}
% \vspace{-\baselineskip}
\end{figure}
%% figure ends

The implemented PCB canceller includes only $\NumTap=2$ FDE taps due to its design (see Section~\ref{sec:impl}). However, it is practically feasible to include more parallel FDE taps. For numerical evaluation purposes, we model the PCB canceller with $\NumTap>2$ FDE taps by extending the validated model {\eqref{eq:pcb-tf-calibrated}} with symmetric FDE taps (i.e., all BPFs in the FDE taps behave identically). Although the canceller configuration scheme has a computational complexity of 4$^{\NumTap}$ (i.e., four DoF per FDE tap), we will show that $\NumTap=4$ taps can achieve sufficient amount of RF SIC in realistic scenarios.

In practice, the canceller configuration parameters cannot be arbitrarily selected from a continuous range as described in {\OptProblemPCB} and {\OptProblemIC}. Instead, they are often restricted to discrete values given the resolution of the corresponding hardware components. To address this problem, we evaluate the canceller models in both the \emph{ideal} case and the case \emph{with practical quantization constraints}. The canceller configuration with quantization constraints are obtained by rounding the configuration parameters returned by solving {\OptProblemPCB} or {\OptProblemIC} to their closest quantized values.

In particular, the RFIC canceller has the following constraints: $\forall i$, $\ICTapAmp{i} \in [-40, -10]\thinspace\textrm{dB}$, $\ICTapPhase{i} \in [-\pi, \pi]$, $\ICTapCF{i} \in [875, 925]\thinspace\textrm{MHz}$, and $\ICTapQF{i} \in [1, 50]$. When adding practical quantization constraints, we assume that the amplitude $\ICTapAmp{i}$ has a {0.25}\thinspace{dB} resolution. For $\ICTapPhase{i}$, $\ICTapCF{i}$, and $\ICTapQF{i}$, an 8-bit resolution constraint is introduced, which is equivalent to 256 discrete values spaced equally in the given range. These constraints are practically selected and can be easily realized in an IC implementation.  The PCB canceller model has following constraints: $\forall i$, $\PCBTapAmp{i} \in [-15.5, 0]\thinspace\textrm{dB}$, $\PCBTapPhase{i} \in [-\pi, \pi]$, $\PCBTapCFCap{i} \in [0.6,2.4]\thinspace\textrm{pF}$, and $\PCBTapQFCap{i} \in [2,14]\thinspace\textrm{pF}$. When adding the quantization constraints, we consider {0.5}\thinspace{dB}, {0.12}\thinspace{pF}, and {0.39}\thinspace{pF} resolution to $\PCBTapAmp{i}$, $\PCBTapCFCap{i}$, and $\PCBTapQFCap{i}$, respectively, and $\PCBTapPhase{i}$ has an 8-bit resolution. These numbers are consistent with our implementation and experiments (see Sections~\ref{ssec:impl-pcb} and~\ref{sec:exp}).

%%
%%
\subsection{Performance Evaluation and Comparison between the RFIC and PCB Cancellers}

Fig.~\ref{fig:sim-ideal} shows the TX/RX isolation achieved by the RFIC and PCB cancellers with optimized canceller configuration, with varying $\NumTap$ and $\BW$ in the ideal case (i.e., without quantization constraints). It can be seen that: (i) under a given value of $\BW$, a larger number of FDE taps results in higher average RF SIC, and (ii) for a larger value of $\BW$, more FDE taps are required to achieve sufficient RF SIC. For example, the ideal RFIC and PCB cancellers with 2 FDE taps can achieve an average $50/46/42\thinspace\textrm{dB}$ and $50/42/35\thinspace\textrm{dB}$ RF SIC across $20/40/80\thinspace\textrm{MHz}$ bandwidth, respectively.

Fig.~\ref{fig:sim-quan} shows the TX/RX isolation achieved by the RFIC and PCB cancellers with optimized canceller configuration under practical quantization constraints. Comparing to Fig.~\ref{fig:sim-ideal}, the results show a performance degradation due to limited hardware resolutions, which is more significant as $\NumTap$ increases. This is because a larger value of $\NumTap$ introduces a higher number of DoF with more canceller parameters that can be flexibly controlled. As a result, the RF SIC performance is more sensitive to the coupling between individual FDE tap responses after quantization. The results show that under practical constraints, the RFIC and PCB cancellers with 4 FDE taps can still achieve an average $54/50/45\thinspace\textrm{dB}$ and $52/45/39\thinspace\textrm{dB}$ RF SIC across $20/40/80\thinspace\textrm{MHz}$ bandwidth, respectively. Fig.~\ref{fig:sim-quan} also shows that the RFIC canceller under the optimized configuration scheme achieves a {10}\thinspace{dB} higher RF SIC compared with that achieved by the heuristic approach described in~\cite{Zhou_WBSIC_JSSC15} (labeled ``Heur'').

It is interesting to observe that the RF SIC profile of the PCB canceller with 2 FDE taps is very similar to our experimental results (see Fig.~\ref{fig:exp-usrp-algo} in Section~\ref{ssec:exp-node}). It is also worth noting that, in practice, adding more FDE taps cannot improve the amount of RF SIC in some scenarios (e.g., with {20}\thinspace{MHz} bandwidth), which is limited by the quantization constraints. However, performance improvement is expected by relaxing these constraints (e.g., through using components with higher resolutions and/or wider tuning ranges).
% Since the quantized FDE canceller configuration is only obtained after solving the original {\OptProblemPCB} in the continuous domain, negligible overhead will be introduced when finding the closest quantized values. ``Asymmetric'' FDE taps with different characteristics (i.e., center frequency) can also be designed to further enhance the performance.

%% table begins
\begin{table}[!t]
\caption{Comparison between the PCB and RFIC cancellers.}
\label{table:comparison-pcb-rfic}
\vspace{-\baselineskip}
\footnotesize
\begin{center}
% \begin{tabular}{| p{0.1\columnwidth} | p{0.2\columnwidth} | p{0.1\columnwidth} | p{0.2\columnwidth} |}
\begin{tabular}{|c|c|c|}
\hline
& PCB (this work) & RFIC~\cite{Zhou_WBSIC_JSSC15} \\
\hline
Center Frequency & {900}\thinspace{MHz} & {1.37}\thinspace{GHz} \\
\hline
\# of FDE Taps & 2 & 2 \\
\hline
Antenna Interface & \makecell{A single antenna \\ and a circulator} & \makecell{A TX/RX \\ antenna pair} \\
\hline
Antenna Isolation & {20}\thinspace{dB} & {35}\thinspace{dB} \\
% \hline
% Antenna Isolation & $\SI{20}{dB}$ & $\SI{32}{dB}$ \\
\hline
Canceller SIC ({20}\thinspace{MHz}) & {32}\thinspace{dB} & {20}\thinspace{dB} \\
\hline
Canceller Configuration & Optimization {\OptProblemPCB} & Heuristic \\
\hline
Digital SIC & {43}\thinspace{dB} & N/A \\
\hline
Evaluation & Node/Link/Network & Node \\
\hline
\end{tabular}
\end{center}
\vspace{-\baselineskip}
\end{table}
%% table ends

Table~\ref{table:comparison-pcb-rfic} shows the comparison between our implemented PCB canceller and the RFIC canceller presented in~\cite{Zhou_WBSIC_JSSC15}.
To summarize, we numerically show that the performance of the RFIC and PCB cancellers is similar. The results based on measurements and validated canceller models confirm that the PCB canceller accurately emulates its RFIC counterpart, and that the FDE-based approach is valid and suitable for achieving wideband RF SIC in small-form-factor devices.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../paper_fde"
%%% End:

